TNIC: A Trusted NIC Architecture

We introduce TNIC, a trusted NIC architecture for building trustworthy distributed systems deployed in heterogeneous, untrusted (Byzantine) cloud environments. TNIC builds a minimal, formally verified, silicon root-of-trust at the network interface level. We strive for three primary design goals: (1) a host CPU-agnostic unified security architecture by providing trustworthy network-level isolation; (2) a minimalistic and verifiable TCB based on a silicon root-of-trust by providing two core properties of transferable authentication and non-equivocation; and (3) a hardware-accelerated trustworthy network stack leveraging SmartNICs. Based on the TNIC architecture and associated network stack, we present a generic set of programming APIs and a recipe for building high-performance, trustworthy, distributed systems for Byzantine settings. We formally verify the safety and security properties of our TNIC while demonstrating its use by building four trustworthy distributed systems. Our evaluation of TNIC shows up to 6x performance improvement compared to CPU-centric TEE systems.

==> backups/background.tex <==
%\dimitra{Integrate that into the perforamnce part!Design Requirements for a Trusted NIC} \label{sec:background}

\if 0
\myparagraph{Requirements for security} In our \projecttitle{}, we materialize the theoretical principles of Clement et al.~\cite{clement2012} to design replication protocols for the modern cloud that meet the security and performance requirements of hosted applications without increasing the replication factor. This theoretical work sets the lower bound for transforming a CFT protocol into one that is Byzantine tolerant requiring the same replication degree as the CFT counterpart. Specifically, they have shown that such a translation {\em exists} if the following two properties are guaranteed:
\begin{itemize}
    \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
    \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
\end{itemize}

In \projecttitle{} we guarantee non-equivocation by assigning a monotonically increased trusted hardware counter (or sequencer) to each message before its transmission~\cite{clement2012, levin2009trinc, minBFT}. This technique forces a total order on network messages of sender allowing other (honest) nodes to detect missing (past) messages. For the transferable authentication property, the theoretical translation leverages digital signatures~\cite{10.1007/978-3-540-87779-0_2}. In our \projecttitle{} we decided against them due to their high computational latency. Instead, as in~\cite{levin2009trinc} we used cryptographic MACs along with a specific id that is uniquely bound to each device. We explain the \projecttitle{} mechanisms in $\S$~\ref{subsec:tfpga}.

%According to Clement et al~\cite{clement2012} the translated protocol needs to be adapted to ensure consistency and correctness, i.e., that the message that is received is legitimate. We have shown fapplications 
\fi 



\subsection{Summary: Research Question}
We advocate that modern distributed systems must be fast and trustworthy, operating correctly under the BFT model that characterizes the modern cloud infrastructure. We further showed that while TEEs could help in this direction, they cannot meet the requirements of such systems in terms of variations in performance. At the same time, they also have overheads in programmability and their security analysis.

To this end, we pose the following research question:
{\em How to design a network abstraction for high-perfomant trustworthy distributed systems under BFT that meets the {\bf performance} requirements of modern systems while it formally guarantees their {\bf secure and correct execution in the heterogeneous (Byzantine) cloud infrastructure}?}
%\pramod{I think this section should end with a new subsection or overall question on high-level design requirements for building high-performance trustworthy distributed systems.}

%In our work, we extend the scope of the FPGA-based SmartNICS~\cite{u280_smartnics, alveo_sn1000} to extend the security semantics of the network operations they provide . We implement a minimal TCB on the NIC level to materialize the aforementioned security properties (i.e., hardware-assisted authenticated equivocation-free messages) on the network data path eliminating the device communication costs. Our design choice of leveraging SmartNICs  is not hypothetical; SmartNIC devices have already been launched by major cloud providers~\cite{alibaba_smartnics, nitro_smartnics, msr_smartnics}.

%because their programmable FPGA allowing us to design and implement on hardware the security properties we need while all network traffic is on the communication path optimizing for latency~\cite{fpga_netstack}. %As such, FPGA-based SmartNICs are the best choice for our 

%mateterializing the security properties at the NIC level trusted hardware would allow us to generate and verify hardware-assisted authenticated equivocation-free messages on the network data path eliminating the device communication costs.

%To achieve that our work leverages the 
%SmartNIC devices~\cite{liquidIO_smartnics, u280_smartnics, bluefield_smartnics, broadcom_smartnics, netronome_smartnics, alibaba_smartnics, nitro_smartnics, msr_smartnics} that have already showed their performance benefits in networked systems~\cite{211249, 10.1145/3341302.3342079} and have already been launched by major cloud providers~\cite{alibaba_smartnics, nitro_smartnics, msr_smartnics}. % have launched SmartNICs in their datacenters to offload tasks from the host CPU onto dedicated hardware. 

%These devices present great opportunities for high-performant networking because they offer a fully programmable hardware ``on-path'' with the NIC device, e.g., (multicore) (ARM) cores~\cite{bluefield_smartnics, alibaba_smartnics, broadcom_smartnics, liquidIO_smartnics} and FPGAs~\cite{u280_smartnics, alveo_sn1000, msr_smartnics}. As such, we rely on FPGA-based SmartNICs because their on-path programmable FPGA allowing us to design and implement on hardware the security properties we need while all network traffic is on the communication path optimizing for latency~\cite{fpga_netstack}. %As such, FPGA-based SmartNICs are the best choice for our 

%These SmartNICs can be categorized into three different hardware designs: {\em (1)} ASIC-based NICs~\cite{netronome_smartnics} that have dedicated hardware for common network processing functions (TCP checksum and segmentation, RSS, etc.), {\em (2)} (multicore) SoC-based NICs~\cite{bluefield_smartnics, alibaba_smartnics, broadcom_smartnics, liquidIO_smartnics} that have an on-chip set of embedded (ARM) cores, and {\em (3)} FPGAs~\cite{u280_smartnics, alveo_sn1000, msr_smartnics} that introduce a fully programmable hardware ``on-path'' with the NIC device. 

%All these hardware designs for SmartNICs present different characteristics in performance and programmability. The ASIC NICs provide the highest performance potential but they suffer from a lack of programmability and adaptability over time~\cite{211249}. Current ASIC NIC designs cannot guarantee the properties of non-equivocation and transferable authentication and as such they are not an option for \projecttitle{}. On the other hand, the SoC-based SmartNICs are able to support our \projecttitle{} security requirements because their on-chip cores have full OS support and are fully programmable. However, we only had access to Bluefield 2~\cite{bluefield_smartnics} cards where the embedded cores are ``off-path'' with no support for DMA transfers between the on-chip and host memory. As such, a network operation would involve an extra (intra-host) operation for forwarding the request from the application to the device cores increasing the operation's latency.

%\projecttitle{} is built on top of the FPGA-based SmartNICs because they are combining the best of both worlds. First, the FPGAs are fully programmable allowing us to design and implement on hardware the exact security properties the \projecttitle{} requires. Secondly, the FPGA resides on-path with the NIC allowing \projecttitle{} to process all incoming/outgoing network traffic on the communication path optimizing for latency~\cite{fpga_netstack}. %As such, FPGA-based SmartNICs are the best choice for our \projecttitle{} design.

%These cloud solutions build primarily on top of programmable FPGA-based SmartNICs for acceleration or SoC-based SmartNICs that integrate off-path arrays of wimpy ARM cores (up to 16) to improve programmability (at the cost of performance).

%Our \trustednic{} has been built on top of FPGA-based SmartNICs to optimize for performance. \trustednic{} is an on-path SmartNIC that processes all incoming/outgoing messages directly on the communication path, ensuring that their security properties are met. In contrast, off-path SoC-based SmartNICs, which do not offer any security guarantees out of the box, do not optimize for performance. For example, the host needs to send the outgoing messages to the SoC cores for further processing. As DMA transfers are not supported between host and SoC cores, the re-routing is resolved at the NIC level, incurring extra overheads.

%Overall, \trustednic{} is a simpler SmartNIC because it just involves an FPGA on the communication path as in~\cite{msr_smartnics}. %Commercial SmartNICs are complete Systems-on-Chip, involving far more hardware (not
%only arrays of cores but also dedicated ASICs for network
%processing, packet switching, memory controllers, potentially
%storage controllers, etc.). As such, they can do more, but they
%also cost more, require more energy, and are more complex
%to deploy, program, and use.


==> backups/background_back.tex <==
\section{Design goals for the \projecttitle{} architecture}
\label{sec:requirements}
Our proposal for the design of a \projecttitle{} architecture targets to resolve the tension between security and performance when it comes to the design and implementation of replication protocols that are widely deployed in modern heterogeneous datacenters. To this end, our \projecttitle{} is specifically designed to help system designers build efficient, fault-tolerant, and robust systems under the presence of Byzantine actors in the untrusted cloud infrastructure. Specifically, our system targets the following design properties: 
\begin{itemize}
    \item {\bf{Robustness}} for building and deploying fault-tolerant distributed protocols and applications that remain correct and available in the untrusted cloud infrastructure.
    \item {\bf{Performance and scalability}} for efficiently exchanging and authenticating network messages. Particularly, our \projecttitle{} allows for BFT with the minimum possible number of involved servers ($2f+1$), mitigating clients' costs and resource usage.
    \item {\bf{Adaptability}} for allowing protocol designers to build robust protocols that can seamlessly run in modern heterogeneous DCs without them having to be BFT experts. 
\end{itemize}

\vspace{1pt}
Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 

\antonis{Consider another subsection here.}
Next, we explain the two core problems aroused from prior research efforts on BFT protocols and how our \projecttitle{} overcomes those.


%\dimitra{
%\begin{enumerate}
%    \item Problem
%    \item Prior work 
%    \item Our solution
%\end{enumerate}
%}

\myparagraph{Problem 1: Security and performance} Prior research~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} introduced replication protocols that are executed correctly in the presence of Byzantine actors (e.g., malicious adversaries, compromised participant nodes, faulty network links and memory). Unfortunately, while these protocols offer BFT, they give up on performance and scalability rendering them impractical for modern high-end distributed systems~\cite{bftForSkeptics}. 

More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.

\myparagraph{Proposal} In our work, we target to bridge this gap between robustness (BFT) and performance. Our \projecttitle{} offers the system designers the necessary foundations for building BFT protocols while it optimizes the performance and scalability of the derived protocols. Specifically, we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

More precisely, our design relies on the theoretical findings of Clement et al.~\cite{clement2012}. Their work has shown that a translation between any CFT protocol to a BFT protocol always exists iff the following properties are guaranteed:
\begin{itemize}
    \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
    \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
\end{itemize}

Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.

%In contrast, our trusted NIC allows heterogeneous nodes to communicate with each other in a secure manner over the untrusted cloud infrastructure. 
\myparagraph{Problem 2: Seamless adoption in heterogeneous DCs} While the classical BFT protocols significantly limit performance, a new line of research has made an attempt to optimize such protocols introducing a new family of hybrid BFT protocols that operate with fewer replicas. Hybrid BFT protocols~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} rely on Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}  to prevent equivocation.  Unfortunately, when it comes to their implementation, hybrid protocols have been built on top of specific and CPU-dependant TEEs---in fact, we found that all open-sourced hybrid protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are specifically built on top Intel SGX~\cite{intel-sgx}.

We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
\antonis{may mention arm as well?}
Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.

\myparagraph{Proposal} Our \projecttitle{} attacks this challenge and removes the protocols' dependencies on homogeneous CPUs and TEEs. We offer a unified abstraction, a network library ( ..), that allows designers to implement BFT protocols on various CPU machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%\dimitra{
%\begin{enumerate}
%    \item Problem
%    \item Prior work 
%    \item Our solution
%\end{enumerate}
%}

%Our proposal for the Trusted NIC architecture design needs to consider three design properties: security, performance and adaptability to heterogeneous host CPUs. Our system is based on a hardware-based trusted subsystem that guarantees the minimum properties that are required to be exposed to system and protocols designers to implement robust distributed protocols~\cite{} while it is designed for heterogeneous (untrusted) cloud infrastructures. 


%Prior research has introduced distributed (replication) protocols~\cite{} that are executed correctly even when some participants or parts of the infrastructure (e.g., network links, memory) are malicious, e.g., \emph{Byzantine}~\cite{}. Unfortunately, these protocols usually present a trade-off between performance and heterogenity. To operate under the Byzantine Fault Model~\cite{},  they need to increase their replication factor~\cite{}. Compared to the deployed protocols that only target crashed, but honest nodes (Crash Fault Model~\cite{}), traditional BFT protocols will add an extra $f$ set of replicas, in total $3f+1$ replicas to operate when up to $f$ nodes behave arbitrarily. As such, while necessary in the modern untrusted cloud infrastructure~\cite{}, these protocols have seen little recognition and adoption due to their performance and scalability limitations~\cite{}. On the other hand, state-of-the-art BFT protocols rely on trusted CPU-dependant hardware components (i.e., Trusted Execution Environments~\cite{}) to cut down on the replication factor using only $2f+1$ nodes. Unfortunately, their reliance on TEEs requires that all participant machines support such hardware which comes with different security guarantees and programmability. As such, these protocols give up on their adaptability to modern heterogeneous data centers. 


\dimitra{
\begin{itemize}
    \item section 2: requirements for robust distributed systems (problem/solution briefly)
    \item section 3: background on the technologies: smartNICs -- translation properties 
    \item section 4: overview --> Discuss the system/fault/threat model here too!
\end{itemize}
}






\section{Background} 

\myparagraph{Translation requirements}


\myparagraph{\trustednic{} compared to other SmartNICs}
SmartNIC devices~\cite{liquidIO_smartnics, u280_smartnics, bluefield_smartnics, broadcom_smartnics, netronome_smartnics, alibaba_smartnics, nitro_smartnics, msr_smartnics} have started to appear in several applications showing their benefits to both applications and network acceleration~\cite{211249, 10.1145/3341302.3342079}. Indeed, major cloud providers~\cite{alibaba_smartnics, nitro_smartnics, msr_smartnics} have launched SmartNICs in their datacenters to offload tasks from the host CPU cores onto dedicated hardware.
These cloud solutions build primarily on top of programmable FPGA-based SmartNICs for accelaration~\cite{msr_smartnics} or SoC-based SmartNICs~\cite{bluefield_smartnics} that integrate off-path arrays of wimpy ARM cores (up to 16) to improve programmability (at the cost of performance).

Our \trustednic{} has been built on top of FPGA-based SmartNICs to optimize for performance. \trustednic{} is an on-path SmartNIC that processes all incoming/outgoing messages directly on the communication path, ensuring that their security properties are met. In contrast, off-path SoC-based SmartNICs, which do not offer any security guarantees out of the box, do not optimize for performance. For example, the host needs to send the outgoing messages to the SoC cores for further processing. As DMA transfers are not supported between host and SoC cores, the re-routing is resolved at the NIC level, incurring extra overheads.

Overall, \trustednic{} is a simpler SmartNIC because it just involves an FPGA on the communication path as in~\cite{msr_smartnics}. %Commercial SmartNICs are complete Systems-on-Chip, involving far more hardware (not
%only arrays of cores but also dedicated ASICs for network
%processing, packet switching, memory controllers, potentially
%storage controllers, etc.). As such, they can do more, but they
%also cost more, require more energy, and are more complex
%to deploy, program, and use.


==> backups/conclusion.bak.tex <==
\section{Discussion and Limitations}
\pramod{maybe instead of general conclusion - we can write this section as two paragraphs: 1) Discussion on generality (see the last sentence), and 2) limitations.}
In this paper, we present the design and implementation of \projecttitle{}, a trusted NIC architecture. \projecttitle{} proposes a host CPU-agnostic unified security architecture based on trustworthy network-level isolation. We materialize the \projecttitle{} architecture using SmartNICs by exposing a minimal and formally verified silicon root-of-trust with low TCB, relying on just two fundamental properties of transferable authentication and non-equivocation. Using \projecttitle{}, we implement a hardware-accelerated trustworthy network stack that efficiently transforms a range of distributed systems under the fail-stop operation model for untrusted (Byzantine) cloud environments. Notably, we realize the \projecttitle{} architecture-based FPGA-based SmartNICs on Alveo U280 cards; we believe other commercial SmartNIC vendors can implement our NIC-level interface.


%\projecttitle{} outperforms the state-of-the-art CPU-based trusted hardware, TEEs, while offering a unified, general, programmable, formally verified, and minimalist interface to build trustworthy distributed systems. 
\myparagraph{Ethical considerations and artifact availability} This work raises no ethical issues. The \projecttitle{} (HW and SW) artifact and formal security proofs will be publicly available.

% We present \projecttitle{}, a trusted NIC architecture for trustworthy distributed systems. \projecttitle{} leverages the state-of-the-art network hardware, i.e., SmartNICs and extends their security properties, implementing a minimalistic TCB, the attestation kernel that materializes the lower bound of properties---the non-equivocation and transferable authentication properties---to transform distributed systems for Byzantine settings. We formally verified the security and safety properties of \projecttitle{} while we also applied it to transform four systems: a single-node trusted log system, a state-machine-replication (SMR) protocol, a chain replication system and an accountability protocol. Our evaluation shows that \projecttitle{} outperforms the state-of-the-art CPU-based trusted hardware, TEEs while offering unification, generality and minimalism.



% \section{Conclusion}
% In this paper, we present the design and implementation of \projecttitle{}, a trusted NIC architecture. Our, we make the following contributions:
% \begin{itemize}[leftmargin=*]
%     \item We designed and built \projecttitle{}, a {\em host-agnostic unified trusted high-performant} NIC architecture for building fast and trustworthy systems in the heterogeneous cloud infrastructure. We expose a trusted network programming library that offers the powerful properties of non-equivocation and transferable authentication to system designers while we show {\em how} to strengthen existent systems with \projecttitle{}.
%     %\dimitra{Hardware level implementation + minimalism taht allows verifiable + NIC level implementation tfor high performance}
%     \item We offer a {\em unified minimalistic verifiable silicon root of trust (TCB)}  that realizes an efficient transformation between existing system under the fail-stop operation model for the Byzantine settings in the cloud. We further conduct an end-to-end formal verification of our \projecttitle{} operations from bootstrapping and remote attestation to normal operation.
%     \item We built \projecttitle{} extending the scope of the state-of-the art SmartNIC devices to boost performance. We built our minimalistic TCB, \projecttitle{} attestation kernel, in NIC-level hardware by extending and shielding an FPGA-based RDMA network stack.
    
% \end{itemize}

%  We formally verified the security and safety properties of \projecttitle{} while we also applied it to transform four distributed systems: Attested Append-Only Memory (A2M), Byzantine Fault Tolerance (BFT), Chain Replication, and Accountable Distributed Systems using PeerReview. Our evaluation shows that \projecttitle{} outperforms the state-of-the-art CPU-based trusted hardware, TEEs while offering unification, generality and minimalism.

==> backups/design-overview.tex <==
%\section{Design}
%\dimitra{
%\begin{itemize}
%    \item Intro
%    \item Background + Motivation
%    \item Overview (including sys/data model etc.)
%    \item Design + Implementation (TNIC: hw architecture, TNIC libraries: sw abstraction, Applications: use-cases)
%\end{itemize}
%}


\subsection{System Model}

\myparagraph{Model sketch}
We model the distributed system as a set of {\tt N} nodes each of which is attached to a single \projecttitle{} instance that is loaded into an FPGA-based SmartNIC as Alveo U280~\cite{u280_smartnics}. The nodes communicate by exchanging messages through bi-directional network links that connect their FPGAs. The system is managed and owned by the third-party cloud infrastructure which is untrusted.

\myparagraph{Threat model}
We target a strong adversary that can gain full control over the cloud infrastructure including any privileged CPU software (e.g., the OS, VMM, and device drivers) and the FPGA-based SmartNIC devices (post-manufacturing). Such an adversary can also have full access to the infrastructure (e.g., shutdown the servers, or even try to re-program the FPGAs) although, as in ~\cite{levin2009trinc, minBFT, Castro:2002} they cannot compromise the cryptographic primitives. As in~\cite{10.1145/3503222.3507733, 10.1145/2168836.2168866}, we further assume that the physical package, supply chain, and manufacturer of the FPGAs are trusted.  The bitstreams are implemented and synthesized correctly whereas any secret data are distributed securely using remote attestation ($\S$~\ref{subsec:nic_attest_kernel}). The tool flow used to generate the accelerator is trusted and run in a secure environment for covert channels resilience. 

The host CPU is considered untrusted and we do not rely on any CPU TEE. Specifically, while we use the application code to transfer data, we assume the host CPU is untrusted, i.e., can exhibit Byzantine behavior~\cite{Lamport:1982}, as well as the local host memory, storage, etc. Similarly, we make no assumptions about the network infrastructure, e.g., adversaries can drop, re-order, double-send, read, and manipulate the messages in any way. 

We do not consider denial-of-service (DoS) attacks; the cloud provider has physical control of the hardware and can simply unpower it. Nevertheless such attacks affect availability and not the correctness.


%The CSP is incentivized to prevent DoS attacks due to the revenue loss when the FPGA instance is unavailable. %We do not consider attacks against the CSP, as the Shell already protects against malicious FPGA users. 


%We trust that the RDMA stack, along with the attestation kernel, are implemented and synthesized correctly, whereas the bitstream and the keys are distributed and flushed to the FPGAs securely using remote attestation.





%The \projecttitle{} architecture implements a  network stack, similarly to~\cite{erpc, rdma-scale}, but focuses on security leveraging SmartNICs---specifically, FPGA-based NICs~\cite{intel_smartnics, alveo_smartnics}. 




\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/trusted-nic-attestation_kernel.drawio.pdf}
    \caption{\trustedfpga{} attestation kernel overview (transmission path).}
    \label{fig:attestation_kernel}
\end{figure}    
\fi




\subsection{Design Challenges}
\myparagraph{Challenge \#1: Robustness} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and, importantly, can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.


\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}.  Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 

==> backups/design_challenges.bak.tex <==
\section{Overview}
\subsection{Design goals and overview}
\label{sec:requirements}
\pramod{let's keep it consistent high-performance trustworthy distributed systems.}
We propose a trusted NIC architecture to accommodate the requirements for high-performant trustworthy distributed systems for the untrusted cloud infrastructure. Our trusted NIC aims to attack the trade-offs between performance, security, and heterogeneity, targeting the following design goals:

\pramod{i think it's still not crystal clear the three design goals. Nevertheless we should blend the formal verification part of it.}
\begin{itemize}
    \item {\bf{Security}} for guaranteeing the correct execution of a distributed system in the Byzantine (untrusted) cloud infrastructure.
    \item {\bf{Unification and minimalism}} for {\em seamlessly} building distributed systems with strong security in the heterogeneous cloud infrastructure. 
    \item {\bf{High-performance networking}} for efficiently exchanging and authenticating network messages required for BFT guarantees.
\end{itemize}


%\subsection{\projecttitle{} Overview} 

\myparagraph{System overview} To this end, we propose \projecttitle{}, a trusted NIC architecture that fulfills the aforementioned design goals. Figure~\ref{fig:overview} shows the high-level overview of our \projecttitle{} system. A \projecttitle{} system must be attached to each participating machine of the distributed application.% A \projecttitle{} instance is connected to the (host) CPU through the PCIe~\cite{pcie} whereas the distributed \projecttitle{} instances are connected through direct (Ethernet) links or a switch. 


\pramod{i think it would be good to explain the system components in bottom up manner because this is how we structure the design section.}

\pramod{please highlight each componenent in BOLD.}

As shown in Figure~\ref{fig:overview}, \projecttitle{} is comprised of three layers: (1) the \projecttitle{} trusted network library (blue box) that exposes \projecttitle{}'s programming API ($\S$~\ref{sec:t-nic-software}) to the application layer, (2) the \projecttitle{} trusted system network stack (yellow box) that intermediates between the application layer and the \projecttitle{} hardware access ($\S$~\ref{sec:t-nic-network}) and (3) the \projecttitle{} hardware architecture (green box) that implements trusted network operations on top of SmartNIC devices ($\S$~\ref{sec:t-nic-hardware}). 


\pramod{Same here -- bottom up explaination.}
The  \projecttitle{} trusted network library (blue box) exposes a {\em trusted} API that is built on top of one-sided RDMA (reliable) operations. The \projecttitle{} trusted network stack (yellow box) runs in user-space and it is responsible for configuring the \projecttitle{} device (MAC address, IP, etc.), while it runtime if offers kernel-bypass device access for low-latency operations. Lastly, the \projecttitle{} hardware architecture (green box) implements and extends the networking IB/RDMA protocol~\cite{rdma_specification} on top of the FPGA-based SmartNIC devices, Alveo U280~\cite{u280_smartnics}. Critically, it extends the conventional protocol implementation with a minimal hardware security module, the attestation kernel, to efficiently materialize the security properties of the non-equivocation and the transferable authentication.


%The hardware implementation of \projecttitle{} runs the RDMA protocol on top of FPGA-based SmartNIC hardware. We further extend the network protocol kernel with a minimal hardware security module, the attestation kernel which shields and verifies the network traffic across the participant nodes. Specifically, the security module  constructs a secure message format that is verifiable and the network stack module implements the RDMA network protocol. In contrast to the control and configuration paths shown in Figure~\ref{fig:overview}, the message to be sent, is fetched from the application's memory directly to the device through DMA transfers. After being shielded, the message is then forwarded to the network stack module for transmission.  % to preserve the authentication and non-equivocation properties across all network operations.
%On top of our trusted network stack, we implement a networking library, \projectlibrary{}, that exposes the developers to the classical RDMA API enhanced with two security properties, i.e., the transferable authentication and the non-equivocation.


\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.5\textwidth]{figures/trusted-nic-overview.drawio.pdf}
    \includegraphics[width=0.45\textwidth]{figures/system_overview-2.pdf}
    \caption{\projecttitle{} system overview.}
    \label{fig:overview}
\end{figure}


%Our proposal for \projecttitle{} seeks to resolve the tension between security and performance for (distributed) applications in the modern cloud infrastructure, specifically targeting replication protocols\pramod{focus on building trusted distributed systems -- PLEASE DONT MAKE THIS PAPER a REPLICATION protocol paper.}. To this end, our goal is to help system designers to build efficient, fault-tolerant, and robust systems that remain correct even when the untrusted cloud infrastructure fails arbitrarily. 

%\section{Design}
%\dimitra{
%\begin{itemize}
%    \item Intro
%    \item Background + Motivation
%    \item Overview (including sys/data model etc.)
%    \item Design + Implementation (TNIC: hw architecture, TNIC libraries: sw abstraction, Applications: use-cases)
%\end{itemize}
%}


%\subsection{System Model}

%\myparagraph{Model sketch}
%We model the distributed system as a set of {\tt N} nodes each of which is attached to a single \projecttitle{} instance that is loaded into an FPGA-based SmartNIC as Alveo U280~\cite{u280_smartnics}. The nodes communicate by exchanging messages through bi-directional network links that connect their FPGAs. The system is managed and owned by the third-party cloud infrastructure which is untrusted.

\myparagraph{Threat model} We inherit the fault and threat model from the classical BFT~\cite{Castro:2002} and trusted computing domains~\cite{intel-sgx} where the cloud infrastructure, e.g., machines, network, etc. can exhibit (Byzantine) arbitrary behavior. In addition, a \projecttitle{} system is subject to privileged attackers that can gain control over the host CPU, including the privileged software (e.g., the OS, VMM, and device drivers) and the FPGA-based SmartNIC devices (post-manufacturing). Such a powerful adversary can even attempt to re-program the FPGA; however, they cannot compromise the cryptographic primitives as in~\cite{levin2009trinc, minBFT, Castro:2002}. 

We assume that the physical package, supply chain, and manufacturer of the SmartNICs are trusted~\cite{10.1145/3503222.3507733, 10.1145/2168836.2168866}. The \projecttitle{} implementation (bitstream) is synthesized by a trusted IP vendor with a trusted tool flow that runs in a secure environment (for covert channels resilience). The protocol designers source the \projecttitle{} from trusted IP vendors.

%We do not consider denial-of-service (DoS) attacks; the cloud provider has physical control of the hardware and can simply unpower it. Nevertheless such attacks affect availability and not the correctness.


%( target a strong adversary that can gain full control over the cloud infrastructure including any privileged CPU software (e.g., the OS, VMM, and device drivers) and the FPGA-based SmartNIC devices (post-manufacturing). Such an adversary can also have full access to the infrastructure (e.g., shutdown the servers, or even try to re-program the FPGAs) although, as in ~\cite{levin2009trinc, minBFT, Castro:2002} they cannot compromise the cryptographic primitives. As in~\cite{10.1145/3503222.3507733, 10.1145/2168836.2168866}, we further assume that the physical package, supply chain, and manufacturer of the FPGAs are trusted. The bitstreams are implemented and synthesized correctly whereas any secret data are distributed securely using remote attestation ($\S$~\ref{subsec:nic_attest_kernel}). The tool flow used to generate the accelerator is trusted and run in a secure environment for covert channels resilience. 

%The host CPU is considered untrusted and we do not rely on any CPU TEE. Specifically, while we use the application code to transfer data, we assume the host CPU is untrusted, i.e., can exhibit Byzantine behavior~\cite{Lamport:1982}, as well as the local host memory, storage, etc. Similarly, we make no assumptions about the network infrastructure, e.g., adversaries can drop, re-order, double-send, read, and manipulate the messages in any way. 

%We do not consider denial-of-service (DoS) attacks; the cloud provider has physical control of the hardware and can simply unpower it. Nevertheless such attacks affect availability and not the correctness.


%The CSP is incentivized to prevent DoS attacks due to the revenue loss when the FPGA instance is unavailable. %We do not consider attacks against the CSP, as the Shell already protects against malicious FPGA users. 


%We trust that the RDMA stack, along with the attestation kernel, are implemented and synthesized correctly, whereas the bitstream and the keys are distributed and flushed to the FPGAs securely using remote attestation.





%The \projecttitle{} architecture implements a  network stack, similarly to~\cite{erpc, rdma-scale}, but focuses on security leveraging SmartNICs---specifically, FPGA-based NICs~\cite{intel_smartnics, alveo_smartnics}. 




\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/trusted-nic-attestation_kernel.drawio.pdf}
    \caption{\trustedfpga{} attestation kernel overview (transmission path).}
    \label{fig:attestation_kernel}
\end{figure}    
\fi

\pramod{we should not restrict ourselves to replication protocols.}

\pramod{Minimalism and verifiabile hardware interface should be a separate challenge.}

\subsection{Design Challenges}
\projecttitle{} aims to offer high-performant and unified trusted networking that can apply to a wide range of distributed systems. As such, we need to overcome the following challenges:

\myparagraph{Challenge \#1: Performance vs. security} Distributed systems in the third-party cloud infrastructure need to be fast, scalable, and trustworthy. While performance is critical in all of them, with TEEs themselves introducing significant performance limitations, the problem is even more exacerbated in fault-tolerant systems. Building replication protocols for distributed systems under the Byzantine fault model has always been a complex endeavor with performance, scalability, and engineering challenges~\cite{bftForSkeptics}. Even well-studied protocols, e.g., PBFT~\cite{Castro:2002}, are limited in scalability (it requires at least $f$ nodes w.r.t to its CFT counterpart), incur high latency (it runs three all-to-all broadcasting phases with $O(n^2)$ message complexity) and are hard to verify and optimize~\cite{10.1145/2658994}.


\myparagraph{Solution} Our \projecttitle{} bridges the gap between performance, scalability, and security. We implement a minimal TCB, the attestation kernel ($\S$~\ref{subsec:nic_attest_kernel}), that materializes all the necessary properties for transforming systems for Byzantine settings. We build the attestation kernel as part of the state-of-the-art NIC hardware for high performance ($\S$~\ref{subsec:roce_protocol_kernel}). The semantics we provide are powerful and generic too; we can use \projecttitle{} to transform a wide range of distributed systems for Byzantine settings (we show four use-cases in $\S$~\ref{sec:use_cases})  and even for transforming CFT replication protocols to BFT ones with the same number of machines as the CFT protocol. As such, our \projecttitle{} improves scalability compared to traditional BFT systems. We show this generic {\em recipe} of such a transformation using \projecttitle{} in $\S$~\ref{subsec:transformation}.

%protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%\myparagraph{Challenge \#1: Security vs high-performance} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

%\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.

\myparagraph{Challenge \#2: Minimalism vs TEEs TCBs} 

\myparagraph{Challenge \#2: Safety vs Heterogeneity} Prior BFT systems with trusted hardware were implemented on top of CPU-specific TEEs. In fact, we found that almost all of the open-source system implementations~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a}  require {\em homogeneous} {\tt x86} machines with SGX extensions of a specific version; a trusted hardware that for long had been under fire for its major security vulnerabilities~\cite{intel_sgx_vulnerabilities1, intel_sgx_vulnerabilities2, intel_sgx_vulnerabilities3, intel_sgx_vulnerabilities4, intel_sgx_vulnerabilities5}. Safety in BFT systems has always been a concern---e.g., Zyzzyva~\cite{unsafe_Zyzzyva} has proven to be unsafe almost ten years after its original publication---let alone when distributed systems rely on unstable heterogeneous TEEs.  

\myparagraph{Solution} To attack this challenge, \projecttitle{}'s key idea is minimalism. We design a minimalistic fully verifiable (TCB) attestation kernel at NIC-hardware level that exposes a unified API to system designers. As such, we offer BFT while removing the distributed system's dependencies on the host CPU, rendering our approach highly favorable in the heterogeneous cloud infrastructure. In addition, our minimalistic hardware-assisted TCB allows us to fully verify the safety and security properties of our \projecttitle{} from its initialization and remote attestation process to its normal operation ($\S$~\ref{subsec::formal_verification_remote_attestation}).

%\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

%\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


%\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}. Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


%\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 


\if 0

\subsection{Design Challenges}
\dimitra{here}
\myparagraph{Challenge \#1: Security} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and, importantly, can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.


\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}. Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 
\fi

==> backups/design_challenges.bak2.tex <==
\section{Overview}

% \subsection{Design Goals and System Overview}
% \label{sec:requirements}
% %\pramod{let's keep it consistent high-performance trustworthy distributed systems.}
% We propose a trusted NIC architecture to accommodate the requirements for high-performant trustworthy distributed systems for the untrusted cloud infrastructure. Our trusted NIC aims to attack the trade-offs between performance, security, and heterogeneity, targeting the following design goals:

% %\pramod{i think it's still not crystal clear the three design goals. Nevertheless we should blend the formal verification part of it.}
% \begin{itemize}
%     \item {\bf{A host CPU-agnostic unified security architecture.}} We need to provide foundational security guarantees across the network for building distributed systems that offer correct execution in the Byzantine (untrusted) cloud infrastructure.
%     \item {\bf{A minimalistic and verifiable TCB based on a silicon root-of-trust.}} Our system needs to offer a unified trusted network silicon root of trust that is host-agnostic for building trustworthy systems across heterogeneous machines in the cloud. Additionally, we strive for minimalism as the key component to offer a verifiable yet stable silicon root of trust.
%     \item {\bf{Hardware-accelerated trustworthy network stack.}} We need to offer high performance trusted network operations that are at the core of any distributed (networked) system in the cloud infrastructure.
% \end{itemize}


% %\subsection{\projecttitle{} Overview} 

% \myparagraph{System overview} To this end, we propose \projecttitle{}, a trusted NIC architecture that fulfills the aforementioned design goals. Figure~\ref{fig:overview} shows the high-level overview of our \projecttitle{} system. A \projecttitle{} system must be attached to each participating machine of the distributed application.% A \projecttitle{} instance is connected to the (host) CPU through the PCIe~\cite{pcie} whereas the distributed \projecttitle{} instances are connected through direct (Ethernet) links or a switch. 


%\pramod{i think it would be good to explain the system components in bottom up manner because this is how we structure the design section.}

%\pramod{please highlight each componenent in BOLD.}



\subsection{System Overview}
We advocate that modern distributed systems must be fast and trustworthy, operating correctly under the BFT model that characterizes the modern cloud infrastructure. We further show that while TEEs could help in this direction, they cannot meet the requirements of such systems in terms of variations in performance. At the same time, they also have overheads in programmability and their security analysis.

To this end, we propose \projecttitle{}, a trusted NIC architecture for high-performance and trustworthy distributed systems under BFT, formally guaranteeing their secure and correct execution in the heterogeneous cloud infrastructure. 
% To this end, we propose \projecttitle{}, a trusted NIC architecture that offers a network abstraction for high-performance, trustworthy distributed systems under BFT that meets the performance requirements of modern systems while it formally guarantees their secure and correct execution in the heterogeneous (Byzantine) cloud infrastructure. 
As shown in Figure~\ref{fig:overview}, \projecttitle{} is comprised of three layers: {\bf (1)  the \projecttitle{} hardware architecture} (green box) that implements trusted network operations on top of SmartNIC devices ($\S$~\ref{sec:t-nic-hardware}), {\bf (2) the \projecttitle{} trusted network stack} (yellow box) that intermediates between the application layer and the \projecttitle{} hardware ($\S$~\ref{sec:t-nic-network}), and {\bf (3)  the \projecttitle{} trusted network library} (blue box) that exposes \projecttitle{}'s programming API ($\S$~\ref{sec:t-nic-software}) to the application layer. 

Our \projecttitle{} hardware architecture implements and extends the networking IB/RDMA protocol~\cite{rdma_specification} on FPGA-based SmartNICs~\cite{u280_smartnics}. 
Specifically, it extends the conventional protocol implementation with a minimal hardware module, the attestation kernel, that materializes the security properties of the non-equivocation and transferable authentication. The \projecttitle{} network stack runs in user space and configures the \projecttitle{} device (MAC address, IP, etc.) on the control path, while it offers the data path as kernel-bypass device access for low-latency operations. Lastly, the  \projecttitle{} network library exposes a {\em trusted} API built on top of one-sided RDMA (reliable) operations. 
% Our \projecttitle{} hardware architecture implements and extends the networking IB/RDMA protocol~\cite{rdma_specification} on top of the FPGA-based SmartNICs, Alveo U280~\cite{u280_smartnics}. Critically, it extends the conventional protocol implementation with a minimal hardware security module, the attestation kernel, that materializes the security properties of the non-equivocation and the transferable authentication. The \projecttitle{} trusted network stack runs in user space. It configures the \projecttitle{} device (MAC address, IP, etc.) on the control path, while the data path is offered as kernel-bypass device access for low-latency operations. Lastly, The  \projecttitle{} trusted network library exposes a {\em trusted} API that is built on top of one-sided RDMA (reliable) operations. 

\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.5\textwidth]{figures/trusted-nic-overview.drawio.pdf}
    \includegraphics[width=0.38\textwidth]{figures/system_overview-2.pdf}
    \caption{\projecttitle{} system overview.}
    \label{fig:overview}
\end{figure}
%The hardware implementation of \projecttitle{} runs the RDMA protocol on top of FPGA-based SmartNIC hardware. We further extend the network protocol kernel with a minimal hardware security module, the attestation kernel which shields and verifies the network traffic across the participant nodes. Specifically, the security module  constructs a secure message format that is verifiable and the network stack module implements the RDMA network protocol. In contrast to the control and configuration paths shown in Figure~\ref{fig:overview}, the message to be sent, is fetched from the application's memory directly to the device through DMA transfers. After being shielded, the message is then forwarded to the network stack module for transmission.  % to preserve the authentication and non-equivocation properties across all network operations.
%On top of our trusted network stack, we implement a networking library, \projectlibrary{}, that exposes the developers to the classical RDMA API enhanced with two security properties, i.e., the transferable authentication and the non-equivocation.




%Our proposal for \projecttitle{} seeks to resolve the tension between security and performance for (distributed) applications in the modern cloud infrastructure, specifically targeting replication protocols\pramod{focus on building trusted distributed systems -- PLEASE DONT MAKE THIS PAPER a REPLICATION protocol paper.}. To this end, our goal is to help system designers to build efficient, fault-tolerant, and robust systems that remain correct even when the untrusted cloud infrastructure fails arbitrarily. 

%\section{Design}
%\dimitra{
%\begin{itemize}
%    \item Intro
%    \item Background + Motivation
%    \item Overview (including sys/data model etc.)
%    \item Design + Implementation (TNIC: hw architecture, TNIC libraries: sw abstraction, Applications: use-cases)
%\end{itemize}
%}


%\subsection{System Model}

%\myparagraph{Model sketch}
%We model the distributed system as a set of {\tt N} nodes each of which is attached to a single \projecttitle{} instance that is loaded into an FPGA-based SmartNIC as Alveo U280~\cite{u280_smartnics}. The nodes communicate by exchanging messages through bi-directional network links that connect their FPGAs. The system is managed and owned by the third-party cloud infrastructure which is untrusted.

\subsection{Threat Model} We inherit the fault and threat model from the classical BFT~\cite{Castro:2002} and trusted computing domains~\cite{intel-sgx}. The cloud infrastructure (machines, network, etc.) can exhibit Byzantine behavior while it is subject to attackers that can gain control over the host CPU (e.g., the OS, VMM, etc.) and the SmartNICs (post-manufacturing). The adversary can attempt to re-program the SmartNIC, but they cannot compromize the cryptographic primitives~\cite{levin2009trinc, minBFT, Castro:2002}. The physical package, supply chain, and manufacturer of the SmartNICs are trusted~\cite{10.1145/3503222.3507733, 10.1145/2168836.2168866}. The \projecttitle{} implementation (bitstream) is synthesized by a trusted IP vendor with a trusted tool flow for covert channels resilience. %(in a trusted environment) The system designers source the \projecttitle{} from trusted IP vendors.

%We do not consider denial-of-service (DoS) attacks; the cloud provider has physical control of the hardware and can simply unpower it. Nevertheless such attacks affect availability and not the correctness.


%( target a strong adversary that can gain full control over the cloud infrastructure including any privileged CPU software (e.g., the OS, VMM, and device drivers) and the FPGA-based SmartNIC devices (post-manufacturing). Such an adversary can also have full access to the infrastructure (e.g., shutdown the servers, or even try to re-program the FPGAs) although, as in ~\cite{levin2009trinc, minBFT, Castro:2002} they cannot compromise the cryptographic primitives. As in~\cite{10.1145/3503222.3507733, 10.1145/2168836.2168866}, we further assume that the physical package, supply chain, and manufacturer of the FPGAs are trusted. The bitstreams are implemented and synthesized correctly whereas any secret data are distributed securely using remote attestation ($\S$~\ref{subsec:nic_attest_kernel}). The tool flow used to generate the accelerator is trusted and run in a secure environment for covert channels resilience. 

%The host CPU is considered untrusted and we do not rely on any CPU TEE. Specifically, while we use the application code to transfer data, we assume the host CPU is untrusted, i.e., can exhibit Byzantine behavior~\cite{Lamport:1982}, as well as the local host memory, storage, etc. Similarly, we make no assumptions about the network infrastructure, e.g., adversaries can drop, re-order, double-send, read, and manipulate the messages in any way. 

%We do not consider denial-of-service (DoS) attacks; the cloud provider has physical control of the hardware and can simply unpower it. Nevertheless such attacks affect availability and not the correctness.


%The CSP is incentivized to prevent DoS attacks due to the revenue loss when the FPGA instance is unavailable. %We do not consider attacks against the CSP, as the Shell already protects against malicious FPGA users. 


%We trust that the RDMA stack, along with the attestation kernel, are implemented and synthesized correctly, whereas the bitstream and the keys are distributed and flushed to the FPGAs securely using remote attestation.





%The \projecttitle{} architecture implements a  network stack, similarly to~\cite{erpc, rdma-scale}, but focuses on security leveraging SmartNICs---specifically, FPGA-based NICs~\cite{intel_smartnics, alveo_smartnics}. 




\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/trusted-nic-attestation_kernel.drawio.pdf}
    \caption{\trustedfpga{} attestation kernel overview (transmission path).}
    \label{fig:attestation_kernel}
\end{figure}    
\fi

%\pramod{we should not restrict ourselves to replication protocols.}

%\pramod{Minimalism and verifiable hardware interface should be a separate challenge.}

\subsection{Design Challenges and Key Ideas} \label{subsec:challenges} While designing \projecttitle{}, we overcome the following challenges:

%\projecttitle{} aims to offer high-performant and unified verifiable trusted networking that can apply to a wide range of distributed systems. 



%that complicate TEEs' adoption for trustworthy systems, introducing engineering and correctness challenges.
\myparagraph{\#1: Heterogeneous hardware} 

The host CPU-side TEEs in the cloud infrastructure are heterogeneous with different programmability~\cite{Baumann2014, scone, 10.1145/3079856.3080208, 10.1145/3460120.3485341, tsai2017graphene, Rkt-io} and security properties~\cite{10.1145/3600160.3600169, 7807249, 10.1007/978-3-031-16092-9_7} that complicate their adoption and also affect the system's correctness~\cite{10.1145/3460120.3485341}. For example, Intel SGX~\cite{cryptoeprint:2016:086} offers code confidentiality and attestation while ARM TrustZone~\cite{arm-realm} does not. Prior work {\em could} not address this heterogeneity challenge; almost all prior systems' implementations~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} require {\em homogeneous} {\tt x86} machines with SGX extensions of a specific version, which is rather unrealistic in modern distributed systems. 
An alternative approach is to {\em stitch heterogeneous TEEs together} to build trustworthy distributed systems, however, this tactic introduces significant overheads in two directions. First, due to significant engineering efforts, TEEs'  {programmability differences limit} their adoption as a widely accepted general approach for trustworthy systems. Secondly, TEE's fundamental heterogeneity in {security semantics} complicates the correctness of the derived system; system designers must carefully consider the derived system's security guarantees.

% The host CPU-side TEEs in the cloud infrastructure are heterogeneous with different programmability~\cite{Baumann2014, scone, 10.1145/3079856.3080208, 10.1145/3460120.3485341, tsai2017graphene, Rkt-io} and security properties~\cite{10.1145/3600160.3600169, 7807249, 10.1007/978-3-031-16092-9_7} that affect their adoption while also raising concerns about the system's correctness~\cite{10.1145/3460120.3485341}. As an example of this heterogeneity, Intel SGX~\cite{cryptoeprint:2016:086} offers code confidentiality and attestation, but ARM TrustZone~\cite{arm-realm} does not. Likewise, AMD-sev~\cite{amd-sev} and Intel TDX~\cite{intelTDX} offer OS-based programming interfaces, whereas Keystone~\cite{riscv-multizone} and SGX require specific SDKs~\cite{KeystoneSDK}. Prior work {\em could} not address this heterogeneity challenge; in fact, we found that almost all prior systems' implementations~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} require {\em homogeneous} {\tt x86} machines with SGX extensions of a specific version.

% The requirement of homogeneous TEEs is rather unrealistic in modern cloud environments, resulting in system designers being compelled to {\em stitch heterogeneous TEEs together} to build trustworthy distributed systems. Unfortunately, this tactic introduces significant overheads in two directions. First, due to significant engineering efforts, TEEs'  {programmability differences limit} their adoption as a widely accepted general approach for trustworthy systems. Secondly, TEE's fundamental heterogeneity in {security semantics} complicates the correctness of the derived system; system designers must carefully consider the derived system's security guarantees.

\myparagraph{Key idea: A host CPU-agnostic unified security architecture based on trustworthy network-level isolation} Our \projecttitle{} offers a unified and host-agnostic network-interface level isolation that guarantees the specific and well-defined security properties of the non-equivocation and the transferable authentication. At the same time, we resolve the programmability burden through generic programming APIs. We build our \projecttitle{} system on SmartNIC hardware to achieve those goals, offering network-level isolation for our offered security properties. Importantly, our host-agnostic \projecttitle{} network interface is highly favorable in the heterogeneous Byzantine cloud infrastructure. In contrast, \projecttitle{}'s security properties of the non-equivocation and the transferable authentication have been proven to be sufficient for {\em correctly} transforming a wide variety of distributed systems for Byzantine settings. In fact, we show the power of \projecttitle{} with a generic transformation {\em recipe} ($\S$~\ref{subsec:transformation}) as well as its application to transform four widely adopted distributed systems ($\S$~\ref{sec:use_cases}).

%. To show the generality and applicability of our approach suffices to transform a wide variety of systems for Byzantine settings rending \projecttitle{} highly fa

%We offer a trusted unified programming interface that exposes the generic, yet powerful, security properties of the non-equivocation and transferable authentication. The properties, implemented at NIC-hardware level within the \projecttitle{}'s attestation kernel, suffice to transform distributed systems for Byzantine settings ($\S$~\ref{sec:background}). Our ; we offer BFT guarantees without relying on the host-sided TEEs. 

\if 0
\begin{itemize}
    \item {\bf Programmability:}

    \item {\bf Security:}
\end{itemize}

Our proposal: A unified host-agnostic trustworthy network-level isolation based on NICs
\fi 


\myparagraph{\#2: Large TCB in the TEE-based silicon root of trust} Prior works~\cite{avocado, minBFT, hybster, 10.1145/3492321.3519568} have established the {\em silicon root of trust}, e.g., TEEs, to be a promising direction to build trustworthy systems. Unfortunately, even the state-of-the-art TEEs integrate a {\em large} TCB. For example, we calculated the TCB size of the state-of-the-art Intel TDX~\cite{intelTDX}. The TEE ports within the trusted hardware the entire Linux kernel (specifically, v5.19~\cite{linuxlifecircle}) and ``hardens'' at least 2K lines of usable code, leading to a final TCB of 19MB. Such large TCBs have been accused of increasing the area of faults and attacks~\cite{10.1145/3379469, 10.5555/1756748.1756832} of commercial TEEs that are already under fire for their {major security vulnerabilities}~\cite{intel_sgx_vulnerabilities1, intel_sgx_vulnerabilities2, intel_sgx_vulnerabilities3, intel_sgx_vulnerabilities4, intel_sgx_vulnerabilities5}. As such, modern TEEs suffer from security flaws, whereas their large TCBs complicate their {security analysis and formal verification}, rendering the derived ``trustworthy'' distributed system {\em incoherent}. 


\myparagraph{Key idea: A minimal and formally verifiable silicon root-of-trust with low TCB} In our work, we advocate that a {\em minimalistic silicon root of trust} (TCB) at the NIC level hardware is the foundation for building verifiable, trustworthy distributed systems. In fact, \projecttitle{} builds a minimalistic and verifiable attestation kernel (TCB) at the SmartNIC hardware that guarantees the non-equivocation and the transferable authentication properties for the network messages. Moreover, since we rely on a minimalistic interface for trusted computing, we have formally verified the \projecttitle{} secure hardware protocols in the Tamarin theorem prover ($\S$~\ref{subsec::formal_verification_remote_attestation}).

%that have already been proven to be the lower bound for transforming distributed systems to BFT ones~\cite{clement2012}. As such, our \projecttitle{} offers strong foundations to system designers without relying on the TEEs' extended TCB's with lot's of unnecessary features.


%In fact, state-of-the-art TEEs are still under fire for major security vulnerabilities~\cite{intel_sgx_vulnerabilities1, intel_sgx_vulnerabilities2, intel_sgx_vulnerabilities3, intel_sgx_vulnerabilities4, intel_sgx_vulnerabilities5}. As an example of this, we calculated the TCB size of the state-of-the-art Intel TDX~\cite{intelTDX}. The TEE ports within the trusted hardware the entire Linux kernel (specifically, v5.19~\cite{linuxlifecircle}) and ``hardens'' at least 2K lines of usable code, leading to a final TCB of 19MB. Safety in BFT systems has always been a challenge---e.g., Zyzzyva~\cite{unsafe_Zyzzyva} has proven to be unsafe almost ten years after its original publication---let alone when the {\em supposed} BFT system relies on ``unstable'' TEEs. 


%With the performance being critical in all of them, offering security with TEEs is a poor design choice due to their performance limitations. 
\myparagraph{\#3: Performance} Distributed systems in the third-party cloud infrastructure must be fast and trustworthy. Their overheads are significantly exacerbated in the context of networked systems~\cite{avocado, treaty, minBFT,10.1145/3492321.3519568}--- the foundational building block in the core of any distributed system. Prior research~\cite{avocado} have reported an average of 4$\times$---8$\times$ performance degradation for networking between two host-sided TEEs instances (Intel SGX) even with using a sophisticated network stack implementation that had carefully been optimized for this specific TEE version. Other systems on top of TEEs~\cite{10.1145/3492321.3519568, hybster, minBFT} also can limit performance due to the communication costs between the untrusted and TEE-based counterparts of the system~\cite{10.1145/2168836.2168866}. Based on performance analysis of heterogeneous TEEs~\cite{9460547, 9935045}, the actual performance overheads of a distributed system in the heterogeneous cloud can be even more exacerbated. As such host-sided trusted hardware cannot {\em naturally} offer high-performant trusted networking. 

\myparagraph{Key idea: Hardware-accelerated trustworthy network stack} Our \projecttitle{} bridges the gap between performance and security with two design insights. First \projecttitle{} minimalistic TCB, the attestation kernel, offers the foundations to transform CFT distributed systems to BFT distributed systems without affecting the number of participating machines. This is especially important in the context of replication protocol as the transformation significantly improves scalability; we can have BFT with the same number of participating nodes as in the CFT system. Secondly, we offer a user-space network stack that bypasses the OS while we build our attestation kernel at the NIC-level hardware---specifically, on SmartNICs---offloading at the hardware the security processing of the non-equivocation and transferable authentication. 

%We implement a minimal TCB, the attestation kernel ($\S$~\ref{subsec:nic_attest_kernel}), that materializes all the necessary properties for transforming systems for Byzantine settings. We build the attestation kernel as part of the state-of-the-art NIC hardware for high performance ($\S$~\ref{subsec:roce_protocol_kernel}). Our evaluation shows that \projecttitle{}, applied in four widely-adopted systems, outperforms the TEE-based versions of that systems ($\S$~\ref{sec:eval}).

\if 0
\myparagraph{Challenge \#1: Heterogeneity and Programmability} Prior trustworthy systems were built on top of CPU-specific TEEs. Importantly, we found that almost all of the open-source systems' implementations~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} require {\em homogeneous} {\tt x86} machines with SGX extensions of a specific version.

The requirement for homogeneous TEEs is not realistic in modern cloud environments as the cloud data centers are comprised by heterogeneous machines and continuously update their hardware infrastructure~\cite{}. Following this, system developers are compelled to {\em stitch together} heterogeneous TEEs to build trustworthy systems. Unfortunately, this task is challenging in two aspects. First, it introduces a significant programmability overhead that limits TEEs' adoption as a general approach for trustworthy systems. Secondly, it raises concerns about the safety and the correctness of the designed system; heterogeneous TEEs come with different security properties which complicate the design and safety analysis of the derived system.


\myparagraph{Solution} To attack this challenge, \projecttitle{}'s key idea is unification. We offer a trusted unified programming interface that exposes the generic, yet powerful, security properties of non-equivocation and transferable authentication. The properties, implemented at NIC-hardware level within the \projecttitle{}'s attestation kernel, suffice to transform distributed systems for Byzantine settings ($\S$~\ref{sec:background}). Our \projecttitle{}' approach is highly favorable in the heterogeneous Byzantine cloud infrastructure; we offer BFT guarantees without relying on the host-sided TEEs. In fact, we show the power of \projecttitle{} with a generic transformation {\em recipe} ($\S$~\ref{subsec:transformation}) as well as its application to transform four widely-adopted systems ($\S$~\ref{sec:use_cases}).
%onsequently, . In addition, our minimalistic hardware-assisted TCB allows us to fully verify the safety and security properties of our \projecttitle{} from its initialization and remote attestation process to its normal operation ($\S$~\ref{subsec::formal_verification_remote_attestation}).

\myparagraph{Challenge \#2: Minimalistic TCB} The state-of-the-art TEEs~\cite{amd-sev, intelTDX} integrate a huge TCB that vastly increases the area of faults and attacks. In fact, state-of-the-art TEEs are still under fire for major security vulnerabilities~\cite{intel_sgx_vulnerabilities1, intel_sgx_vulnerabilities2, intel_sgx_vulnerabilities3, intel_sgx_vulnerabilities4, intel_sgx_vulnerabilities5}. As an example of this, we calculated the TCB size of the state-of-the-art Intel TDX~\cite{intelTDX}. The TEE ports within the trusted hardware the entire Linux kernel (specifically, v5.19~\cite{linuxlifecircle}) and ``hardens'' at least 2K lines of usable code, leading to a final TCB of 19MB. Safety in BFT systems has always been a challenge---e.g., Zyzzyva~\cite{unsafe_Zyzzyva} has proven to be unsafe almost ten years after its original publication---let alone when the {\em supposed} BFT system relies on ``unstable'' TEEs. 

\myparagraph{Solution} In our work, we advocate that a {\em minimal TCB}, that materializes the {\em foundational security primitives}, is the key to building verifiable trustworthy distributed systems. In fact, our minimalistic attestation kernel implements the properties of non-equivocation and transferable authentication that have already been proven to be the lower bound for transforming distributed systems to BFT ones~\cite{clement2012}. As such, our \projecttitle{} offers strong foundations to system designers without relying on the TEEs' extended TCB's with lots of unnecessary features.

%To attack this challenge, \projecttitle{}'s key idea is minimalism. We design a minimalistic fully verifiable (TCB) attestation kernel at NIC-hardware level that exposes a unified API to system designers. As such, we offer BFT while removing the distributed system's dependencies on the host CPU, rendering our approach highly favorable in the heterogeneous cloud infrastructure. In addition, our minimalistic hardware-assisted TCB allows us to fully verify the safety and security properties of our \projecttitle{} from its initialization and remote attestation process to its normal operation ($\S$~\ref{subsec::formal_verification_remote_attestation}).

\myparagraph{Challenge \#3: Performance and security} Distributed systems in the third-party cloud infrastructure need to be fast and trustworthy. With the performance being critical in all of them, offering security with TEEs is a poor design choice due to their performance limitations. In addition to the examples in $\S$~\ref{subsec::tees}, we also acknowledge from experience the difficulty to optimise TEE-based programs even with using the state-of-the-art programming frameworks~\cite{scone}. For example, while porting a simple distributed client/server application into \textsc{scone}---an optimized framework that shields (unmodified) applications with Intel SGX---we found that increasing the (protected) swap memory (paging area), even unused, led to a performance degradation by a factor of two for the exact same unmodified application. Consequently, TEEs cannot {\em intuitively} offer performance and security.

%, the problem is even more exacerbated in fault-tolerant systems. Building replication protocols for distributed systems under the Byzantine fault model has always been a complex endeavor with performance, scalability, and engineering challenges~\cite{bftForSkeptics}. Even well-studied protocols, e.g., PBFT~\cite{Castro:2002}, are limited in scalability (it requires at least $f$ nodes w.r.t to its CFT counterpart), incur high latency (it runs three all-to-all broadcasting phases with $O(n^2)$ message complexity) and are hard to verify and optimize~\cite{10.1145/2658994}.

%\myparagraph{Challenge \#1: Performance vs. security} Distributed systems in the third-party cloud infrastructure need to be fast, scalable, and trustworthy. While performance is critical in all of them, with TEEs themselves introducing significant performance limitations, the problem is even more exacerbated in fault-tolerant systems. Building replication protocols for distributed systems under the Byzantine fault model has always been a complex endeavor with performance, scalability, and engineering challenges~\cite{bftForSkeptics}. Even well-studied protocols, e.g., PBFT~\cite{Castro:2002}, are limited in scalability (it requires at least $f$ nodes w.r.t to its CFT counterpart), incur high latency (it runs three all-to-all broadcasting phases with $O(n^2)$ message complexity) and are hard to verify and optimize~\cite{10.1145/2658994}.



\myparagraph{Solution} Our \projecttitle{} bridges this gap between performance and security. We implement a minimal TCB, the attestation kernel ($\S$~\ref{subsec:nic_attest_kernel}), that materializes all the necessary properties for transforming systems for Byzantine settings. We build the attestation kernel as part of the state-of-the-art NIC hardware for high performance ($\S$~\ref{subsec:roce_protocol_kernel}). Our evaluation shows that \projecttitle{}, applied in four widely-adopted systems, outperforms the TEE-based versions of those systems ($\S$~\ref{sec:eval}).

%protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%\myparagraph{Challenge \#1: Security vs high-performance} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

%\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.




  


\myparagraph{Challenge \#4: Hardware verifiability} Some (but not all) TEEs offer (remote) attestation so that the application owner can verify the integrity of the TEE and its executing code. To attest the system, the application code needs to be known to the TEEs' hardware provider (e.g., Intel Attestation Service~\cite{ias}) so that its functionality can be evaluated, {\em measured} before the trust is established. However, there are real-world application scenarios (e.g., proprietary algorithm~\cite{}) where the program itself need to comply with strict privacy policies and cannot be {\em openly} exposed to multiple parties. 

\myparagraph{Solution} Our \projecttitle{} overcomes the limitation. While its offered security properties are decoupled from the CPU running code, we further formally verify the safety and security guarantees of our system.

%\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

%\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


%\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}. Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


%\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 
\fi 

\if 0

\subsection{Design Challenges}
\dimitra{here}
\myparagraph{Challenge \#1: Security} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and, importantly, can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.


\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}. Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 
\fi


==> backups/design_requirements.tex <==
\section{Overview}
\dimitra{here}
\subsection{Design challenges for a trusted NIC}
\label{sec:requirements}
Our work is motivated by 
Our proposal for \projecttitle{} seeks to resolve the tension between security and performance for (distributed) applications in the modern cloud infrastructure, specifically targeting replication protocols\pramod{focus on building trusted distributed systems -- PLEASE DONT MAKE THIS PAPER a REPLICATION protocol paper.}. To this end, our goal is to help system designers to build efficient, fault-tolerant, and robust systems that remain correct even when the untrusted cloud infrastructure fails arbitrarily. 

To sum up, we target the following design properties: 
\begin{itemize}
    \item {\bf{Robustness}} for building and deploying fault-tolerant distributed protocols and applications that remain correct and available in the untrusted cloud infrastructure.
    \item {\bf{Performance and scalability}} for efficiently exchanging and authenticating network messages. Particularly, our \projecttitle{} allows for BFT with the minimum possible number of involved servers ($2f+1$), mitigating clients' costs and resource usage.
    \item {\bf{Adaptability}} for allowing protocol designers to build robust protocols that can seamlessly run in modern heterogeneous DCs without them having to be BFT experts. 
\end{itemize}


\myparagraph{Challenge \#1: Robustness} The distributed applications hosted in the third-party cloud infrastructure need to be highly available. As such, cloud services and applications build on top of replication protocols that offer fault tolerance and, importantly, can remain available when failures occur~\cite{Jimenez-Peris2001}. The vast majority of such deployed protocols in the cloud operate under the Crash Fault Tolerant model (CFT) where the machines can {\em only} fail by crashing or omitting some steps. However, the CFT model is inadequate in modern cloud infrastructure as it has been observed that the machines or other parts of the infrastructure can fail arbitrarily (i.e., exhibit Byzantine behavior~\cite{Lamport:1982}) due to malicious adversaries, compromised OS/hypervisor in machines, faulty network links and compromised memory and storage medium~\cite{Gunawi_bugs-in-the-cloud, ciad, fast-08-corruption, security-one-sided-communication, accountable-cloud}. Consequently, the current replication protocols target a quite limited fault model which does not match modern's applications security needs that are hosted in the (untrusted) cloud.

\myparagraph{Solution} Our \projecttitle{} overcomes this limitation by offering  trusted and easily adoptable network operations, which are at the core of any distributed protocol, to help system designers building more robust protocols. To achieve this, we build an extended implementation of the classical, widely-adopted, RDMA network stack~\cite{rdma} on programmable hardware, i.e., FPGA-based SmartNICs~\cite{u280_smartnics}, offloading on this hardware the necessary required security processing and mechanisms. 

%More importantly, conventional BFT protocols present the following characteristics. First, they require an extra set of $f$ participant machines to tolerate up to $f$ failures. Compared to CFT protocols that operate with $2f+1$ participants, classical BFT protocols present limited scalability as they require at least $3f+1$ participants~\cite{BFT_THEORY}. In addition to this, BFT protocols can be slow as they usually run at least three phases of broadcasts~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} and incur high message complexity (e.g., $O(n^2)$). Lastly, BFT protocols are complex: they are hard to understand, let alone be optimised~\cite{10.1145/2658994}. Even intuitive algorithmic improvements to optimize for the common case or recovery can significantly affect other parts of the protocol (e.g., view-change in~\cite{10.1145/1658357.1658358}, normal case adds 2 extra phases in~\cite{DBLP:journals/corr/abs-1803-05069}) .% Consequently, they have seen little adoption in commercial cloud applications due to their limited scalability and performance.


\myparagraph{Challenge \#2: Performance and scalability} Researchers~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358} presented a range of robust replication protocols that remain correct when arbitrary failures occur targeting the BFT model~\cite{Lamport:1982}. Unfortunately, these BFT protocols have recognised little adoption because they cannot meet the performance requirements of deployed applications~\cite{bft-time-is-now}. In addition, the vast majority~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069} introduces resources overheads and limits scalability because it requires at least $3f+1$ machines to tolerate up to $f$ faults. That is, at least more $f$ machines compared to currently deployed CFT protocols. Consequently, BFT protocols are not well suited for performance in modern high-end distributed systems~\cite{bftForSkeptics}.

\myparagraph{Solution} We bridge the gap between performance, scalability and robustness. Our \projecttitle{} offers robustness by materialising the necessary foundations for building BFT protocols~\cite{clement2012} in programmable, yet fast, hardware, while it also improves performance and scalability by limiting the number of required participant machines to the minimum, i.e., $2f+1$. More specifically, \projecttitle{} implements the theoretical foundations of Clement et. al~\cite{clement2012} to translate a CFT protocol to a BFT protocol without having to increase the CFT protocol's replication degree. We explain this mechanism in $\S$~\ref{sec:background}.  %Their work has shown that a translation between any CFT protocol to a BFT protocol {\em always} exists if the security properties of the transferable authentication and the non-equivocation are guaranteed. We discuss the properties and the translation mechanism in$\S$~\ref{}. 

%\begin{itemize}
 %   \item {\bf{Transferable authentication.}} Potentially malicious nodes cannot impersonate other (honest) nodes. Essentially, any node can verify that a message is signed by the correct sender, even for forwarded messages.
 %   \item {\bf{Non-equivocation.}} A sender cannot send different messages to different nodes in the same round while it is supposed to send the same message according to the protocol.
%\end{itemize}

%we designed and implemented \projecttitle{} to offer the two properties of non-equivocation and transferable authentication that allow us to design and build BFT protocols with the minimum possible participant nodes ($2f+1$), resolving the trade-off of scalability, performance, and BFT at once. 

%More precisely, our design relies on the theoretical findings 

%Our \projecttitle{} materializes these properties on the NIC-level by implementing and integrating an attestation kernel for generating message authentication certificates or attestations and verifying those when messages are received ($\S$~\ref{subsec:tfpga}). That way \projecttitle{} builds and exposes the minimal abstraction required for implementing robust protocols under the Byzantine Fault model with $2f+1$ participant nodes.


\myparagraph{Challenge \#3: Adaptability} Due to the traditional BFT protocols limitations, a new line of research has attempted to optimize them~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, trinc} making use of trusted hardware, precisely, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}.  Unfortunately, the safety requirements of these optimized protocols highly depend on very specific and CPU-dependant TEEs. Consequently, in addition to their limit adaptability and generality, these protocols' correct implementation and deployment requires that there will {\em always} be available the required number of machines equipped with specific CPU generation and TEE hardware versions. In any other case, system designers are compelled to be able to quickly learn and program any another available TEE. This complicates the widespread adoption of such protocols because the task of programming heterogeneous TEEs as rather challenging~\cite{10.1145/3460120.3485341} as error prone; various TEEs present different programming models and security properties~\cite{10.1007/978-3-031-16092-9_7}. %To sum up, this heterogeneity complicates the widespread adoption of such protocols.
%it raises questions regarding performance and correctness. 

%---in fact, we found that all such open-sourced protocols~\cite{hybster, 10.1145/3492321.3519568, minBFT, DBLP:journals/corr/LiuLKA16a} are built on top Intel SGX~\cite{intel-sgx}.

%We argue that the protocols' reliance on such specific TEEs limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to deploy these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU generation and TEE hardware versions. In cases where there are no machines available, or the TEE has been discontinued (e.g., this is the case with Intel SGX~\cite{sgx_deprecated}), protocol designers are compelled to be able to quickly learn and program another available TEE. However, programming heterogeneous TEEs is a task rather challenging~\cite{10.1145/3460120.3485341}, and it raises questions regarding performance and correctness. Heterogeneous TEEs not only have different programming and performance characteristics but the security properties they offer can greatly vary too~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB), only up to 256MB, compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. 
%\antonis{may mention arm as well?}
%Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness, and confidentiality), whereas not all of them come with built-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}. All these characteristics make the widespread adoption of existing BFT protocols impractical.


\myparagraph{Solution} We attack this challenge by removing any dependencies on CPU-based TEEs and unshackling the designers from having to continuously learn and program various TEEs. Our \projecttitle{} makes use of programmable hardware, i.e., FPGAs, to implement a trusted network stack offloading any security-related processing in the NIC hardware ($\S$~\ref{subsec:tfpga}) and to offer a unified abstraction (network library) to the system designers ($\S$~\ref{sec:net-lib}). While our \projecttitle{} shifts the homogeneity from the CPU layer to the FPGA-based NIC layer, our architectural design is not hypothetical; \projecttitle{} fits well in recent deployments in commercial clouds, e.g. Microsoft's Catapult design~\cite{msr_smartnics, 211249}. 

%machines. To achieve this, we implement our entire network stack, including the trusted subsystem for non-equivocation and authentication, on the NIC's hardware-level, leveraging the SmartNIC technology~\cite{}. Essentially, our \projecttitle{} shifts the homogeneity from the CPU layer to the NIC layer:  while the host CPUs participating in a protocol can be heterogeneous, our \projecttitle{} is built on top of homogeneous SmartNICs \antonis{seems stricter than what we assume? maybe FPGA-enabled networking?}, exposing a unified abstraction for exchanging and verifying network messages.

%We implemented our network stack on top of FPGA-based SmartNICs, specifically Alveo U280~\cite{alveo_smartnics}. While our design could be adapted to be applicable to  SoC-based SmartNICs (e.g., Mellanox BlueField~\cite{bluefield_smartnics}, Alveo SN1000~\cite{alveo_sn1000}), we decided against it due to their performance limitations in 100G era~\cite{211249}.\antonis{weak argument, Bluefield 3 is up to 400Gbits. Let's say: "Our design is applicable to ... and our evaluation shows that hardware implementation is more beneficial.} Instead, given the increasingly wide deployment of such specialized hardware in DCs as an efficient way to offload network processing our architectural design is not hypothetical. \projecttitle{} fits well in recent deployments in commercial clouds. An example of this is Microsoft’s Catapult, where the FPGA, which sits on the data path in front of the network card and applies ``smart'' processing, could be extended (as in $\S$~\ref{subsec:tfpga}) to improve security.

%Our system achieves these goals by implementing a minimal hardware-based authentication subsystem, the \emph{attestation kernel}, that guarantees the necessary security properties required for BFT. The attestation kernel generates and verifies authentication certificates for the network messages to ensure two core security properties: the non-equivocation and the (transferable) authentication properties. These two properties have been proven to be necessary and sufficient for decreasing the replication factor for BFT protocols~\cite{clement2012}. Further, we carefully implemented \projecttitle{} to optimize for performance and scalability by integrating the attestation kernel ``on path'' at the NIC-level. That way, our system offers security without introducing unnecessary overheads both in performance and adoption: data is processed \emph{on their way} to the network whereas the protocols do not have to rely on a specific TEE in the host CPU layer. 

\section{Overview}
To this end we propose \projecttitle{}, a trusted NIC architecture that fullfils the afforementioned design goals. Figure~\ref{fig:overview} shows our \projecttitle{} system design. The system is comprised of three layers: (1) the application layer that runs the (distributed) protocol code (We show four uses cases of \projecttitle{} application in $\S$~\ref{sec:use_cases}), (2) the \projecttitle{} software library which exposes the \projecttitle{} API ($\S$~\ref{sec:net-lib}) and (3) the \projecttitle{} hardware implementation on top of FPGA devices ($\S$~\ref{sec:t-nic-hardware}). Each machine comprises a (host) CPU to which it is attached a \projecttitle{} through the PCIe~\cite{pcie}. The \projecttitle{} devices are connected through direct (Ethernet) links or a switch. %a $X$Gbps Ethernet switch through its QSFP port 0.

The  \projecttitle{} software library implements the programming framework and the \projecttitle{} device access interface. The programming framework exposes a user-space network library for trusted one-sided RDMA (reliable) operations. In addition, we expose a memory management API for correctly initializing and registering the registered-to-the-NIC memory. The software part of our \projecttitle{} also includes a driver that inserts a kernel module to set up the device with the static configuration (MAC address, IP, etc.) and further allocates and maps a specific (host) memory area to the device. While the driver runs only once at the initialization, the mapped memory is used to pass down to the device requests and any related parameters. 


The hardware implementation of \projecttitle{} runs the RDMA protocol on top of FPGA-based SmartNIC hardware. We further extend the network protocol kernel with a minimal hardware security module, the attestation kernel which shields and verifies the network traffic across the participant nodes. Specifically, the security module  constructs a secure message format that is verifiable and the network stack module implements the RDMA network protocol. In contrast to the control and configuration paths shown in Figure~\ref{fig:overview}, the message to be sent, is fetched from the application's memory directly to the device through DMA transfers. The message, after being shielded, is then forwarded to the network stack module for transmission.  % to preserve the authentication and non-equivocation properties across all network operations.
%On top of our trusted network stack, we implement a networking library, \projectlibrary{}, that exposes the developers to the classical RDMA API enhanced with two security properties, i.e., the transferable authentication and the non-equivocation.


\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.5\textwidth]{figures/trusted-nic-overview.drawio.pdf}
    \includegraphics[width=0.5\textwidth]{figures/system_overview-2.pdf}
    \caption{\projecttitle{} system overview.}
    \label{fig:overview}
\end{figure}

==> backups/evaluation.tex <==
\section{Implementation and Evaluation}
\label{sec:eval}
\dimitra{EVALUATION PLAN TODO}
\subsection{Hardware evaluation}
\myparagraph{Research questions}
\begin{itemize}
    \item[1] What is the overall latency and throughput of the (single-node) Attestation kernel, i.e., the invocations of \texttt{Attest}/\texttt{Verify} functions (secure operations)?
    \item[2] Performance breakdown: how much does the PCI transfer and the secure operations cost w.r.t. the overall execution?
    \item[3] {\bf \color{red} BONUS:} What is the comparison of an Attestation kernel in the SGX vs SmartNics? 
\end{itemize}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.5\textwidth]{eval-plots/plots/rsa.pdf}
    \caption{Attestation kernel (transmission path) latency evaluation.}
    \label{fig:initialization}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.5\textwidth]{eval-plots/plots/sha.pdf}
    \caption{Attestation kernel (transmission path) latency evaluation.}
    \label{fig:initialization}
\end{figure}

\myparagraph{Current progress/planning}

{\color{blue} 
\begin{itemize}
    \item[1]  {\bf{SKETCH:}} @Robert has (almost) implemented the functions, and we have both discussed and sketched the code for the benchmarking. \\{\bf STATUS: on-track}
    \item[2]  {\bf{SKETCH:}} To measure the PCI transfers we execute the benchmark, calling into the device/FPGA executing an empty kernel.\\{\bf STATUS: on-track}.
    \item[3] \color{red} {\bf{SKETCH:}} A stand-alone running SGX process that receives and sends localhost requests for attest and verify.\\ {\bf STATUS: optional}. 
\end{itemize}
}

\subsection{Benchmark \#2: \projecttitle{}}
\begin{itemize}
    \item[1] What is the overall latency and throughput of a native SmartNic-based \texttt{send}/\texttt{recv} operations w.r.t. state-of-the-art networking, RDMA/DPDK (e.g., eRPC)?
    \item[2] What is the overheads for BFT w.r.t. the native SmartNic-based \texttt{send}/\texttt{recv} operations?
    \item[3] {\bf \color{red} BONUS (optional for completeness)} Can we have two network stacks, i.e., openNIC and Coyote comparison?
\end{itemize}


\begin{center}
\begin{table}[ht]
\centering
\begin{tabular}{ |m{3cm}||m{2cm}|m{2cm}|}
 \hline
  & Tps (MB/s) & Latency (us) \\
  \hline
 native RDMA & 270 & 5  \\
 \projecttitle{} w/o rsa & 10.87 & 16 \\
 TEE-RDMA &  &  \\
 \projecttitle{} w/o rsa & 10.87 & 16 \\
 \projecttitle{} & 2.41 & 100 \\
 \hline
 \end{tabular}
\caption{\projecttitle{} throughput (Tps) and latency evalaution w.r.t. a native (untrusted) RDMA stack.}
\end{table}\label{res:net_stack}
\end{center}






\myparagraph{Current progress/planning}

{\color{blue} 
\begin{itemize}
    \item[1] {\bf SKETCH:} We compare a native port of a SmartNic-based network stack (openic or Coyote) with native RDMA/DPDK to measure latency, throughput (would be nice to also show scalability, in terms of network connections). 
    \\ {\bf STATUS: planned: Felix-openic (and dimitra-Coyote)}.
\end{itemize}
}


\subsection{Benchmark \#3: Use cases}
\begin{itemize}
    \item[1] What is the overheads of BFT (transformed) protocols w.r.t. to their native versions?
\end{itemize}
{\color{blue} 
\begin{itemize}
    \item[1] {\bf SKETCH:} We compare a native implementations of 3 Crash-Fault-Tolerant protocols with their BFT versions. The code runs with eRPC (native RDMA/DPDK) where we mock the latency of the attestation kernel.
    \\ {\bf STATUS: native protocols done --- BFT protocols design/implementation in progress}.
\end{itemize}
}

==> backups/evaluation_apps.bak.tex <==
\subsection{Distributed Applications Evaluation}
\label{subsec:use_cases_eval}

\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
 \hline
 System & $N$ & $f$ ($N=3$) & Byz. faults \\ [0.5ex] \hline \hline
 A2M    & 1 & 0 & Prevention\\
 BFT &  $2f+1$ & $f=1$ & Prevention\\
 Chain Replication &  $2f+1$ & $f=1$ & Prevention\\
 PeerReview & $f+1$ & $f=2$ & Detection\\
 \hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{Properties of the four systems implemented with \projecttitle{}.}
\label{tab:use_cases_options}
%\vspace{-18pt}
\end{table}
We implement the four systems of $\S~\ref{sec:use_cases}$ with \projecttitle{}. Table~\ref{tab:use_cases_options} summarizes the systems' properties where $N$ refers to the number of machines used for the protocol, and $f$ is the number of failures the system can tolerate.

\myparagraph{Methodology and experiments} We execute all four of our codebases on Cluster 2, utilizing its three servers, which form the minimum required setup capable of withstanding a single failure ($N=2f+1$, where $f=1$). Furthermore, due to our limited resources, with only two Alveo U280 cards available and the physical separation of Cluster 2 from Cluster 1, we were unable to access Alveo U280 cards for these specific experiments. Instead, we compiled our code using the D-I/O network stack as previously detailed in $\S$~\ref{subsec:net_lib}. We replicate these delays within the CPU to emulate latency delays for generating and verifying attested messages in the \projecttitle{} system. Our code uses busy waiting to accurately emulate latency rather than sleep functions. 

We evaluate each protocol using five systems that generate and verify the attestations: {\em (i)} the Nat-lib a library that is integrated into the codebase (no tamper-proof), {\em (ii)} the Nat, the OpenSSL-based server where we run one server instance in each protocol node (no tamper-proof), {\em (iii)} SGX and {\em (iv)} AMD-sev, and {\em (v)} \projecttitle{} which are all an integrated library (Nat-lib) to the codebase and further adds a configurable delay to represent the operation's latency in each system. The added delay for each system is the respective latency we measured in $\S$~\ref{subsec:hw_eval}.

Given that the D-I/O for small messages operates roughly three times the speed of the hardware-based RDMA network stack implementation, the latencies outlined in this section for \projecttitle{} are anticipated to reflect the upper limit.

\myparagraph{\projecttitle{}-log} We implement a prototype of A2M system, \projecttitle{}-log, an effective building block for reducing the replication factor and improving performance in various BFT systems~\cite{A2M, sundr, Castro:2002, AbdElMalek2005FaultscalableBF}. Similarly to the original implementation of the system, our SGX-based implementation ports the entire log within the TEE. All other versions place the attested log in the (untrusted) host memory, using the implemented systems to generate attested entries as  in~\cite{levin2009trinc}. \atsushi{Does this paragraph repeat explanations in s7.1? If so, like the following applications, can we simply say "We evaluate the A2M system (TNIC-log described in $\S$~\ref{sec:use_cases::a2m})..."?}

In this experiment, we first append 100M entries in the log and sequentially lookup for them individually. Each entry is comprised of the appended data (context)---in our case, 64B---and an extra 36B for the metadata, specifically the computed authenticate (32B) and the sequence number of the entry (4B). In short, we append 100M of 100B entries, leading to a log size of approximately 9GB. \atsushi{Can we somehow shorten the description?}

\noindent{\underline{Results.}} Figure~\ref{fig:a2m_eval} shows the throughput---measured in operations per second---and the average (mean) latency in microseconds of our implemented \projecttitle{}-log system using various system configurations. The append operation throughput in the Nat-lib case illustrates the maximum bound. Specifically, the operation running natively in the CPU reports a latency of 1.26us, which is dominated by the HMAC computation latency.
Placing the log within the SGX, we avoid costly communication, and as such, the system only experiences a 2$\times$ slowdown compared to the native case. On the other hand, we are using the AMD-sev as the trusted subsystem, which incurs 15$\times$ overheads compared to when porting the log within the SGX \antonis{Why?}. Lastly for \projecttitle{}, we observe approximately 5$\times$ and 2.4$\times$ slowdown compared to the native and SGX execution, respectively. The slowdown is primarily due to the HMAC calculation.

Regarding the lookup operation, all of the Nat-lib, AMD-sev and \projecttitle{} systems report similar throughput and latency as the operation lookups the untrusted host memory for the requested entry. However, the SGX-lib system reports a 66$\times$ slowdown for lookups due to its trusted memory size constraints and the effects of the Intel SGX paging mechanism~\cite{treaty}.



\begin{figure}[t!]
\begin{center}
\minipage{0.22\textwidth}
  \centering
\begin{tabular}{lrr}
\hline
& \multicolumn{2}{c}{Throughput (Op/s)} \\
System          & append    & lookup  \\
\hline
Nat-lib         & 790K      & 256M      \\
SGX-lib             & 380K      & 3.8M       \\
AMD-sev         & 30K       & 263M      \\
\projecttitle{} & 158K      & 257M      \\
\end{tabular}
\endminipage
\hfill
\minipage{0.18\textwidth}
\centering
\begin{tabular}{rrr}
\hline
\multicolumn{2}{c}{Latency (us)} \\
 append     & lookup  \\
\hline
 1.26       & 0.0039      \\
 2.6        & 0.26       \\
 32.37      & 0.0038      \\
 6.34       & 0.0039      \\
 
\end{tabular}
\endminipage
\end{center}
\caption{Performance evaluation of \projecttitle{}-log using various trusted components.}%\dimitra{@experiments: maybe you try run A2M into an SGX server to also show the communication costs}}
\label{fig:a2m_eval}
\end{figure}

\myparagraph{Byzantine SMR} 
We evaluate the performance of our implemented Byzantine SMR protocol (discussed in $\S$~\ref{sec:use_cases::byz_smr}) with various network batching factors. Network batching is a standardized optimization; we implement it in software as part of the application's message format. 
% We evaluate the performance of our implemented Byzantine SMR protocol (discussed in $\S$~\ref{sec:use_cases::byz_smr}) using various trusted components and network batching factors. Network batching is a standardized optimization; we implement it in software as part of the application's message format. 

We allocate one {\em message} structure for each client's request in this experiment. The {\em message} contains command and output fields (16B each), which store the initial command and results of the command's execution in a node, respectively. In addition, the message contains metadata, which includes a sequencer and signed hashes of the replicas' states known to each node. The sequencer is used for serialization, and it is equivalent to the counter value assigned to each message from \projecttitle{}. The signed hashes representing the replicas' states are obtained from the last messages received from each replica.

\noindent{\underline{Results.}} Figures~\ref{fig:byz_smr_throuthput} and~\ref{fig:byz_smr_lat} show the throughput and the latency of the implemented protocol. Our \projecttitle{} incurs about 2.4$\times$ overheads compared to the Nat-lib version. Similarly, SGX and AMD-sev versions incur 13.5$\times$ and 9.6$\times$ overheads compared to the Nat-lib. As such, leveraging the TEEs can be 4---6$\times$ less performant our \projecttitle{}. Recall that the Nat-lib version is the upper bound in performance we can possibly achieve as it calculates the attestations natively and does not incur the communication overheads that a realistic solution (SGX, AMD-sev) would occur. Nat-lib is not tamper-proof \atsushi{Can we highlight that TNIC is temper-proof but the Nat-lib (best perf) is not?}.
\antonis{Are the differences/benefits of TEE vs. TFPGA tamper-proofness discussed earlier than the evaluation? Seems its something important.}


Secondly, we observe that batching can increase throughput (and decrease the latency) proportionally to the number of batched messages. Specifically, for all but the Nat-lib version, we report a 7$\times$ and 15$\times$ throughput boost for 8 and 16 batching factor compared with the experiment run with batching factor equal to 1. This is because our batching technique improves the network utilization and reduces the overall attestation calculations, e.g., one per 8 and 16 messages. The technique is moderately effective when using the Nat-lib, approximately 4---6$\times$ faster than without batching. This is primarily because, in that case, the latency is dominated by the network stack latency as the attestation function running natively generates attestations fast. As such, we show that conventional techniques can drastically eliminate the overheads for BFT and improve \projecttitle{}'s adoption into practical systems.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bft_pb.pdf} 
    \caption{Throughput of the BFT SMR using various trusted components.} \label{fig:byz_smr_throuthput}
\end{figure}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.7\linewidth]{atc-submission-plots/bft_pb_lat.pdf} 
%    \caption{Average latency of the BFT SMR using various trusted components.} \label{fig:byz_smr_lat}
%\end{figure}


\myparagraph{Byzantine Chain Replication} We evaluate the performance of the Byzantine Chain Replication protocol (discussed in $\S$~\ref{sec:use_cases::byz_chain_rep}). % using various trusted components. 
In this experiment, we do not employ batching, and we allocate one message structure as discussed in $\S$~\ref{sec:use_cases::byz_chain_rep} per client request. The context of the message allocates 60B comprised of an 8B key and a 32B value as well as 16B for metadata (e.g., source and destination nodes, message idx, etc.) and 4B for the operation type. As before, the HMAC adds 32B to the message. We implemented the replication protocol without any underlying Key-Value store data structure.

\noindent{\underline{Results.}} Figure~\ref{fig:byz_chain_replication} shows the throughput and average mean latency of Byzantine Chain replication using various trusted components. Concerning the Nat-lib implementation, \projecttitle{} incurs 4.6$\times$ overhead. In addition, in the Nat version, where the OpenSSL server incurs the communication costs with the protocol process, we see 5.8$\times$ overhead. Our \projecttitle{} is 1.2$\times$ faster compared to Nat execution; the performance benefit is primarily due to the on-the-data-path approach we follow.
Compared to the SGX and AMD-sev versions, Byzantine Chain Replication with \projecttitle{} is 5$\times$ and 3.4$\times$ faster.
\begin{figure}
    \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a Byzantine Chain Replication using various trusted components.} \label{fig:byz_chain_replication}
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of the accountability protocol using various trusted components.} \label{fig:accountability_protocol}
\end{figure}

\if 0
\begin{figure*}[t!]
\begin{center}
\minipage{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a Byzantine Chain Replication using various trusted components.} \label{fig:byz_chain_replication}
\endminipage
\minipage{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of the accountability protocol using various trusted components.} \label{fig:accountability_protocol}
\endminipage
\end{center}
\end{figure*}
\fi


\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a BFT version of CR using various trusted components.} \label{fig:lat_throughput_kernel}
\end{figure}
\fi






\myparagraph{Accountability protocol} We evaluate the performance of the Accountability protocol (discussed in $\S$~\ref{sec:use_cases::accountability}). % using various trusted components. 
We evaluate the protocol by both activating and deactivating the audit protocol. In our implementation, we use one witness for the source node that {\em periodically} audits its log. The witness process is co-located in the same node, and as such, reading the log implies reading a shared memory. We decide in favor of that implementation to carefully isolate the overheads for inspection and replay of the log. In our experiments, the witness is configured to audit the log after every send operation in the source node until both clients acknowledge the receipt of all source messages.

The log entries consist of the context, a sequencer, a signed hash of the context, and the sequencer (authenticator) \antonis{is this different than the aforementioned "sequencer"?} as well as the cumulative digest, which is the signed hash of the authenticator and the previous entry's digest in the log. The context is comprised of the data (16B), the output of the protocol specification for that input data (16B), some metadata, and the response sent from the clients that have a similar format. In total, the messages allocate about 200B, and we do not use batching. \atsushi{I feel that the description of these data formats (as well as the other applications) is too detailed, so it'll be fine to omit for cutting the text.}

\noindent{\underline{Results.}} Figure~\ref{fig:accountability_protocol} shows the throughput and latency measurements of the accountability protocol with the audit protocol (blue line) and without the audit protocol (green line).
\atsushi{a bit difficult to read because 'log' is used as both noun and verb. Can we somehow use another word?} When the protocol does not activate the witness process to audit the log, the source node sends the streaming data to the client nodes. The clients execute and log the message and then reply to the source. Then, the source logs its own message along with the client's reply. This is required to make sure that any participant cannot lie to a witness about the data it sends to the clients. \atsushi{The sentences until here explain the application workflow, but we should show the results first and then start the discussion with an extra explanation.} We see that using a TEE to generate attested messages increases the throughput slowdown up to 30$\times$ compared to the native embedded library (Nat-lib). Using our \projecttitle{} we improve the overheads---specifically, we incur 5.8$\times$ slowdown, that is 3---5$\times$ better throughput compared to when using AMD-sev and SGX as trusted messages' singers.

When we activate the audit protocol, we observe similar performance behavior as before. The \projecttitle{} outperforms both AMD-sev and SGX implementations by 3.7---5$\times$. Importantly, activating the witness in the source node, when using \projecttitle{}, leads to a performance slowdown of 1.33$\times$ compared to when not executing the witness. More specifically, the audit protocol consumes approximately 25\% (17us) of the overall execution latency. \atsushi{What's the takeaway from this experiment?}

\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a BFT version of PR using various trusted components.} \label{fig:lat_throughput_kernel}
\end{figure}
\fi

==> backups/evaluation_apps.bak2.tex <==
\subsection{Distributed Applications Evaluation}
\label{subsec:use_cases_eval}

\if 0
\begin{table}
\begin{center}
\small
\begin{tabular}{ |c|c|c|c| } 
 \hline
 System & $N$ & $f$ ($N=3$) & Byz. faults \\ [0.5ex] \hline \hline
 A2M    & 1 & 0 & Prevention\\
 BFT &  $2f+1$ & $f=1$ & Prevention\\
 Chain Replication &  $2f+1$ & $f=1$ & Prevention\\
 PeerReview & $f+1$ & $f=2$ & Detection\\
 \hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{Properties of the four systems implemented with \projecttitle{}.}
\label{tab:use_cases_options}
%\vspace{-18pt}
\end{table}
\fi
We implement the four systems of $\S~\ref{sec:use_cases}$ with \projecttitle{}. All systems run in three nodes ($N=3$) except for the A2M that is a single node system.
% the systems' properties where $N$ refers to the number of machines used for the protocol, and $f$ is the number of failures the system can tolerate.

\myparagraph{Methodology and experiments} We execute all four of our codebases on Intel Cluster, utilizing all its three servers (as the minimum required setup capable of withstanding a single failure, $N=2f+1$, where $f=1$). Furthermore, due to our limited resources, with only two Alveo U280 cards available and the physical separation of Intel Cluster from AMD-FPGA Cluster, we cannot access Alveo U280 cards for these specific experiments. Instead, we compiled our code using the DRCT-IO network stack as previously detailed in $\S$~\ref{subsec:net_lib} and do busy waiting to accurately replicate the \projecttitle{} delays within the CPU for generating and verifying attested messages.% in the \projecttitle{} system. %Our code uses busy waiting to accurately emulate latency rather than sleep functions. 

We evaluate each protocol using five systems that generate and verify the attestations: {\em (i)} the SSL-lib a library that is integrated into the codebase (no tamper-proof), {\em (ii)} the SSL-server (no tamper-proof), {\em (iii)} SGX and {\em (iv)} AMD-sev, and {\em (v)} \projecttitle{}. To perform a fair comparison we integrate into our protocols' codebases an library that accurately emulate all latencies (measured in $\S$~\ref{subsec:hw_eval}) within the CPU. We do not emulate the SSL-lib latency and for the AMD latency we use 30us which represents the lower bound of the latencies measured in $\S$~\ref{subsec:hw_eval}.

 %which are all an integrated library to the codebase and further adds a configurable delay to represent the operation's latency in each system. The added delay for each system is the respective latency we measured in

Given that the DRCT-I/O for small messages operates roughly three times the speed of the hardware-based RDMA network stack implementation, the latencies outlined in this section are anticipated to reflect the upper limit for all four systems with \projecttitle{}.

\myparagraph{A2M} We implement a prototype of A2M system with \projecttitle{}, an effective building block for imporving the scalability and performance in various systems~\cite{A2M, sundr, Castro:2002, AbdElMalek2005FaultscalableBF}. Similarly to its original implementation, we port the entire log within the TEE, i.e., SGX, building a large TCB. We refer to this system as SGX-lib. All other versions place the attested log in the (untrusted) host memory, using the trusted systems to generate attestations as in~\cite{levin2009trinc}. %\atsushi{Does this paragraph repeat explanations in s7.1? If so, like the following applications, can we simply say "We evaluate the A2M system (TNIC-log described in $\S$~\ref{sec:use_cases::a2m})..."?}

In this experiment, we first construct a log of size 9GB with 100M entries and then sequentially we lookup for them individually. Each log entry is comprised of 64B of appended data (context) and an extra 36B for the metadata.

%specifically the computed authenticate (32B) and the sequence number of the entry (4B). In short, we append 100M of 100B entries, leading to a log size of approximately 9GB. \atsushi{Can we somehow shorten the description?}

\noindent{\underline{Results.}} Figure~\ref{fig:a2m_eval} shows the throughput (operations per second) and the average (mean) latency of our implemented A2M system using various systems. The append operation throughput in the SSL-lib case illustrates the throughput upper bound as it incurs no communication costs. Specifically, the A2M with SSL-lib running natively in the CPU reports a latency of 1.26us, which is dominated by the HMAC computation latency.
Placing the log within the SGX (SSL-lib), we avoid the costly communication w.r.t. to an SGX-based server implementation, and as such, the system only experiences a 2$\times$ slowdown compared to the native case. The communications costs are reflected in the AMD-sev case; that runs the SSL-server. Compared to when porting to SGX, AMD-sev incurs 15$\times$. Lastly for \projecttitle{}, we observe approximately 5$\times$ and 2.4$\times$ slowdown compared to the SSL-lib and SGX-lib execution, respectively which is due to the HMAC calculation.

Regarding the lookup operation, all of the SSL-lib, AMD-sev and \projecttitle{} systems report similar throughput and latency as the operation lookups the untrusted host memory for the requested entry. However, the SGX-lib system reports a 66$\times$ slowdown for lookups due to its trusted memory size constraints and the effects of the Intel SGX paging mechanism~\cite{treaty}. As a result, while \projecttitle{} offers slower append operations compared to when porting the entire log into the TEE, \projecttitle{} greatly optimizes lookup latencies due to its minimal TCB.



\begin{figure}[t!]
\begin{center}
\small
\minipage{0.22\textwidth}
  \centering
\begin{tabular}{lrr}
\hline
& \multicolumn{2}{c}{Throughput (Op/s)} \\
System          & append    & lookup  \\
\hline
SSL-lib         & 790K      & 256M      \\
SGX-lib             & 380K      & 3.8M       \\
AMD-sev         & 30K       & 263M      \\
\projecttitle{} & 158K      & 257M      \\
\hline
\end{tabular}
\endminipage
\hfill
\minipage{0.18\textwidth}
\centering
\begin{tabular}{rrr}
\hline
\multicolumn{2}{c}{Latency (us)} \\
 append     & lookup  \\
\hline
 1.26       & 0.0039      \\
 2.6        & 0.26       \\
 32.37      & 0.0038      \\
 6.34       & 0.0039      \\
 \hline
\end{tabular}
\endminipage
\end{center}
\caption{Throughput and latency evaluation of A2M using various trusted components.}%\dimitra{@experiments: maybe you try run A2M into an SGX server to also show the communication costs}}
\label{fig:a2m_eval}
\end{figure}

\myparagraph{BFT} We evaluate the performance of our implemented BFT protocol (discussed in $\S$~\ref{sec:use_cases::byz_smr}) with various network batching factors. Network batching is a standardized optimization; we implement it in software as part of the application's message format. 
% We evaluate the performance of our implemented Byzantine SMR protocol (discussed in $\S$~\ref{sec:use_cases::byz_smr}) using various trusted components and network batching factors. Network batching is a standardized optimization; we implement it in software as part of the application's message format. 

We allocate one {\em message} structure for each client's request in this experiment. The {\em message} contains command and output fields (16B each), which store the initial command and results of the command's execution in a node, respectively. In addition, the message contains metadata, which includes a sequencer and signed hashes of the replicas' states known to each node. The sequencer is used for serialization, and it is equivalent to the counter value assigned to each message from \projecttitle{}. The signed hashes representing the replicas' states are obtained from the last messages received from each replica.

\noindent{\underline{Results.}} Figure~\ref{fig:byz_smr_throuthput} show the throughput and the latency of the protocol. Our \projecttitle{} incurs about 2.4$\times$ throughput overhead and up to 7$\times$ higher latency compared to the SSL-lib version. Similarly, SGX and AMD-sev versions incur 13.5$\times$ and 9.6$\times$ throughput overheads compared to the SSL-lib. As such, our \projecttitle{} improves throughput and latency 4---6$\times$ compared to TEE-based versions. Recall that the SSL-lib version is the upper bound in performance we can possibly achieve as it calculates the attestations natively and eliminates the communication overheads that a realistic solution (SGX, AMD-sev) occurs. However, in contrast to our \projecttitle{}, SSL-lib is not tamper-proof (Table~\ref{tab:hw_options}) as the security-related processing runs in the untrusted host CPU and can be accessed and compromised by malicious adversaries.

%\atsushi{Can we highlight that TNIC is temper-proof but the Nat-lib (best perf) is not?}.
%\antonis{Are the differences/benefits of TEE vs. TFPGA tamper-proofness discussed earlier than the evaluation? Seems its something important.}


In addition, we observe that batching increases throughput (and decreases latency) proportionally to the number of batched messages. For all but the SSL-lib version, we report a 7$\times$ and 15$\times$ throughput boost for batching factor to be equal to 8 and 16 respectively compared with the experiment run with batching factor equal to 1. This is because our batching technique improves the network utilization and reduces the overall attestation calculations, e.g., one attestation per 8 and 16 messages. The technique is moderately effective when using the SSL-lib, approximately 4---6$\times$ faster than without batching. This is primarily because, in that case, the latency is dominated by the network stack latency as the attestation function running natively generates attestations fast. As such, we show that conventional techniques can drastically eliminate the overheads for BFT and improve \projecttitle{}'s adoption into practical systems.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bft_pb.pdf} 
    \caption{Throughput (and latency numbers) of BFT using various trusted components.} \label{fig:byz_smr_throuthput}
\end{figure}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.7\linewidth]{atc-submission-plots/bft_pb_lat.pdf} 
%    \caption{Average latency of the BFT SMR using various trusted components.} \label{fig:byz_smr_lat}
%\end{figure}


\myparagraph{Chain Replication} We evaluate the performance of the Chain Replication protocol (discussed in $\S$~\ref{sec:use_cases::byz_chain_rep}) without bactching. % using various trusted components. 
We allocate one message structure per client request comprising of 60B context (that includes metadata, e.g., source, destination nodes, message id, etc.) and  4B for the operation type. As before, the 32B attestation  adds to the message. %We implemented the replication protocol without any underlying Key-Value store data structure.
%of the message allocates 60B comprised of an 8B key and a 32B value as well as 16B for metadata (e.g., source and destination nodes, message idx, etc.) and

\noindent{\underline{Results.}} Figure~\ref{fig:byz_chain_replication} shows the throughput and average mean latency of our implemented Chain Replication with various trusted components. Compared with the SSL-lib implementation, \projecttitle{} incurs 4.6$\times$ overhead and SSL-server incurs 5.8$\times$ overhead. Our trusted \projecttitle{} is 30\% faster compared to an non-tamper-proof (native) SSL-server. The performance benefit stems primarily from the \projecttitle{}'s attestation kernel being on the transmission/reception data path.
Compared to the SGX and AMD-sev versions, Byzantine Chain Replication with \projecttitle{} is 5$\times$ and 3.4$\times$ faster.
\begin{figure}
    \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput (and latency numbers) of Chain Replication using various trusted components.} \label{fig:byz_chain_replication}
\end{figure}

\begin{figure}
  \includegraphics[width=\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput (and latency numbers) of PeerReview using various trusted components.} \label{fig:accountability_protocol}
\end{figure}

\if 0
\begin{figure*}[t!]
\begin{center}
\minipage{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a Byzantine Chain Replication using various trusted components.} \label{fig:byz_chain_replication}
\endminipage
\minipage{0.5\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of the accountability protocol using various trusted components.} \label{fig:accountability_protocol}
\endminipage
\end{center}
\end{figure*}
\fi


\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bftcr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a BFT version of CR using various trusted components.} \label{fig:lat_throughput_kernel}
\end{figure}
\fi






\myparagraph{PeerReview} We evaluate the performance of our PeerReview system (discussed in $\S$~\ref{sec:use_cases::accountability}). % using various trusted components. 
We evaluate the protocol by both activating and deactivating the audit protocol. In our implementation, we use one witness for the source node that {\em periodically} audits its log. The witness process is co-located in the same node, and as such, reading the log implies reading a shared memory. We decide in favor of that implementation to carefully isolate the overheads for inspection and replay of the log. In our experiments, the witness is configured to audit the log after every send operation in the source node until both clients acknowledge the receipt of all source messages.

The log entries consist of the context, a sequencer, a signed hash of the context (authenticator) as well as the cumulative digest, which is the signed hash of the authenticator and the previous entry's digest in the log. In total, the messages allocate about 200B.% and we do not use batching. 
%\atsushi{I feel that the description of these data formats (as well as the other applications) is too detailed, so it'll be fine to omit for cutting the text.}

%The log entries consist of the context, a sequencer, a signed hash of the context, and the sequencer (authenticator) \antonis{is this different than the aforementioned "sequencer"?} as well as the cumulative digest, which is the signed hash of the authenticator and the previous entry's digest in the log. The context is comprised of the data (16B), the output of the protocol specification for that input data (16B), some metadata, and the response sent from the clients that have a similar format. In total, the messages allocate about 200B, and we do not use batching. \atsushi{I feel that the description of these data formats (as well as the other applications) is too detailed, so it'll be fine to omit for cutting the text.}

\noindent{\underline{Results.}} Figure~\ref{fig:accountability_protocol} shows the throughput and latency measurements of PeerReview system with and without enabling the audit protocol.
Without the audit protocol, the use of TEEs to generate attestations incurs a throughput slowdown up to 30$\times$ compared to the SSL-lib. Using our \projecttitle{} we improve the overheads---specifically, we incur 5.8$\times$ slowdown, that is 3---5$\times$ better throughput compared to when using AMD-sev and SGX.


When we activate the audit protocol, the systems behavior is similar. The \projecttitle{} outperforms both AMD-sev and SGX implementations by 3.7---5$\times$. Importantly, when using \projecttitle{}, the audit protocol leads to a performance slowdown of 1.33$\times$ compared to when not enabling it. The audit protocol itself consumes approximately 25\% (17us) of the overall execution latency. Even with the audit protocol, \projecttitle{} offers 3.7---5.42$\times$ lower latency compared to its TEEs-based competitors.

%\atsushi{a bit difficult to read because 'log' is used as both noun and verb. Can we somehow use another word?} When the auditing protocol is de-activated, the source node sends the (streaming) data to the client nodes. The clients execute and append the message to their log, and then reply to the source. The source appends its own message to the log along with the client's reply. This is required to make sure that any participant cannot lie to a witness about the data it sends to the clients. \atsushi{The sentences until here explain the application workflow, but we should show the results first and then start the discussion with an extra explanation.} We see that using a TEE to generate attested messages increases the throughput slowdown up to 30$\times$ compared to the native embedded library (Nat-lib). Using our \projecttitle{} we improve the overheads---specifically, we incur 5.8$\times$ slowdown, that is 3---5$\times$ better throughput compared to when using AMD-sev and SGX as trusted messages' singers.


\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/bftpr_lat_throughput.pdf} 
    \caption{Throughput-latency evaluation of a BFT version of PR using various trusted components.} \label{fig:lat_throughput_kernel}
\end{figure}
\fi


==> backups/evaluation_hw.bak2.tex <==
\section{Evaluation}
\label{sec:eval}
\myparagraph{Implementation}
We implement our prototype of \projecttitle{} extending the Coyote~\cite{coyote} codebase on top of Alveo U280~\cite{u280_smartnics}. We build the attestation kernel based on the HMAC module provided by Xilinx with the SHA-384 as the hashing algorithm~\cite{vitis-security-lib}. We wire the attestation kernel to the RoCE kernel input and output data cables (\texttt{axis\_rdma\_sink} and \texttt{axis\_host\_sink}) through 64B data paths (512-bit AXI4 Stream interfaces). The attestation kernel and the host memory communicate through an AXI4 memory-mapped Master. Lastly, the RoCE kernel is connected to a 32B bus width (parameters), a 20B bus width (requests opcodes), and a 12B bus width for local DMA operations. For the data transfers, \projecttitle{} builds on top of an XDMA IP~\cite{xdma, fpga_dma} that enables DMA over PCIe. The 100Gb MAC is implemented with a CMAC IP~\cite{license} that exposes two 512-bit AXI4-Stream interfaces to the RoCE protocol kernel for the transmitting (Tx) and receiving (Rx) network paths.

%Precisely, we extend the data path of Coyote, adopting the abstraction of {\em virtual} FPGA areas to plug in our attestation functionality. \projecttitle{} leverages the Coyote paradigm and wires the control domain and the data domain into different paths.


%The data flow from the host memory to the device memory using the Xilinx streaming protocol (i.e., \texttt{hls\_stream<>}) that divides data into 512-bit packets. 
%At the transmission path, we implemented and plugged in two FIFO queues that redirect the packets from the host memory to the device memory -- specifically into the HMAC module and the RoCE IP. The role of the first queue is to buffer data and calculate the HMAC of all packets of the transmission.
%The module is based on the HMAC module in the Xilinx Vitis Security Library using SHA-384 as the hash function~\cite{vitis-security-lib}.
%The data of the second queue is passed through to the RoCE IP until the last packet of the transmission is reached.
%When the HMAC has been calculated, the last packet of the transmission is replaced by the 384-bit HMAC padded to 512 bits.

%At the reception path, we also augment the stack with two queues.
%The first queue sends the data to the verification module that will calculate the {\em expected} HMAC for verification. If the verification process succeeds we reconstruct the received message and deliver it to the application layer (host memory). Otherwise, all corresponding packets are dropped which naturally affects liveness.

\if 0
\myparagraph{Implementation}
We implement \projecttitle{} extending Coyote~\cite{coyote} codebase. Precisely, we extend the data path of Coyote, adopting the abstraction of {\em virtual} FPGA areas to plug in our attestation functionality. \projecttitle{} leverages the Coyote paradigm and wires the control domain and the data domain into different paths.

The RoCE kernel input and output data cables, e.g., \texttt{axis\_rdma\_sink} and \texttt{axis\_host\_sink}, are connected through the Attestation kernel through 64B data paths (512-bit AXI4-Stream interfaces). Then, the attestation kernel and the host memory communication are achieved through an AXI4 memory-mapped Master interface using the Xilinx streaming protocol. It is the responsibility of the host code to allocate and initialize host memory. Further, the kernel is connected to a 32B bus to receive the parameters, a 20 B bus to issue RDMA write operations, and a 12 B bus to issue local DMA commands.

%The data flow from the host memory to the device memory using the Xilinx streaming protocol (i.e., \texttt{hls\_stream<>}) that divides data into 512-bit packets. 
At the transmission path, we implemented and plugged in two FIFO queues that redirect the packets from the host memory to the device memory -- specifically into the HMAC module and the RoCE IP. The role of the first queue is to buffer data and calculate the HMAC of all packets of the transmission.
The module is based on the HMAC module in the Xilinx Vitis Security Library using SHA-384 as the hash function~\cite{vitis-security-lib}.
The data of the second queue is passed through to the RoCE IP until the last packet of the transmission is reached.
When the HMAC has been calculated, the last packet of the transmission is replaced by the 384-bit HMAC padded to 512 bits.

At the reception path, we also augment the stack with two queues.
The first queue sends the data to the verification module that will calculate the {\em expected} HMAC for verification. If the verification process succeeds we reconstruct the received message and deliver it to the application layer (host memory). Otherwise, all corresponding packets are dropped which naturally affects liveness.
\fi 

\myparagraph{Evaluation setup}
We perform our experiments on a real hardware testbed using two clusters: AMD-FPGA Cluster and Intel Cluster. AMD-FPGA Cluster is equipped with two machines powered by AMD EPYC 7413 (24 cores, 1.5 GHz) and 251.74 GiB memory. Each machine also has two U280 Alveo cards~\cite{u280_smartnics} that are connected over a 100 Gbps interconnect. Intel Cluster is equipped with three machines powered by Intel(R) Core(TM) i9-9900K (8 cores, 3.2 GHz) with 64 GiB memory and three Intel Corporation Ethernet Controllers (XL710).

%, caches: 32 KiB (L1 data and code), 256 KiB (L2) and 16 MiB (L3). Cluster 2 nodes are connected over a 40GbE QSFP+ network switch.


%, caches: 32 KiB (L1 data and code), 512 KiB (L2) and 32 MiB (L3). Each machine also has two U280 Alveo cards~\cite{u280_smartnics} that are connected over a 100 Gbps cable.
%\atsushi{Can we simplify the above like this: Cluster 1 is equipped with two machines powered by AMD EPYC 7413 (24 cores, 1.5 GHz) and 251.74 GiB memory.}

%Cluster 2 is equipped with three machines with CPU (marked as CPU-2 in the respective plots): Intel(R) Core(TM) i9-9900K (8 cores, 3.2 GHz), memory: 64 GiB, caches: 32 KiB (L1 data and code), 256 KiB (L2) and 16 MiB (L3). Cluster 2 nodes are connected over a 40GbE QSFP+ network switch.
%\antonis{CPU-1 and CPU-2 are not memorable names, consider AMD, x86?} %\atsushi{I agree with Antonis. Also, can we rename Cluster 1 and 2 like this: AMD-FPGA Cluster and Intel Cluster?} \atsushi{Cluster 2 is equipped with three machines powered by Intel(R) Core(TM) i9-9900K (8 cores, 3.2 GHz) with 64GiB memory.}

%We perform our experiments on a real hardware testbed using two clusters: Cluster 1 and Cluster 2. Cluster 1 is equipped with two machines with CPU (marked as CPU-1 in the respective plots): AMD EPYC 7413 (24 cores, 1.5 GHz), memory: 251.74 GiB, caches: 32 KiB (L1 data and code), 512 KiB (L2) and 32 MiB (L3). Each machine also has two U280 Alveo cards~\cite{u280_smartnics} that are connected over a 100 Gbps cable.
%\atsushi{Can we simplify the above like this: Cluster 1 is equipped with two machines powered by AMD EPYC 7413 (24 cores, 1.5 GHz) and 251.74 GiB memory.}

%Cluster 2 is equipped with three machines with CPU (marked as CPU-2 in the respective plots): Intel(R) Core(TM) i9-9900K (8 cores, 3.2 GHz), memory: 64 GiB, caches: 32 KiB (L1 data and code), 256 KiB (L2) and 16 MiB (L3). Cluster 2 nodes are connected over a 40GbE QSFP+ network switch.
%\antonis{CPU-1 and CPU-2 are not memorable names, consider AMD, x86?} %\atsushi{I agree with Antonis. Also, can we rename Cluster 1 and 2 like this: AMD-FPGA Cluster and Intel Cluster?} \atsushi{Cluster 2 is equipped with three machines powered by Intel(R) Core(TM) i9-9900K (8 cores, 3.2 GHz) with 64GiB memory.}



We evaluate the performance of \projecttitle{} across three dimensions: {\em (i)} the hardware evaluation which focuses on the Attestation kernel evaluation (\S~\ref{subsec:hw_eval}), {\em (ii)} the network library evaluation which assesses and compares the \projecttitle{} with competitive network stack baselines (\S~\ref{subsec:net_lib}) and {\em (iii)} different use-cases we built to evaluate our four secure primitive-examples we constructed on top of \projecttitle{} (\S~\ref{subsec:use_cases_eval}). 





\subsection{Hardware Evaluation: \trustedfpga{}}
\label{subsec:hw_eval}


\begin{table}
\begin{center}
\small
\begin{tabular}{ |c|c|c| } 
 \hline
 System &  (host) TEE-free & Tamper-proof \\ [0.5ex] \hline \hline
 SSL-lib & Yes & No\\
 SSL-server/x86*/AMD  &  Yes & No\\
 SGX/AMD-sev &  No & Yes\\
% TEE-P [Hybster, Damysus, Trinc] & Yes & Yes & Yes & Assumes trusted local persistent state\\
 %TEE-DS & Yes & Yes & Yes & Builds a DS of $f+2u+1$ TEEs\footnote{$f$ is the compromised TEEs and $u$ is the number of unresponsive TEEs}\\
 \projecttitle{} & Yes & Yes\\
 \hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{(Trusted) Host-sided hardware baselines and \projecttitle{}. (*) We also the term SSL-server for this run unless stated otherwise.}
\label{tab:hw_options}
%\vspace{-18pt}
\end{table}

\myparagraph{Baselines} We evaluate the performance of the \projecttitle{}'s attestation kernel {\tt Attest} function (Algorithm~\ref{algo:primitives}) compared with four competitive (host-sided) systems: (Intel-)x86 (untrusted), AMD (untrusted), SGX (TEE-based) and AMD-sev (TEE-based). For these host-sided versions we build servers based on OpenSSL that run natively or within a TEE and attest and forward the network messages to the interested host process. From now on we use the term x86 and AMD to refer to a native run of the server process (SSL-server) and the terms SGX and AMD-sev to refer to their tamper-proof versions within a TEE. Both the server process and the host process run in the same machine to eliminate network latency and communicate through TCP sockets. We implement the SGX system using the {\scone{}} framework~\cite{scone} that optimizes (exit-less) syscalls execution while AMD-sev system runs in a QEMU VM using the official supported kernel image~\cite{AMDSEV}. In addition, we build the SSL-lib which integrates the {\tt Attest} function as a library (natively). Recall that both SSL-lib and SSL-server are not tamper-proof. Table~\ref{tab:hw_options} summarizes our baselines with \projecttitle{}. %To avoid distortion, our plots do not include Trinc~\cite{levin2009trinc} because its reported latencies are an order of magnitude slower (85-105 ms) than all other evaluated solutions.


%(Table~\ref{tab:hw_options})
%Nat-lib is an OpenSSL-based library integrated into the code logic that generates and verifies messages. Nat is an OpenSSL-based server that communicates through kernel TCP sockets with the interested process to attest and verify its messages. \atsushi{can we shorten the description of Nat and Nat-lib?} Similarly, SGX and AMD-sev are OpenSSL-based servers that run within a tamper-proof TEE---specifically, Intel SGXv1~\cite{cryptoeprint:2016:086} and AMD-sev~\cite{amd-sev} (configured without offering confidentiality), respectively.  We implement the SGX-based server using the {\tt SCONE} framework~\cite{scone} to execute (exit-less) syscalls in a performant fashion. We run AMD-sev as a QEMU VM using the official supported kernel image~\cite{AMDSEV}, which efficiently runs un-modified Linux applications. Experiments with CPU-1, CPU-2, and SGX ran on Cluster 2, whereas we ran AMD-sev experiments on Cluster 1 \atsushi{CPU-1 should also be on Cluster 1, right?}. 
%On purpose, we exclude  Trinc~\cite{levin2009trinc} because it reported latencies that are an order of magnitude slower (85-105 ms) than \projecttitle{}. 
%To avoid distortion, our plots do not include 
%Trinc~\cite{levin2009trinc} because its reported latencies are an order of magnitude slower (85-105 ms) than all other evaluated solutions.
% \projecttitle{}

%\antonis{Differences between Nat and Nat-lib are not clear. Also, names could be more descriptive/memorable (Nat-lib is also very similar to NET-LIB).}

%\atsushi{can we remove this paragraph? (due to the space)} In short, we seek to answer the following research questions:
%\begin{itemize}
%\item {\bf{RQ1.}} What is the performance for generating and verifying attested messages in \projecttitle{}?
%\item {\bf{RQ2.}} What is the performance breakdown and latencies?
%    \item[\bf{RQ3}]  How much resources \projecttitle{} uses for the attestation kernel (Table~\ref{table:resources_usage})?
 %   \item[\bf{RQ4}] What is the hardware network latency and throughput (Fig~\ref{fig:hw_lat_breakdown})?
%\end{itemize}

\myparagraph{Methodology and experiments}
We use Vitis XRT v2022.2 for the stand-alone evaluation of \projecttitle{} attestation kernel. We load the shell \texttt{xilinx\_u280\_gen3x16\_xdma\_base\_1} and use Vitis XRT synchronous data transfers from host to device and vice versa. We measure and report the {\tt Attest} function average latency as well as the communication costs executing an empty funcation body.
%To isolate the latencies between data transfers and computation we further execute the same experiment without computing the HMAC (empty kernel). \atsushi{I wanna simplify the texts here... work on it later}

%We use Vitis XRT v2022.2 for the stand-alone evaluation of \projecttitle{} attestation kernel on top of which we build the host and the \trustedfpga{} processes (\texttt{xilinx\_u280\_gen3x16\_xdma\_base\_1}). We use Vitis XRT synchronous data transfers from host to device and vice versa. We measure and report the HMAC average latency on these competitive systems. To isolate the latencies between data transfers and computation we further execute the same experiment without computing the HMAC (empty kernel). \atsushi{I wanna simplify the texts here... work on it later}


\myparagraph{Results}
Figure~\ref{fig:attest_kernel} shows the average latency of the {\tt Attest} function based on the HMAC algorithm for data inputs of 64B and 128B. The {\tt Verify} function's latency is similar and, as such, it is omitted. Our \projecttitle{} achieves performance in the microseconds range (23 us) and outperforms its equivalent TEE-based competitors at least by a factor of 2. Importantly, \projecttitle{} is approximately 1.2$\times$ faster than the native runs of the SSL-server in AMD system, although it is approximately 2$\times$ slower than the Intel-x86. Recall that both ADM and Intel-x86 are not tamper-proof.

Figure~\ref{fig:latency_breakdown} shows the latency breakdown of the  {\tt Attest} function. Accessing the \projecttitle{} device and the TEEs can be expensive ranging from 30\% to 90\% of the total operation latency among the systems. Specifically, for \projecttitle{}, the transfer time takes about 16 us, which accounts for 70\% of the total execution time. This is not a concern in \projecttitle{} as it effectively eliminates this cost by enabling asynchronous (user-space) DMA data transfers. Regarding the native runs, i.e., Intel-x86 and AMD, the communication costs including the syscalls execution, data transfers between the two processes account for the $~$90\% of the latency.  

Our evaluation showed that in the TEE-based systems, e.g., SGX and AMD-sev, the communication and system call execution costs account for up to 40\% of the total execution (on average). To our surprise this implies that the HMAC computation itself within any of the two TEEs experiences more than 30$\times$ overheads compared to its native run. We further analyzed TEEs' behavior instrumenting the client's code to accurately measure the operations' individual latency at various periods of time during the experiment. 

Figure~\ref{fig:latency_distribution} illustrates the individual operations latency for three systems: SGX (which runs the HMAC within an SGX SSL-server), SGX-empty (the SGX SSL-server copies and returns the input data without HMAC computation) and Intel-x86 (the SSL-server runs natively).  As shown in Figure~\ref{fig:latency_distribution}, the execution of HMAC within the SGX quite often experiences huge spikes in latency. While these spikes are very frequent, they are not guaranteed. We calculate an average mean of 45us and a geometric mean of 30 us. We attribute this behavior to scheduling effects and the asynchronous exitless system call API which is involved~\cite{scone}. Similar variations were observed for the AMD runs with latencies spiking up to 200--500 us.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{atc-submission-plots/hw_eval_attest_latency.pdf} 
  \caption{{\tt Attest} function latency.}
  \label{fig:attest_kernel}
\end{figure}

\begin{figure}
    \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/latency_breakdown.pdf}
  \caption{{\tt Attest} function latency breakdown.}\label{fig:latency_breakdown}
\end{figure}

\begin{figure}
    \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/foo100.pdf}
  \caption{{\tt Attest} function latency over time in SGX.}\label{fig:latency_distribution}\label{fig:latency_breakdown}
\end{figure}

\if 0
\begin{figure*}[t!]
\begin{center}
\minipage{0.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/hw_eval_attest_latency.pdf} 
  \caption{HMAC (Attest) latency}
  \label{fig:attest_kernel}
\endminipage
\minipage{0.33\textwidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/latency_breakdown.pdf}
  \caption{Latency breakdown}\label{fig:latency_breakdown}
\endminipage

\minipage{0.50\textwidth}%
  \centering
  %\includegraphics[width=\linewidth]{atc-submission-plots/lat_distribution_sgx.pdf}
  \includegraphics[width=\linewidth]{atc-submission-plots/foo50.pdf}
  \caption{Latency distribution over time}\label{fig:latency_distribution}
\endminipage
\end{center}
%\caption{Performance evaluation of the trusted component in different hardware setups.} \label{fig:hw_eval}
\end{figure*}
\fi

\if 0
\begin{figure}[t!]
    \centering
    \includegraphics[width=.5\textwidth]{eval-plots/plots/hw_net_lat_throughput.pdf}
    \caption{Throughput latency plots for network operation.}
    \label{fig:hw_lat_breakdown}
\end{figure}
\fi

\if 0
\begin{center}
\begin{table}[ht]
\centering
\begin{tabular}{ |m{1.5cm}||m{1cm}| m{1cm}| m{1cm}|}
 \hline
  & LUTs &  BRAM & Regs  \\
 \texttt{Attest()} &  &  &\\
 \texttt{Verify()} &  &  &\\
 \hline
 \end{tabular}
\caption{Resources usage.}
\end{table}\label{table:resources_usage}
\end{center}
\fi



==> backups/evaluation_net.bak2.tex <==
\subsection{Software Evaluation: \projecttitle{} Network Stack}\label{subsec:net_lib}

\myparagraph{Baselines} We evaluate the performance of our \projecttitle{} where we seek to show {\em{(i)}} the effectiveness of our decision to shift the network stack from host CPUs to modern data accelerators and {\em{(ii)}} the overheads that our system incurs due to materializing the requirements for CFT systems transformation (discussed in $\S~\ref{sec:requirements-ds}$). As such, we evaluate and compare \projecttitle{} across four other network stacks implemented on software or hardware with different security properties. %Specifically, we use the acronym D-I/O to refer to a Direct I/O network stack that bypasses the kernel stack (for performance). The acronyms D-I/O w/ A. and \projecttitle{} w/ A. means that the network stack generates and sends attested messages without verifying them at the receiving side. 
%\atsushi{What do you think new labels like this: RDMA-hw, DRCT-IO, DRCT-IO-acc, TNIC, TNIC-acc}

Specifically, we evaluate five different network stacks: {\em (i)} RDMA-hw which implements a reliable, untrusted RoCE protocol on FPGAs, {\em (ii)} our \projecttitle{}, {\em (iii)} DRCT-IO, a direct I/O, untrusted, software-based network stack that bypasses the kernel stack, {\em (iv)} DRCT-IO-att, the previous stack that offers trust by sending attested messages (using an SGX-based SSL-server) without verifying them at the receiving side and {\em (v)} \projecttitle{}-att that similarly sends attested messages but does not verify them. We build the RDMA-hw experiment on top of Coyote~\cite{coyote} network stacks imilarly to \projecttitle{}, . For the DRCT-IO versions, we base our design on eRPC~\cite{erpc} with DPDK~\cite{dpdk} that offers similar reliability guarantees with RDMA-hw. The benchmarks with hardware implementation run on AMD-FPGA Cluster, whereas the rest run on Intel Cluster.
%\antonis{again names are not very memorable. Something more %descriptive/relevant to the paper than D-I/O, etc.?}
%\atsushi{Which term we should use for our proposal: \projecttitle{} or \projectlibrary{}?}

%Specifically, our evaluation answers the following questions:
%\begin{itemize}
%    \item {\bf RQ1.} How much does \projecttitle{}'s offered security cost?
%    \item {\bf RQ2.} How does \projectlibrary{} performs compared to competitive network %stacks?
%\end{itemize}

\begin{figure*}
    \centering
   \includegraphics[width=\linewidth]{atc-submission-plots/rpc_lat.pdf} 
  \caption{Latency evaluation of send operations for various packet sizes across five competitive network stacks with various security properties.}
  \label{fig:net_latencies}
\end{figure*}

\begin{figure}
    \centering
   \includegraphics[width=0.9\linewidth]{atc-submission-plots/rpc_thr.pdf} 
    \caption{Throughput evaluation of send operations for various packet sizes across five competitive network stacks with various security properties.}
  \label{fig:net_throughput}
\end{figure}

\if 0
\begin{figure}[t!]
\begin{center}
\minipage{0.7\linewidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/tnic_overheads.pdf} 
\endminipage
\minipage{0.3\linewidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/tnic_speedup.pdf} 
  %\label{fig:net_speedup}
\endminipage
\end{center}
\caption{Left figure shows the slowdown of \projecttitle{} w.r.t. to RDMA-hw. Right figure shows the speedup of \projecttitle{} w.r.t. DRCT-IO-att.}\label{fig:net_slowdown}
\end{figure}
\fi

\myparagraph{Methodology and experiments} All our runs in the section have been conducted through a single-threaded client-server implementation that uses the respective network stack. In the throughput experiments the client issues more than one on-going operation whereas to optimize for the latency (and accurately measure it) the client process sends one operation at a time in the respective experiments.  We decided on these settings for two reasons. First, commercial blockchain systems whose design relies on BFT systems to implement ordering services~\cite{10.1145/3190508.3190538} for the ledger have shown that ordering operations dominates the overall latency. As such we want to reliably illustrate \projecttitle{} latencies. Secondly, parallelism in (totally-ordered) consensus protocols (e.g., ~\cite{10.1145/3190508.3190538}) have been evaluated to have little or minimal performance improvements~\cite{f04eb9b864204bab958e72055062748c, 10.1145/3299869.3319893}.
%have already shown that parallelism in (totally-ordered) consensus protocols (as in~\cite{10.1145/3190508.3190538})  offer minimal to no performance improvements.
%\atsushi{Can we simplify the paragraph like this: we run experiments in such settings... for two reasons. First, commercial blockchain systems... Second, parallelism in consensus... has already been evaluated. }

\myparagraph{Results} 
Figure~\ref{fig:net_latencies} and~\ref{fig:net_throughput} show the latency and the throughput of the send operation with of various sizes data transfers between two machines across the network. The latencies of both \projecttitle{} and \projecttitle{}-att. increase linearly with the packet size in contrast to the (untrusted) RDMA-hw latencies which remain stable (5---7us) for packet sizes up to 4KiB and are tripled thereafter (18---20us). Our \projecttitle{}'s offers trusted networking with latencies that are 3$\times$---20$\times$ higher than the untrusted RDMA-hw. \projecttitle{} network latency is dominated primarily by the HMAC calculation. As this algorithm fundamentally cannot be parallelized, the higher the message size, the higher the latency our \projecttitle{} incurs. More specifically, in \projecttitle{}, for packet sizes that are less than 1~KiB, doubling the packet size results in 13\%---20\% increment in the overall latency. For packet sizes bigger or equal to 1~KiB, doubling the packet size increases the latency by 30\%---40\%. 

Compared to the DRCT-IO-att (82us) our \projecttitle{} is up to 5.6$\times$ faster. Importantly, DRCT-IO-att reported extreme latencies (2000us or more) for packet sizes larger than 521B. We attribute these latencies to the scheduling effects of the framework to access the TEE~\cite{scone} and we omitted these numbers to avoid plot distortion. 

For packet sizes up to 1~KiB the DRCT-IO offers minimal latency (16-16.6us) due to zero-copy transmission/reception optimizations~\cite{erpc} that are only effective for up to 1460B (MTU is 1500B but 40B are reserved for metadata).  The RDMA-hw achieves 3$\times$ lower latency (5-5.5us) for packet sizes up to 2~KiB. For bigger data transfers, the RDMA-hw latency increases steadily up to 19~us whereas DRCT-IO does not scale well with latencies up to 100us.  Overall, the RDMA-hw is 3$\times$---5$\times$ faster than the DRCT-IO showing that network offloading to the hardware boosts performance.

%We now compare the untrusted software and hardware implementations of the network stacks. The RDMA-hw is 3$\times$---5$\times$ faster than the DRCT-IO. For packet sizes up to 1~KiB the DRCT-IO offers minimal latency (16-16.6us) due to zero-copy transmission/reception optimizations~\cite{erpc} that are only effective for up to 1460B (MTU is 1500B but 40B are reserved for metadata). Recall that even with such optimizations .  For bigger data transfers, the RDMA-hw latency increases steadily up to 19~us for packet size to be equal to 32KiB. DRCT-IO, on the other hand, does not scale well for bigger packet sizes, reporting latency up to 100us, mainly because network stack operations (e.g., packet fragmentation, packet construction, etc.) are running in software in contrast to RDMA-hw. 


%Lastly, D-I/O-att. shows stable latency (82us) for packet sizes up to 512. For larger packet sizes, we measured extreme latencies (2000us or more), which we attribute to the scheduling effects of the framework to access the TEE~\cite{scone}. We omit these numbers to avoid plot distortion.


%Latencies of both \projecttitle{} and \projecttitle{} w/ A. increase linearly with the packet size. This is primarily due to HMAC calculation, which fundamentally is not improved by parallelism. As such, the higher the message size, the higher the latency our \projecttitle{} incurs. Specifically, in \projecttitle{}, for packet sizes that are less than 1~KiB, doubling the packet size results in 13\%---20\% increment in the overall latency. For packet sizes bigger or equal to 1024, doubling the packet size increases the latency by 30\%---40\%. \projecttitle{} w/ A. shows similar behavior. Lastly, D-I/O w/ A. shows stable latency (82us) for packet sizes up to 512. For larger packet sizes, we measured extreme latencies (2000us or more), which we attribute to the scheduling effects of the framework to access the TEE~\cite{scone}. We omit these numbers to avoid plot distortion.


Lastly, we calculated the slowdown of \projecttitle{} compared to the RDMA-hw (Figure~\ref{fig:net_slowdown} (left)) and the speedup of \projecttitle{} compared to DRCT-IO-att  (Figure~\ref{fig:net_slowdown} (right)). As expected, the bigger the packet size, the higher the respective overhead; this is due to HMAC calculations, as explained.  \projecttitle{} has 3---20$\times$ overhead compared to RDMA-hw and 3$\times$---5$\times$ speedup compared to its equivalent software based implementation that uses SGX as network packets authenticator. The overheads are the result of the HMAC calculation whereas the speedup is the result of both the network stack offloading in hardware and the on-data-path security processing thanks to \projecttitle{} attestation kernel.


==> backups/evaluation_net2.tex <==
\subsection{Software Evaluation: \projecttitle{} Network Stack}\label{subsec:net_lib}

\myparagraph{Baselines} We evaluate the performance of our \projecttitle{} where we seek to show {\em{(i)}} the effectiveness of our decision to shift the network stack from host CPUs to modern data accelerators and {\em{(ii)}} the overheads that our system incurs due to materializing the requirements for CFT systems transformation (discussed in $\S~\ref{sec:requirements-ds}$). As such, we evaluate and compare \projecttitle{} across four other network stacks implemented on software or hardware with different security properties. %Specifically, we use the acronym D-I/O to refer to a Direct I/O network stack that bypasses the kernel stack (for performance). The acronyms D-I/O w/ A. and \projecttitle{} w/ A. means that the network stack generates and sends attested messages without verifying them at the receiving side. 
%\atsushi{What do you think new labels like this: RDMA-hw, DRCT-IO, DRCT-IO-acc, TNIC, TNIC-acc}

Specifically, we evaluate five different network stacks: {\em (i)} RDMA-hw which implements a reliable, untrusted RoCE protocol on FPGAs, {\em (ii)} our \projecttitle{}, {\em (iii)} DRCT-IO, a direct I/O, untrusted, software-based network stack that bypasses the kernel stack, {\em (iv)} DRCT-IO-att, the previous stack that offers trust by sending attested messages (using an SGX-based SSL-server) without verifying them at the receiving side and {\em (v)} \projecttitle{}-att that similarly sends attested messages but does not verify them. We build the RDMA-hw experiment on top of Coyote~\cite{coyote} network stacks imilarly to \projecttitle{}, . For the DRCT-IO versions, we base our design on eRPC~\cite{erpc} with DPDK~\cite{dpdk} that offers similar reliability guarantees with RDMA-hw. The benchmarks with hardware implementation run on AMD-FPGA Cluster, whereas the rest run on Intel Cluster.
%\antonis{again names are not very memorable. Something more %descriptive/relevant to the paper than D-I/O, etc.?}
%\atsushi{Which term we should use for our proposal: \projecttitle{} or \projectlibrary{}?}

%Specifically, our evaluation answers the following questions:
%\begin{itemize}
%    \item {\bf RQ1.} How much does \projecttitle{}'s offered security cost?
%    \item {\bf RQ2.} How does \projectlibrary{} performs compared to competitive network %stacks?
%\end{itemize}

\begin{figure*}
    \centering
   \includegraphics[width=\linewidth]{atc-submission-plots/rpc_lat.pdf} 
  \caption{Latency evaluation of send operations for various packet sizes across five competitive network stacks with various security properties.}
  \label{fig:net_latencies}
\end{figure*}

\begin{figure}
    \centering
   \includegraphics[width=0.9\linewidth]{atc-submission-plots/rpc_thr.pdf} 
    \caption{Throughput evaluation of send operations for various packet sizes across five competitive network stacks with various security properties.}
  \label{fig:net_throughput}
\end{figure}

\begin{figure}[t!]
\begin{center}
\minipage{0.7\linewidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/tnic_overheads.pdf} 
\endminipage
\minipage{0.3\linewidth}
  \centering
  \includegraphics[width=\linewidth]{atc-submission-plots/tnic_speedup.pdf} 
  %\label{fig:net_speedup}
\endminipage
\end{center}
\caption{Left figure shows the slowdown of \projecttitle{} w.r.t. to RDMA-hw. Right figure shows the speedup of \projecttitle{} w.r.t. DRCT-IO-att.}\label{fig:net_slowdown}
\end{figure}

\myparagraph{Methodology and experiments} All our runs in the section have been conducted through a single-threaded client-server implementation that uses the respective network stack. In the throughput experiments the client issues more than one on-going operation whereas to optimize for the latency (and accurately measure it) the client process sends one operation at a time in the respective experiments.  We decided on these settings for two reasons. First, commercial blockchain systems whose design relies on BFT systems to implement ordering services~\cite{10.1145/3190508.3190538} for the ledger have shown that ordering operations dominates the overall latency. As such we want to reliably illustrate \projecttitle{} latencies. Secondly, parallelism in (totally-ordered) consensus protocols (e.g., ~\cite{10.1145/3190508.3190538}) have been evaluated to have little or minimal performance improvements~\cite{f04eb9b864204bab958e72055062748c, 10.1145/3299869.3319893}.
%have already shown that parallelism in (totally-ordered) consensus protocols (as in~\cite{10.1145/3190508.3190538})  offer minimal to no performance improvements.
%\atsushi{Can we simplify the paragraph like this: we run experiments in such settings... for two reasons. First, commercial blockchain systems... Second, parallelism in consensus... has already been evaluated. }

\myparagraph{Results} 
Figure~\ref{fig:net_latencies} and~\ref{fig:net_throughput} show the latency and the throughput of the send operation with of various sizes data transfers between two machines across the network. The latencies of both \projecttitle{} and \projecttitle{}-att. increase linearly with the packet size in contrast to the (untrusted) RDMA-hw latencies which remain stable (5---7us) for packet sizes up to 4KiB and are tripled thereafter (18---20us). Our \projecttitle{}'s offers trusted networking with latencies that are 3$\times$---20$\times$ higher than the untrusted RDMA-hw. \projecttitle{} network latency is dominated primarily by the HMAC calculation. As this algorithm fundamentally cannot be parallelized, the higher the message size, the higher the latency our \projecttitle{} incurs. More specifically, in \projecttitle{}, for packet sizes that are less than 1~KiB, doubling the packet size results in 13\%---20\% increment in the overall latency. For packet sizes bigger or equal to 1~KiB, doubling the packet size increases the latency by 30\%---40\%. 

Compared to the DRCT-IO-att (82us) our \projecttitle{} is up to 5.6$\times$ faster. Importantly, DRCT-IO-att reported extreme latencies (2000us or more) for packet sizes larger than 521B. We attribute these latencies to the scheduling effects of the framework to access the TEE~\cite{scone} and we omitted these numbers to avoid plot distortion.

We now compare the untrusted software and hardware implementations of the network stacks. The RDMA-hw is 3$\times$---5$\times$ faster than the DRCT-IO. For packet sizes up to 1~KiB the DRCT-IO offers minimal latency (16-16.6us) due to zero-copy transmission/reception optimizations~\cite{erpc} that are only effective for up to 1460B (MTU is 1500B but 40B are reserved for metadata). Recall that even with such optimizations the RDMA-hw achieves 3$\times$ lower latency (5-5.5us) for packet sizes up to 2~KiB.  For bigger data transfers, the RDMA-hw latency increases steadily up to 19~us for packet size to be equal to 32KiB. DRCT-IO, on the other hand, does not scale well for bigger packet sizes, reporting latency up to 100us, mainly because network stack operations (e.g., packet fragmentation, packet construction, etc.) are running in software in contrast to RDMA-hw. 


%Lastly, D-I/O-att. shows stable latency (82us) for packet sizes up to 512. For larger packet sizes, we measured extreme latencies (2000us or more), which we attribute to the scheduling effects of the framework to access the TEE~\cite{scone}. We omit these numbers to avoid plot distortion.


%Latencies of both \projecttitle{} and \projecttitle{} w/ A. increase linearly with the packet size. This is primarily due to HMAC calculation, which fundamentally is not improved by parallelism. As such, the higher the message size, the higher the latency our \projecttitle{} incurs. Specifically, in \projecttitle{}, for packet sizes that are less than 1~KiB, doubling the packet size results in 13\%---20\% increment in the overall latency. For packet sizes bigger or equal to 1024, doubling the packet size increases the latency by 30\%---40\%. \projecttitle{} w/ A. shows similar behavior. Lastly, D-I/O w/ A. shows stable latency (82us) for packet sizes up to 512. For larger packet sizes, we measured extreme latencies (2000us or more), which we attribute to the scheduling effects of the framework to access the TEE~\cite{scone}. We omit these numbers to avoid plot distortion.


Lastly, we calculated the slowdown of \projecttitle{} compared to the RDMA-hw (Figure~\ref{fig:net_slowdown} (left)) and the speedup of \projecttitle{} compared to DRCT-IO-att  (Figure~\ref{fig:net_slowdown} (right)). As expected, the bigger the packet size, the higher the respective overhead; this is due to HMAC calculations, as explained.  \projecttitle{} has 3---20$\times$ overhead compared to RDMA-hw and 3$\times$---5$\times$ speedup compared to its equivalent software based implementation that uses SGX as network packets authenticator. The overheads are the result of the HMAC calculation whereas the speedup is the result of both the network stack offloading in hardware and the on-data-path security processing thanks to \projecttitle{} attestation kernel.

==> backups/implementation.tex <==
\section{Implementation}

==> backups/introduction.tex <==
%\section{Introduction}

\antonis{Suggestion: Let's keep \textit{names} (baselines, our solutions, etc.) short, consistent, descriptive, and memorable. Maybe tNIC (tFPGA, tNET-LIB) rather than TNIC (T-FPGA, NET-LIB).}
%\antonis{are we open-sourcing anything from this paper? if so, let's mention it somewhere.}


\myparagraph{intro notes}
\begin{itemize}
    \item[1] distributed systems + cloud, - networking a play an important role and the need for building trusted distributed systems 
    \item[2] secure distributed system properties: safe, live, and correct in presence Byzantine adversary. (define Byzantine here)
    \item[3]  There is PATH: silicon root of trust is promising approach to build trusted distributed systems, in particular TEEs. It is provided by all cloud-providers -- BUT have limitations for DS:  (background of challenges-> bring networking aspect)
\end{itemize}

The challenges of conventional TEE appraoch:

1) host-side TEEs: Progamaaiblity + security/correct challenges (Beefy TCP/OS which we do not need or complicate correctness) + performance + Heterogenity (lack of unified abstraction). How do you stitch all these heterogenous TEEs all together? One unidied abstarction (heterogeneours nodes, blah) at the Network level 


2)  - They provide a lot of features, which mean still High TCB, we don't even need to know all those features!

    => Our goal to find minimal abstraction for trusted distributed systems.

    => Minimal requirements: a) non-equivocation and transferable authentication

3) Performance: Distributed systems are relying of networked-systems, and they need network to be fast and  protocol offloading is already prominent, can we build it on fast path. Why can't we offload the security processing threre too?


Overall question: 

What is the unified, minimal and high-performance networking abstraction for building trusted distributed systems in the untrusted heterogenous cloud?



Our approach:

- Unified abstraction for network level isolation.

- Minimalistic: two properties (just state the properties)-> are guaranteed to build trusted systems. TEEs cannot be verified whereas our minimal can do this! In fact, we do this and ..


- Performance: implement at the NIC.



Cross-layer approach:

- bottom up: hardware nic
- network stack
- library
- applications.

implementation

Evaluation.

Contributions: 

- formal verification


\myparagraph{Design requirements for distributed systems notes}

- Requirements for trustworthy distributed systems:

    - crash vs byzantine systems

-bring what do they need actually? trade-offs? what  how can we secure them with bringing the trusted hardware?
required properties to transform? security only two properties.


- Performance 

 - heterogenous nodes -- unified a set of heterogenosu nodes


 [IMPORTANT] THis section end with the message -- we need to end the NIC level trusted hardware...

\myparagraph{overview notes}

- section: Design requirement for trusted NICs

- system overview

- System model.



%To make matters worse,  large-scale datacenters (DCs) are highly \emph{heterogeneous}: with machines not only differing in terms of configuration space (memory, storage, etc.), but more importantly, with carrying different (host) CPU architectures with various capabilities too~\cite{6756704}. This is an inevitable result of the continuous growth of the cloud~\cite{cloud_growth, google_servers} and the limited lifespan of the machines~\cite{dc_lifespan}. Consequently, the replication protocols and systems need to be designed and implemented to be able to run transparently and preserve their security and correctness properties even in heterogeneous CPUs. 


\myparagraph{Motivation} An ever-increasing amount of data storage and computing is performed in the cloud due to the cost benefits for both the users and the cloud providers. Large-scale cloud providers, (e.g., Amazon EC2~\cite{amazon_ec2}, Microsoft Windows Azure~\cite{microsoft_azure}, Rackspace~\cite{rackspace} and Google Compute Engine~\cite{google_engine}) have built datacenters (DCs) to provide a computing infrastructure for users to run their applications. 

The cloud infrastructure is characterized by {\em (1)} heterogeneity and {\em (2)} distribution. The DCs have an heterogeneous computing infrastructure with machines not only differing in configuration space (memory, storage, etc.), but more importantly, with carrying different (host) CPU architectures~\cite{6756704} with limited lifespan~\cite{dc_lifespan}. At the same time, tens of thousands of user applications mandate more than one distributed machines to cooperate or rely on provided high-end distributed systems (i.e., storage systems and databases~\cite{dynamo,  azure_storage, tao, spanner, 51, zippy, AmazonS3}, management services~\cite{Hunt:2010, Burns2016} and computing frameworks~\cite{aws_lambda, azure_functions, google_cloud_functions}). 

Undoubtedly, these distributed systems and user applications must be highly available, fast, and trustworthy. They need to remain correct even when failures occur~\cite{ford2010availability, Mazieres2002b, Garay2000}. As such, their vast majority ensure availability in the presence of faults by deploying replication protocols~\cite{Raft, azure, Fan-MemC3, DeCandia2007, ford2010availability, cockroachdb, farm, Hermes:2020, fasst, zippydb}. These replication protocols usually target a very limited range of faults: they assume a Crash Fault Tolerant (CFT) model where the participating nodes and the cloud infrastructure are trusted and fail only by crashing~\cite{delporte}. In the rest of the paper, we refer to such protocols as CFT protocols.


%\dimitra{Talk about security implications}

Unfortunately, this widespread and multi-dimensional adoption of the cloud has drastically increased the surface area of faults and attacks that go beyond the CFT model, ranging from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, high_resolution_side_channels}. CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults.




\if 0
To make matters worse, these systems need to be designed and run in large-scale cloud environments equipped with thousands of machines: e.g., Google is estimated to own more than 2\% of all servers in the world~\cite{google_servers}.  Several generations of machines with different specifications are continuously being encountered: First, as the underlying machine types evolve over time, newer machines offer a more attractive price-performance solution. Secondly, (old) machines wear out and are replaced by newer and more powerful ones: the average useful lifespan of a server is estimated to be 3---5 years~\cite{dc_lifespan}. Lastly, the global market of the public cloud is continuously growing---specifically, it is estimated to grow at least $20\%$ each year~\cite{cloud_growth}. As a result, modern datacenters are highly\emph{heterogeneous}: the machines not only can differ in terms of configuration space (memory, storage, etc.), but more importantly, they carry different (host) CPU architectures with various capabilities too~\cite{6756704}. Users need to be able to have the right tools available so they can use the right machines/processors in the right place at the right time.
\fi

%\dimitra{Talk about cloud services and distributed protocols}
\if 0
At the same time, while we more and more rely on online cloud-hosted services, there is an urgent need for systems and applications that are highly available, fast, and trustworthy, and, importantly, they remain correct even when failures occur. For this reason, the vast majority of cloud services are designed to ensure availability in the presence of faults by deploying replication protocols~\cite{Raft, azure, Fan-MemC3, DeCandia2007, ford2010availability, cockroachdb, farm, Hermes:2020, fasst, zippydb}. These replication protocols target a limited spectrum of faults assuming that the participant nodes and the cloud infrastructure can be trusted. More specifically, they target the Crash Fault Tolerant (CFT) model that assumes a fail-stop fault model; the participant machines are trusted (e.g., execute the application code correctly, do not have corrupted memory/storage and network packets, etc.) and can only fail by crashing~\cite{delporte}. We refer to such protocols as CFT protocols.
\fi

%\dimitra{Talk about security implications}
\if 0
However, this wide adoption of the third-party cloud infrastructure has drastically increased the surface of faults and attacks that range, beyond the CFT model, from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, high_resolution_side_channels}. Unfortunately, CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults.
\fi
%\dimitra{Talk about prior work limitations}

\myparagraph{Limitations of state-of-the-art approaches} Prior work has established Byzantine Fault Tolerant (BFT) replication that goes beyond the CFT model and offers important foundations for developing protocols with stronger guarantees~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358, engraft, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, 10.1145/3492321.3519568}. These protocols offer consistent replication when processes that fail in arbitrary ways~\cite{Lamport:1982}. For the rest of the paper, we refer to these protocols as BFT protocols. 
Existing BFT protocols present severe trade-offs between performance, scalability, and adoption that impede their widespread application in the heterogeneous cloud~\cite{bft-time-is-now, 10.1145/1711475.1711494}. %System designers can have BFT either by giving up on scalability and performance~\cite{Castro:2002} \antonis{cite?} or by relying on specific CPU-based hardware trusted modules~\cite{}.


On the one hand, traditional BFT protocols~\cite{Castro:2002, DBLP:journals/corr/abs-1803-05069, 10.1145/1658357.1658358}, can transparently run on any CPU architecture but they have significantly limited performance and scalability~\cite{avocado}. In contrast to CFT protocols that usually operate with $2f+1$ nodes, BFT protocols add up an extra set of $f$ participant nodes, requiring at least $3f+1$ nodes, to tolerate up to $f$ arbitrary faults. They additionally introduce high message complexity~\cite{Castro:2002} or many protocol rounds~\cite{DBLP:journals/corr/abs-1803-05069} which greatly limits low-latency and high-performance operations. 

On the other hand, optimized (hybrid) BFT protocols~\cite{10.1145/3492321.3519568, minBFT, hybster, 10.1145/2168836.2168866, DBLP:journals/corr/LiuLKA16a, 10.1145/1294261.1294280} can operate  with fewer nodes at the cost of generality adoption. In particular, they heavily rely on trusted hardware---more specifically, Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086,arm-realm,amd-sev,riscv-multizone,intelTDX}---to prevent the Byzantine counterparts from making conflicting statements for the same round (equivocation). Unfortunately, hybrid protocols have been built on top of very specific and CPU-dependant TEEs rendering them ill-suited and not easily adopted in modern heterogeneous DCs. 

%In this work, we argue that this reliance on specific TEE limits generality and adoption in modern heterogeneous cloud infrastructure. For example, to run these protocols, a cloud provider must guarantee that there would always be available a required number of machines equipped with specific CPU-generation and TEE hardware version. In cases where this is impossible, protocol designers must be able to program different TEEs. This is rather challenging and raises questions when it comes to performance and correctness: different TEEs not only do they have different programming and performance characteristics but they greatly vary when it comes to security~\cite{10.1007/978-3-031-16092-9_7}. As an example of this, Keystone (RISC-V)~\cite{keystone_eurosys} and Intel SGX (x86)~\cite{intel-sgx} have quite different programming APIs. In addition, Intel SGX can only support a very limited Trusted Computing Base (TCB) compared to Intel TDX~\cite{intelTDX} and AMD-SEV~\cite{amd-sev}. Importantly, commercially available TEEs~\cite{arm-trustzone, intel-sgx, amd-sev, keystone_eurosys, 197162, timber} offer different levels of security (i.e., integrity, freshness and confidentiality) whereas they do not necessarily come with build-in support for secure bootstrapping and remote attestation~\cite{10.1007/978-3-031-16092-9_7, 7807249, secTEE}.


%\dimitra{Research question here:}

\myparagraph{System design and contributions} In this paper, we carefully address these limitations. Specifically, we seek to answer the following question: \emph{How can we design and implement a unified abstraction that is well suited for the heterogeneous modern cloud DCs, to aid in the design of robust replication protocols (e.g., under the BFT model), while targeting performance and scalability??}

%In this paper, we carefully address these limitations. Specifically, we seek to answer the following question: \emph{How can a trusted NIC \antonis{the NIC comes out of the blue here. NICs must be mentioned before.} architecture be designed and implemented to provide a unified abstraction that is well suited for the heterogeneous modern cloud DCs, to aid in the design of robust replication protocols (e.g., under the BFT model), while targeting performance and scalability??}
% \emph{How to design and implement a trusted NIC architecture that offers a unified abstraction well-suited to accommodate performant and scalable BFT replication protocols in heterogeneous DCs?}


%\dimitra{Introduce our \projecttitle{} + properties}

Since network operations are at the core of any distributed system, we tackle the question on the foundational level of a cloud system stack, i.e., the NIC level. In this work, we introduce \projecttitle{}, a trusted NIC architecture for heterogeneous cloud environments. \projecttitle{} aims to address the conflict between performance and adoption by materializing a network stack that allows us to translate CFT protocols to BFT ones without requiring extra rounds and nodes (as in classical BFT), neither homogeneous CPUs or TEEs (as in hybrid BFT). Our \projecttitle{} guarantees the two security properties of non-equivocation and transferable authentication~\cite{clement2012} for the (untrusted) network ensuring that a translation of a CFT protocol to a BFT protocol with $2f+1$ \emph{always} exists ($\S$~\ref{sec:background}). Our \projecttitle{} is carefully designed at the NIC's hardware---specifically, we leverage the SmartNIC technology~\cite{alveo_smartnics, intel_smartnics, bluefield_smartnics, broadcom_smartnics, liquidIO_smartnics, netronome_smartnics}, allowing protocols to seamlessly run in heterogeneous CPUs without relying on homogeneous TEEs hardware.

%\dimitra{Say about components + implementation}

%We designed \projecttitle{} adopting the SmartNIC technology shifting the requirement for homogeneous hardware from the CPU to the NIC-level, removing that way the burden from the protocol designers. 
We implemented \projecttitle{} from the ground-up on real hardware leveraging FPGA-based SmartNICs and, particularly, Alveo U280~\cite{alveo_smartnics}. Our system is comprised of two core components the hardware design of the \projecttitle{} ($\S$~\ref{subsec:tfpga}), and the \projecttitle{} software network library ($\S$~\ref{sec:net-lib}). We build a trusted user-space networking stack based on the RDMA protocol, which we further extend at the hardware level with a minimal hardware component, the attestation kernel, that guarantees the authenticity of the network messages. On top of our trusted network stack, we build the \projecttitle{} networking library that exposes to the developers a trusted, unified-to-heterogeneous-machines, API that \emph{(1)} follows the well-established for distributed programming RDMA programming paradigm and \emph{(2)} improves the security guarantees.

To evaluate the generality and performance of \projecttitle{}, we build four systems using \projecttitle{} APIs ($\S$~\ref{sec:use_cases}): {\em (1)} a single-node trusted log system, {\em (2)} a Byzantine SMR protocol, {\em (3)} a Byzantine Chain Replication protocol, and {\em (4)} an accountability protocol. We compare the \projecttitle{}-based protocols implementations with two TEE-based protocols versions with AMD-sev~\cite{} and Intel SGX~\cite{} ($\S$~\ref{}). Our evaluation shows that \projecttitle{} can improve up to $6\times$ the protocols' throughput compared to their TEE-based versions.


To sum up, we make the following contributions:
\begin{itemize}
    \item We design and implement \projecttitle{}, a trusted NIC architecture on top of FPGA-based SmartNICs, that aids the adoption and the design of highly-performant, scalable, and CPU-independent robust protocols that can be seamlessly deployed in modern heterogeneous DCs.
    \item We build a secure RDMA-based API on top of our \projecttitle{} following the current trends in implementing fast, yet trustworthy distributed protocols.
    \item We show how to use the \projecttitle{} to design and build robust distributed protocols ($\S$~\ref{sec:use_cases}).
\end{itemize}

%\myparagraph{Limitations of \projecttitle{}}
%Contributions:
%\begin{itemize}
    %\item An FPGA kernel that satisfies the CFT$\leftarrow$BFT transformation, by materializing the lower bounds of non-equivocation and transferable authentication from~\cite{}.
    %\item An RPC-library ..
    %\item 3 well-known use-cases
    %\item experimental evaluations

%    \item secure hardware network stack
%    \item secure RCP library
%    \item generality: application to protocols (leader + leaderless)
%\end{itemize}

==> backups/introduction2.tex <==
\section{Introduction}
%as they present the {\em illusion} of a single  giant machine 
%\antonis{"giant machine" seems informal/general, maybe "large computer"?}
%with unlimited resources that {\em transparently} meet the applications' performance and resource requirements
Distributed systems are an integral part of the third-party cloud infrastructure~\cite{amazon_ec2, microsoft_azure, rackspace, google_engine}. While these systems in the cloud manifest in diverse forms, ranging from storage systems~\cite{dynamo, azure_storage, tao, spanner, 51, zippy, AmazonS3} and management services~\cite{Hunt:2010, Burns2016} to computing frameworks~\cite{aws_lambda, azure_functions, google_cloud_functions}, they all must be fast and remain correct when failures occur. %all built on top of networking libraries for communication.

%must be fast and trustworthy
%Undoubtedly, distributed systems . 
Unfortunately, the widespread adoption of the cloud has drastically increased the surface area of faults and attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, high_resolution_side_channels} that go beyond the traditional crash-stop fault model\cite{delporte}. The modern (untrusted) third-party cloud infrastructure severely suffers from arbitrary ({\em Byzantine}) faults~\cite{Lamport:1982} that can range from malicious (network) attacks to configuration errors and bugs that are capable of irreversibly disrupting the correct execution of the system~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, high_resolution_side_channels, Castro:2002}.  %A such, distributed systems in the cloud need now to remain correct even under the presence of arbitrary ({\em Byzantine}) failures~\cite{ford2010availability, Mazieres2002b, Garay2000}.

%prior research has repeatedly showed that TEEs adoption can be complicated and challenging especially in the context of networked  applications ~\cite{avocado, treaty, minBFT,10.1145/3492321.3519568}. 

%Specifically,

A promising solution to build trustworthy distributed systems that remain correct even under the presence of\linebreak Byzantine failures is the {\em silicon root of trust}---specifically, the Trusted Execution Environments (TEEs)~\cite{cryptoeprint:2016:086, arm-realm, amd-sev, riscv-multizone, intelTDX}. While the TEEs offer a (single-node) isolated Trusted Computed Base (TCB),  we have identified three core challenges that render their adoption impractical for building trustworthy distributed systems.
%\dimitra{MAKE the challenges IN a more DIRECT, ABSTRACT WAY}
%% Programmability + heterogeneity -> integration

%\pramod{Could we highlight the keywords in these three design challenges?}

{\bf \em First, TEEs in the cloud are heterogeneous, introducing programmability and security challenges}. TEEs are CPU-dependant environments that come with variations in security~\cite{10.1145/3600160.3600169, 7807249, 10.1007/978-3-031-16092-9_7} and programmability properties~\cite{Baumann2014, scone, 10.1145/3079856.3080208, 10.1145/3460120.3485341, tsai2017graphene, Rkt-io}. Integrating just a few heterogeneous TEEs to build a trustworthy distributed system is a challenging engineering task~\cite{10.1145/3460120.3485341} and complicates the security and correctness analysis of the derived system. We overcome this challenge by designing a {\em host-agnostic} and {\em unified trusted} silicon root of trust at the NIC level, which exposes a trusted network library to resolve the programmability burden.

%Particularly, we desingoffer a {\em trusted  unified} \dimitra{How can we have host agnostic silicon root of trust? Solution we provide a network level abstraction unified, etc. because all machines go through Network... that is attached to the hardware network level} programming interface for the heterogeneous cloud infrastructure without relying on CPU-sided TEEs.

%\dimitra{minimalism + verification}
%% Security properties/vulnerabilities + security analysis -> minimalism
{\bf \em Secondly, TEEs come with a large TCB and an increased attack surface}. Prior research shows a correlation between TCB size and potential vulnerabilities~\cite{10.1145/3379469, 10.5555/1756748.1756832} whereas hundreds of security bugs have already been uncovered in state-of-the-art TEEs~\cite{10.1145/3456631}.  As such, modern TEEs are hard to be formally verified. Our work addresses the challenges by building a {\em minimalistic verifiable TCB}. Our TCB, residing at the NIC level hardware, is equipped with {\em the lower bound of security primitives} (e.g., the non-equivocation and transferable authentication) for building trustworthy distributed systems. We also verify that the offered security properties offer a verifiable silicon root of trust; in fact, we perform an end-to-end formal verification of our offered security and safety properties. 
%For example, we calculated that Intel TDX~\cite{intelTDX}, that ports within the trusted hardware the entire Linux kernel (v5.19~\cite{linuxlifecircle}), ``hardens'' at least 2K lines of (used) code, leading to a TCB of 19MB.


%\antonis{Last sentence here says how we address this problem (which is nice), but previous paragraph does not.}

%temincreases the surface of vulnerabilities and drastically complicates the security analysis of the system. Indeed, prior research has reported hundreds of SGX security flaws that CPU vendors continuously try to patch them by releasing revisions or even introducing new TEEs' architectures. 

%{\bf First}, {HETEROGENEOUS+PROMABABILITY CHALLENGES} TEEs cannot {\em naturally} guarantee correctness properties for the designed system across the heterogeneous machines in the cloud~\cite{}. TEEs are CPU-dependant instructions with varying security properties, threat model and vulnerabilities~\cite{}. As an example, Intel SGX~\cite{} offers different security properties from ARM TrustZone~\cite{}. Stitching all these heterogeneous TEEs together can be as challenging as error prone and violating system safety. 

%{\bf Secondly}, Hundrends of SGX security flaws and many revisions (AMD-sev-snp) and keep patching these things \dimitra{huge TCB->vulnernabliies -> security analysis} TEEs have a high TCB with different programming interfaces that not only does it deteriorate programmability but it complicates the security analysis of the derived distributed system. In this paper, we advocate that minimalism is the key to building secure and trustworthy systems. As such, we target to find a minimal abstraction for building trusted systems.

%\dimitra{two insignts -> (1) CFT-to-BFT and (2) network offloading}
{\bf \em Thirdly, TEEs report significant performance bottlenecks.} The overheads are especially exacerbated in the context of networked systems~\cite{avocado, treaty, minBFT,10.1145/3492321.3519568}--- the foundational building block in the core of any distributed system---due to their slow syscalls execution~\cite{hotcalls}. In our work we offer both security and performance based on two insights: first we materialize a transformation from CFT distributed systems to BFT distributed systems with the minimum required security properties of non-equivocation and transferable authentication. Secondly we offload the security computation at the NIC-level hardware, specifically we extend the scope of the state-of-the-art SmartNICs.


%Recent efforts in academia~\cite{10.1145/3341302.3342079, 10.1145/3476886.3477505, 9040000, 9912712} and industry~\cite{211249, alibaba_smartnics, nitro_smartnics, msr_smartnics} have established that offloading network processing to specialized hardware, i.e., SmartNICs~\cite{liquidIO_smartnics, u280_smartnics, bluefield_smartnics, broadcom_smartnics, netronome_smartnics}, is a promising design to boost performance. Inspired by this trend, we explore the SmartNICs' potential to further extend their scope in building fast and trustworthy distributed systems by offloading security-related processing at the hardware network level. 


%{\bf \em Lastly, TEEs are hard to verify}. As discussed the TEEs integrate a huge TCB that varies between different TEEs complicating its security analysis. In addition to that, while TEEs offer (remote) attestation to   verify the integrity of the TEE and its executing code, the attestation in TEEs (when offered) requires the executing code to be exposed to the TEEs' hardware provider (e.g., Intel Attestation Service~\cite{ias}) which might not be compliant  with any imposed privacy policies. In \projecttitle{} we overcome these limitations. While its offered security properties are decoupled from the application's code, we further formally verify the safety and security guarantees of our system.

%However, there are real-world application scenarios (e.g., proprietary algorithm~\cite{}) where the program itself need to comply with strict privacy policies and cannot be {\em openly} exposed to multiple parties. 

Overall, we seek to answer the following question: {\em What is the minimal host-agnostic high-performant silicon-root-of-trust for building trusted distributed systems in the untrusted heterogeneous cloud?}


Our contribution is the \projecttitle{}, a trusted NIC architecture for distributed systems. Our \projecttitle{} overcomes all the above challenges, offering a {\em unified minimalistic networking abstraction for highly-performant trusted distributed systems} \antonis{"heterogeneity" is not mentioned here.}. 
We design our \projecttitle{} on top of state-of-the-art SmartNICs, removing the dependencies on the CPU-based TEEs for trust. In addition, \projecttitle{} materializes a minimalistic TCB as the key component to design trusted distributed systems in the Byzantine cloud infrastructure. In fact, we opt for the opportunity to prove our argument and formally verify the safety and security guarantees of our \projecttitle{} architecture. %For performance, we offload \projecttitle{}'s TCB  along with the network-level protocol implementation in the specialized SmartNICs hardware. 



Our \projecttitle{} follows a three-layer design: {\em (a)} the \projecttitle{} hardware architecture that implements a trusted RDMA network stack for trusted network operations ($\S$~\ref{sec:t-nic-hardware}), {\em (b)} a trusted (software) network stack that operates as a middle layer between the hardware and the user application bypassing the kernel for performance ($\S$~\ref{sec:t-nic-network}) and {\em (c)} a trusted networking library that exposes programming APIs to system designers ($\S$~\ref{sec:t-nic-software}). 

We have implemented the \projecttitle{}'s hardware architecture on top of Alveo U280 FPGA-based SmartNICs~\cite{u280_smartnics}. Our core component is the \projecttitle{}'s {\em attestation kernel}, the minimal required hardware-assisted TCB that guarantees the necessary security properties across the network ($\S$~\ref{sec:requirements-ds}). In addition to \projecttitle{}'s attestation kernel, we offload to the FPGA an end-to-end implementation of the reliable one-sided RDMA protocol~\cite{rdma_specification} to boost performance. Leveraging \projecttitle{} trusted network library, we show a generic {\em recipe} to transform a distributed system operating under the fail-stop model for Byzantine settings ($\S$~\ref{subsec:transformation}). Lastly, we apply our \projecttitle{}-assisted transformation into four use-cases ($\S$~\ref{sec:use_cases})---specifically, a single-node trusted log system, a state-machine-replication (SMR) protocol, a chain replication system and an accountability protocol---showing the generality of our approach. 


We evaluate \projecttitle{} with a competitive state-of-the-art software-based network stack, eRPC~\cite{erpc}, on top of RDMA~\cite{rdma} and DPDK~\cite{dpdk} that utilizes TEEs to shield the network operations. Our evaluation shows that our \projecttitle{} offers 3$\times$---5$\times$ lower latency than the software-based network stack that relies on CPU-based TEEs for trust. In addition, we evaluate the \projecttitle{}-based versions of the four implemented systems against their (conventional) TEE-based versions. To show the generality of our approach, we implemented the TEE-based versions of the systems using two competitive state-of-the-art TEEs, the Intel SGX~\cite{intel-sgx} and AMD-sev~\cite{amd-sev}. Our evaluation shows that \projecttitle{} can improve the system's throughput by up to $6\times$ compared to their TEE-based implementations.

\pramod{Try to unify the contributions into three? and also use bold keywords/terms to highlight each contribution. -- Maybe we could map them to design contributions?}
In summary, we make the following contributions:
\begin{itemize}
    \item We designed and built \projecttitle{}, a trusted NIC architecture leveraging the state-of-the-art FPGA-based SmartNICs to boost performance while offering security for distributed systems in the untrusted cloud ($\S$~\ref{sec:t-nic-hardware}). 
    \dimitra{Hardware level implementation + minimalism taht allows verifiable + NIC level implementation tfor high performance}
    \item We offer a unified minimalistic high-performant trusted library to system designers ($\S$~\ref{sec:t-nic-software}) on top of a user-space network system stack ($\S$~\ref{sec:t-nic-network}) and we show how to use \projecttitle{} to build a generic transformation of distributed systems for Byzantine settings ($\S$~\ref{subsec:transformation}).
    \item We further demonstrate the generality of our approach in practice by implementing four different secure systems using \projecttitle{} ($\S$~\ref{sec:use_cases}). Specifically, we design and build a single-node trusted log system, an state-machine-replication (SMR) protocol, a chain replication system, and an accountability protocol that are fundamental building blocks in the cloud.
    \item We formally verify the safety and security guarantees of our \projecttitle{} architecture from the bootstrapping process to the normal-operation network operations ($\S$~\ref{subsec::formal_verification_remote_attestation}).
    
    %\item We designed and built \projecttitle{}, a trusted NIC architecture leveraging the state-of-the-art FPGA-based SmartNICs to boost performance while offering security for distributed systems in the untrusted cloud ($\S$~\ref{sec:t-nic-hardware}). 
    %\item We offer a unified minimalistic high-performant trusted library to system designers ($\S$~\ref{sec:t-nic-software}) on top of a user-space network system stack ($\S$~\ref{sec:t-nic-network}) and we show how to use \projecttitle{} to build a generic transformation of distributed systems for Byzantine settings ($\S$~\ref{subsec:transformation}).
    %\item We further demonstrate the generality of our approach in practice by implementing four different secure systems using \projecttitle{} ($\S$~\ref{sec:use_cases}). Specifically, we design and build a single-node trusted log system, an state-machine-replication (SMR) protocol, a chain replication system, and an accountability protocol that are fundamental building blocks in the cloud.
    %\item We formally verify the safety and security guarantees of our \projecttitle{} architecture from the bootstrapping process to the normal-operation network operations ($\S$~\ref{subsec::formal_verification_remote_attestation}).
%   
%    \item \pramod{this could be the concluding para of the intro before summarizing the contributions?} Lastly, we conduct an extensive evaluation of \projecttitle{} on real hardware ($\S$~\ref{sec:eval}). We evaluate \projecttitle{} against a competitive software-based network stack ($\S$~\ref{subsec:net_lib}). We further evaluate \projecttitle{} for practical systems: we compare our \projecttitle{}-based versions of our four implemented systems with their TEE-based implementations. To generalize our findings, we make use of two state-of-the-art TEEs, Intel SGX, and AMD-sev, showing that \projecttitle{} can improve the end-application performance up to $6\times$ w.r.t. when using TEEs.
    
\end{itemize}



==> backups/related_work.tex <==
\section{Related work}
%Several systems have attempted to improve the performance or the security properties of networked and distributed systems. We divide them into two categories: host-side trusted systems that make use of trusted components at the host level to improve systems' security and SmartNIC-based systems that take advantage of SmartNICs or programmable switch devices primarily for performance improvements.
% Several systems have attempted to improve the performance or the security properties of networked and distributed systems. We divide them into two categories: the host-side trusted systems that make use of trusted components at the host level to improve systems' security and the NIC-side systems that take advantage SmartNIC or programmable switch devices primarily for performance improvements.

\myparagraph{Trustworthy distributed systems} Prior research designed BFT systems in the context of replication protocols as in~\cite{Castro:2002, 10.1145/1658357.1658358, 199398, Suri_Payer_2021, DBLP:journals/corr/abs-1803-05069, Chan2018PaLaAS, DBLP:journals/corr/abs-1807-04938, Chan2018PiLiAE}. These systems usually have high complexity and performance overheads. \projecttitle{} on the other hand provides a generic trusted networking library to transform existing systems (under CFT) to BFT materializing a theoretical transformation with non-equivocation and transferable authentication properties that scale better than classical BFT.

\myparagraph{Trusted hardware for distributed systems} Prior systems~\cite{10.1145/3492321.3519568, minBFT, 10.1145/3552326.3587455, 10.1145/3492321.3519568} leverage trusted hardware, e.g., Intel SGX~\cite{intel-sgx}, SmartCards~\cite{levin2009trinc} and FPGAs~\cite{10.1145/2168836.2168866} to optimize for BFT systems. Their trusted components generate attestations similarly to \projecttitle{} although they report higher latencies than \projecttitle{} (e.g., 50us---105ms) due to their slow processing units~\cite{levin2009trinc} or communication costs between the host application and the trusted component~\cite{10.1145/2168836.2168866}. Our \projecttitle{} improves latency offloading the security properties at the NIC on the network data path. 

Other systems optimize~\cite{treaty, avocado, ccf} throughput by porting the entire network library and drivers within the TEE relying on SGX runtime freshness protection. Unfortunately, rollback protection is not available in all TEEs, e.g., AMD-sev in our evaluation does not offer that, while these systems build a large TCB with specific low-level code optimizations. Our \projecttitle{} offers a minimal, high-performant, TCB that is unified in all host machines. %Lastly, Trinc~\cite{levin2009trinc} and CheapBFT~\cite{10.1145/2168836.2168866} rely on peripherals to generate attestations, similarly to \projecttitle{}, with extremely expensive latencies. Our \projecttitle{} improves latencies as by principle it resides on the network data path in contrast to CheapBFT and it operates on faster frequencies compared to Trinc.

%To avoid distortion, our plots do not include Trinc~\cite{levin2009trinc} because its reported latencies are an order of magnitude slower (85-105 ms) than all other evaluated solutions.

%Lastly, recent work~\cite{10.1145/3552326.3587455} found safety violations in some optimized systems as minBFT~\cite{minBFT} on top of TEEs proving that equivocation can happens when the TEE is restarted. Our work does not suffer of such attacks because the physical isolation of FPGA renders rollback attacks to FPGA code impossible %\atsushi{I assume that the rollback attacks are a common issue for host-side trusted systems. I'd suggest we mention it in the last paragraph (as a separate paragraph) after introducing the individual systems.}. 

\myparagraph{SmartNIC-assisted systems} State-of-the-art networked systems are built on top of the emerging (programmable) SmartNIC devices~\cite{liquidIO_smartnics, u280_smartnics, bluefield_smartnics, broadcom_smartnics, netronome_smartnics, alibaba_smartnics, nitro_smartnics, msr_smartnics} for low-latency high-throughput network operations. Some systems~\cite{246498, 211249, 10.1145/3387514.3405895, 10.1145/3365609.3365851, 10.1145/3127479.3132252, 10.1145/2934872.2934897, 258971, 246486, 179716, 227655, 10.1145/3286062.3286068, shan2022supernic}  offload the network functions to the hardware optimizing the network latency while reducing the host processing overheads and energy costs. Others~\cite{10.1145/3341302.3342079, 10.1145/2872362.2872367, 234944, 9220629, 6853195, 10.1145/3477132.3483555, 280678, 10.1145/3132747.3132756, honeycomb} build generic execution frameworks that aim to optimize a wide variety of distributed systems. Our \projecttitle{} follows the trend and builds a high-performant, trusted, generic network stack for distributed systems on top of FPGA-based SmartNICs.

%Researchers also leverage FPGA-based SmartNICs to carefully offload (parts of) the business logic. Xenic~\cite{10.1145/3477132.3483555} and AlNiCo~\cite{280678} optimize transaction execution by intelligently utilizing FPGA-based SmartNICs to resolve conflicts and minimize contention. Similarly, KV-Direct~\cite{10.1145/3132747.3132756} and Honeycomb~\cite{honeycomb} accelerate KV operations by implementing a hybrid data structure co-designing between the host and SmartNIC. Similarly, \projecttitle{} leverages FPGAs, but it targets generality and minimalism. As such, our \projecttitle{} remains agnostic to the business logic and offloads to the hardware the minimal necessary processing for security guarantees. 
%\atsushi{The above two paragraphs can probably be merged because they mention studies using SmartNICs for performance/efficiency (not security). Please correct me if I'm wrong.}




\myparagraph{SmartNIC-assisted network stacks} Storm~\cite{storm}, Coyote~\cite{coyote}, Limago~\cite{8891991} and others~\cite{280712, 9114811} re-design and implement generic network stacks, i.e., RDMA and TCP/IP, for FPGA-based NICs. Our \projecttitle{} builds on top of such stacks and further extends their security semantics with the properties of non-equivocation and transferable authentication. %\atsushi{This paragraph can be moved to the bottom; I wanna prioritize the next paragraph that explains studies using SmartNICs for security. So, I'd suggest this part (SmartNIC-based systems) have three paragraphs in the following order: (1) SmartNICs for performance, (2) SmartNICs for security, (3) FPGA-based programmable NICs offering RDMA and/or TCP/IP, where TNIC can be built.}

%A classic line of work in distributed computing proposes stronger network models, such as atomic broadcast [12 , 32 ] and virtual synchrony [ 10 , 11 ], to simplify distributed
%system designs. These network primitives guarantee that a total order of messages are delivered to all broadcast receivers. However, atomic broadcast and virtual synchrony do not offer performance benefits to distributed systems – implementing them is equivalent to solving consensus [ 18 ]. NOPaxos [39 ] and Eris [ 38 ] pioneered a weaker network model in which messages are delivered in a consistent order, but reliable transmission is not guaranteed. This weaker
%model can be efficiently implemented using programmable switches. NOPaxos proposes an Ordered Unreliable Multicast primitive for state machine replication, while Eris designs a multi-sequenced groupcast primitive for distributed transactions. BIDL [ 46 ] uses sequencers to parallelize consensus and transaction execution in a permissioned blockchain system. However, BIDL still uses traditional BFT protocols for consensus and its sequencer design does
%not improve performance of the BFT protocol itself. The network sequencing approach has also been applied to other distributed system designs [ 7 , 8, 57 ]. Our aom primitive was inspired from these work, but additionally provides transferable authentication, a guarantee crucial for BFT protocols


\myparagraph{Programmable hardware for network security} NeoBFT~\cite{10.1145/3603269.3604874} leverages a programmable switch to offer BFT for permissioned (BFT) blockchain systems~\cite{10.1145/3190508.3190538}. It designs an Authenticated Ordered Multicast (AOM) primitive in the programmable switch hardware and uses an FPGA as a cryptographic co-processor to improve scalability bottlenecks. Our \projecttitle{} is not orthogonal to NeoBFT but it differs in two aspects. First, it offers generality expanding the scope of BFT properties beyond the blockchain domain to general distributed systems. Secondly, it does not rely on a centralized switch for ordering but follows a decentralizing approach requiring each machine to be connected to a \projecttitle{}. In contrast to NeoBFT, the switch is not a single point of failure at the cost of some extra hardware.

Helios~\cite{10.1145/3620678.3624786} and others~\cite{10.1145/3563647.3563654, 10.1145/3321408.3323087} build on top of an ASIC-based SmartNICs and programmable switches to offer security but they target different threat models (e.g., access control, lateral movements between compromised containers, DNS traffic inspection, security functions offloading) from \projecttitle{}.


%\myparagraph{Host-side trusted systems} There has been a lot of work that builds trusted and secure systems on top of CPU-based trusted hardware such as TEEs. Particularly, several systems have designed external trusted services on top of TEEs that run independently as a separate process with the distributed application to generate and verify authenticated network messages~\cite{10.1145/3492321.3519568, minBFT}. These systems require an extra communication step between the untrusted application code and the trusted service, which has been reported to dominate the operations latency~\cite{10.1145/2168836.2168866}. In contrast, our \projecttitle{} offers on the communication path direct processing, optimizing the latency of the system. Importantly, recent work~\cite{10.1145/3552326.3587455} reports that the system can possibly equivocate and violate safety under rollback attacks. Our work does not suffer because the physical isolation of FPGA renders rollback attacks to FPGA code impossible \atsushi{I assume that the rollback attacks are a common issue for host-side trusted systems. I'd suggest we mention it in the last paragraph (as a separate paragraph) after introducing the individual systems.}. Other systems optimize the communication latency by porting the entire network library within the TEE~\cite{treaty, avocado, ccf}. Unfortunately, this leads to a huge TCB and requires low-level and very specific code optimizations which cannot be generalized for a variety of distributed systems. Lastly, Trinc~\cite{levin2009trinc} and CheapBFT~\cite{10.1145/2168836.2168866} rely on peripherals to generate and validate the attested messages with extremely expensive latencies \atsushi{Can we explain if TNIC avoids such latency increases, and how?}. 
%To avoid distortion, our plots do not include Trinc~\cite{levin2009trinc} because its reported latencies are an order of magnitude slower (85-105 ms) than all other evaluated solutions.

%\atsushi{Can we also write a one-sentence conclusion that highlights the advantage of TNIC to the systems mentioned above?}

%Trinc: SmartCards~\cite{levin2009trinc}\\
%CheapBFT: FPGA~\cite{10.1145/2168836.2168866}\\
%Trusted network stack: ~\cite{treaty, avocado} -> HUGE TCB\\
%Trusted message signing service:~\cite{10.1145/3492321.3519568, minBFT}



%\myparagraph{SmartNIC-based systems} A large body of research presented systems on top of the emerging (programmable) SmartNIC devices to optimize various systems. Some systems~\cite{246498, 211249, 10.1145/3387514.3405895, 10.1145/3365609.3365851, 10.1145/3127479.3132252, 10.1145/2934872.2934897, 258971, 246486, 179716, 227655, 10.1145/3286062.3286068, shan2022supernic}  offload the network functions improving the network latencies and reducing the host processing overheads and energy costs. Others~\cite{10.1145/3341302.3342079, 10.1145/2872362.2872367, 234944, 9220629, 6853195} have designed generic frameworks on top of the SmartNIC devices to optimize a wide variety of distributed systems.

%Researchers also leverage FPGA-based SmartNICs to carefully offload (parts of) the business logic. Xenic~\cite{10.1145/3477132.3483555} and AlNiCo~\cite{280678} optimize transaction execution by intelligently utilizing FPGA-based SmartNICs to resolve conflicts and minimize contention. Similarly, KV-Direct~\cite{10.1145/3132747.3132756} and Honeycomb~\cite{honeycomb} accelerate KV operations by implementing a hybrid data structure co-designing between the host and SmartNIC. Similarly, \projecttitle{} leverages FPGAs, but it targets generality and minimalism. As such, our \projecttitle{} remains agnostic to the business logic and offloads to the hardware the minimal necessary processing for security guarantees. 
%\atsushi{The above two paragraphs can probably be merged because they mention studies using SmartNICs for performance/efficiency (not security). Please correct me if I'm wrong.}

%Storm~\cite{storm}, Coyote~\cite{coyote}, Limago~\cite{8891991} and others~\cite{280712, 9114811} re-design and implement generic network stacks, i.e., RDMA and TCP/IP, for FPGA-based NICs. Our \projecttitle{} builds on top of such stacks and further extends their security semantics with the properties of non-equivocation and transferable authentication. \atsushi{This paragraph can be moved to the bottom; I wanna prioritize the next paragraph that explains studies using SmartNICs for security. So, I'd suggest this part (SmartNIC-based systems) have three paragraphs in the following order: (1) SmartNICs for performance, (2) SmartNICs for security, (3) FPGA-based programmable NICs offering RDMA and/or TCP/IP, where TNIC can be built.}

%NeoBFT~\cite{10.1145/3603269.3604874} and Helios~\cite{10.1145/3620678.3624786} leverage programmable NIC devices to offer security. NeoBFT~\cite{10.1145/3603269.3604874} targets the BFT model for permissioned (BFT) blockchain systems~\cite{10.1145/3190508.3190538} by designing an Authenticated Ordered Multicast (AOM) primitive in the programmable switch. To overcome the computation and scalability bottlenecks, they connect to the switch an FPGA device that serves as a cryptographic coprocessor. Our \projecttitle{} is orthogonal to NeoBFT in two aspects. First, it expands the scope of BFT properties in generic distributed systems, including blockchain systems. Secondly, it does not rely on a centralized switch for ordering, but each participating machine is connected to each own \projecttitle{} instance. Helios~\cite{10.1145/3620678.3624786} builds on top of an ASIC-based SmartNIC targeting a different threat model from \projecttitle{}. In particular, Helios targets adversaries that are able to conduct network-based attacks and enable lateral movement from a compromised container to other containers, gaining control over the compromised containers.

%extends RDMA primitives to enable remote direct key-value
%access to the main host memory. Honeycomb~\cite{honeycomb} designs an hardware-accelarated B-tree within the FPGA to accelarate KV operations.

%KV stores co-design~\cite{ 10.1145/3093337.3037731,  9912712}\\
%Network stacks on FPGA~\cite{storm, coyote, 8891991, 280712, 9114811}\\
%Security-based SmartNICs: BFT-concensus->NeoBFT~\cite{} and Helios~\cite{}\\








==> backups/t-nic-hardware-before-cut.tex <==
\begin{figure}[t!]
    \centering
    %\includegraphics[width=.27\textwidth]{figures/trusted-nic-single-node-overview.drawio-1.pdf}
    %\includegraphics[width=0.45\textwidth]{figures/hw-implementation.drawio.pdf}
    %\caption{\projecttitle{} hardware architecture.}
     \includegraphics[width=0.8\linewidth]{figures/hardware-implementation-colored.drawio.pdf}
    \caption{\projecttitle{} hardware architecture.}
     \label{fig:hardware-design}
\end{figure}


\section{Trusted NIC Hardware}
\label{sec:t-nic-hardware}



Figure~\ref{fig:hardware-design} shows our \projecttitle{} hardware architecture that implements trusted network operations on a SmartNIC device. In this section, we introduce two key components: \emph{(i)} the attestation kernel that guarantees the non-equivocation and transferable authentication properties over the untrusted network ($\S$~\ref{subsec:nic_attest_kernel}) and \emph{(ii)} the RoCE protocol kernel that implements the RDMA protocol including transport and network layers ($\S$~\ref{subsec:roce_protocol_kernel}). We also introduce a remote attestation and initialization protocol for \projecttitle{} ($\S$~\ref{subsec:nic_controller}) and formally verify them ($\S$~\ref{subsec::formal_verification_remote_attestation}).
% Lastly, we design a remote attestation protocol for our \projecttitle{} based on the \projecttitle{} Controller module that we discuss $\S$~\ref{subsec:nic_controller}. Importantly, we formally verify \projecttitle{}'s remote attestation and initialization protocol ($\S$~\ref{subsec::formal_verification_remote_attestation}).

\subsection{NIC Attestation Kernel}
\label{subsec:nic_attest_kernel}
\myparagraph{Overview} 
The attestation kernel {\em shields} network messages and materializes the properties of non-equivocation and transferable authentication by generating {\em attestations} for transmitted messages. As shown in Figure~\ref{fig:hardware-design}, the attestation kernel resides in the data pipeline between the RoCE protocol kernel that transmits/receives network messages and the PCIe/Local DMAs that transfer data from/to the host and local memories.
The kernel processes the messages as they {\em flow} from the memory to the network and vice versa to optimize throughput. 
% The module resides in the data pipeline between the RoCE protocol kernel that transmits/receives network messages and the PCIe DMA which fetches and pushes data {\em asynchronously} from the host memory to the FPGA memory.

\myparagraph{Hardware design} The attestation kernel is comprised of three components that represent its state and functionality: the HMAC component that generates the message authentication codes (MAC), the Keystore which stores the keys used by the HMAC module, and the Counters store that keeps the messages latest sent and received timestamp. 

Each \projecttitle{} device is initialized from the Protocol Designer during bootstrapping ($\S$~\ref{subsec:nic_controller}) with a unique identifier (ID) and some shared secret keys---ideally, one shared key for each session, which is stored in static memory (Keystore). The keys are shared and, hence, not known to the untrusted parties. 



\projecttitle{} holds two counters per session in the Counters store: {\tt send\_cnts} to be used for sending messages, and \texttt{recv\_cnts} that holds the latest seen counter value for each session. The counters represent the messages' timestamp and are increased monotonically and deterministically after every send and receive operation to ensure that unique messages are assigned to unique counters for non-equivocation. Consequently, no messages can be lost, re-ordered, or doubly executed.



\begin{algorithm}[t]
\SetAlgoLined
\small
\textbf{function} \texttt{Attest(c\_id, msg)} \{ \\
\Indp
{\tt cnt} $\leftarrow$ {\tt send\_cnts[c\_id]++};\\
$\alpha$ $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)}; \\
\textbf{return} $\alpha${\tt ||msg||cnt};\\
\Indm
\} \\

%\vspace{0.3cm}

\textbf{function} \texttt{Verify(c\_id, $\alpha$||msg||cnt)} \{ \\
\Indp
    $\alpha$' $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)};\\
    \textbf{if} {\tt (}$\alpha$' $=$ $\alpha$ {\tt \&\&} {\tt cnt} $=$ {\tt recv\_cnts[c\_id]++} {\tt )}\\
    \Indp
        \textbf{return} ($\alpha${\tt ||msg||cnt)}; \\
    \Indm
    \textbf{assert(False)}; \\
\Indm
\} \\
%\vspace{0.1cm}
\vspace{-1pt}
\caption{\texttt{Attest()} and \texttt{Verify()} functions.}
\label{algo:primitives}
\end{algorithm}



\myparagraph{Algorithm} 
Algorithm~\ref{algo:primitives} shows the functionality of the attestation kernel. The module implements two core functions: {\tt Attest()} which generates a unique and verifiable attestation for a message and {\tt Verify()} which verifies the attestation of a received message. The message transmission invokes {\tt Attest()}, and likewise, the reception invokes {\tt Verify()}. 
% When an application transmits a message, the message is attested by {\tt Attest()}. Likewise, upon a message reception, the message is verified with {\tt Verify()} before it is copied to the application's (host) memory. 
% Algorithm~\ref{algo:primitives} shows the functionality of the attestation kernel. The module implements two core functions: the {\tt Attest} function which generates a unique and verifiable attestation for a message and the {\tt Verify} function which verifies the attestation of a received message. When the application transmits a message, the data flow passes through the {\tt Attest} function, and upon a message reception, the message is verified (with {\tt Verify} function) before it is copied to the application's (host) memory. 

% The metadata and the request opcode pass through the control path from the host to the device and vice versa \atsushi{What's the metadata here?}. On the other hand, 
Upon transmission, as shown in Figure~\ref{fig:hardware-design}, the message is first forwarded to the attestation kernel, and then, the output is forwarded to the RoCE protocol kernel. 
% the message data passes from the application layer to \projecttitle{} through the data path. 
The attestation kernel upon transmission executes \texttt{Attest()} and generates an {\em attested} message comprised of the message data and its attestation certificate~$\alpha$. The function calculates $\alpha$ as the HMAC of the message concatenated with the counter {\tt send\_cnt} using the {\tt key} for that connection (Algorithm~\ref{algo:primitives}:~L3). It also increases the next available counter for subsequent future messages (Algorithm~\ref{algo:primitives}:~L2). The function forwards the original message with $\alpha$ to the RoCE protocol (Algorithm~\ref{algo:primitives}:~L4).
% As shown in Figure~\ref{fig:hardware-design}, a request passes from the application layer to the \projecttitle{} through two separate paths, i.e., the data and control paths. The metadata and the request opcode pass through the control path from the host to the device and vice versa. On the other hand, the message data is first forwarded to the attestation kernel, and then, the output is forwarded to the RoCE protocol kernel. The attestation kernel upon transmission executes the \texttt{Attest} function and generates an {\em attested} message comprised of the message data and its attestation certificate, or simply attestation $\alpha$. The function calculates $\alpha$ as the HMAC of the message concatenated with the counter {\tt send\_cnt} using the {\tt key} for that connection (Algorithm~\ref{algo:primitives}:~L3). It also increases the next available counter for subsequent future messages (Algorithm~\ref{algo:primitives}:~L2). The function forwards to the RoCE protocol the original message along with $\alpha$ for transmission (Algorithm~\ref{algo:primitives}:~L4).

Upon reception, the received message passes through the attestation kernel for verification before it is delivered to the application. Specifically, \texttt{Verify()} checks the authenticity and the integrity of the received message by re-calculating the {\em expected} attestation $\alpha$' based on the message payload and comparing it with the received attestation $\alpha$ of the message (Algorithm~\ref{algo:primitives}:~L7---8). Following that, the verification also ensures that the received counter matches the expected counter for that connection to ensure \emph{continuity} (Algorithm~\ref{algo:primitives}:~L8). 



\subsection{RoCE Protocol Kernel}
\label{subsec:roce_protocol_kernel}

\myparagraph{Overview} 
The RoCE protocol kernel implements a reliable transport service on top of the IB Transport Protocol with UDP/IPv4 layers (RoCE v2)~\cite{infiniband} (transport and network layers). As shown in Figure~\ref{fig:hardware-design}, to send data at the transmission path, the {\tt Req handler} module in the RoCE kernel receives the request opcode ({\tt metadata}) issued by the host. The message is then fetched through the PCIe DMA engine and passes through the attestation kernel. The request opcode and the attested message are forwarded to the {\tt Request generation} module that constructs a network packet. 
% The RoCE protocol kernel implements a reliable transport service on top of the IB Transport Protocol with UDP/IPv4 layers (RoCE v2)~\cite{infiniband} (transport and network layers), and it is connected to the attestation kernel as discussed in $\S$~\ref{subsec:nic_attest_kernel}. As shown in Figure~\ref{fig:hardware-design}, to send data at the transmission path, the {\tt Req handler} module in the RoCE kernel receives the request opcode (metadata) issued by the host. The message to be sent is then fetched through the PCie DMA engine and passes through the attestation kernel for processing. The request opcode and the attested message are forwarded to the {\tt Request generation} module that constructs the network packet. 

Upon receiving a message from the network, the RoCE kernel parses the packet header and updates the protocol state (stored in the State tables). The attested message is then forwarded to the attestation kernel. Upon successful verification, the message is delivered to the application's (host) memory. 

\myparagraph{Hardware design} The RoCE protocol kernel is additionally connected to a 100Gb MAC IP and an ARP server IP. 

\noindent{\underline{100Gb MAC.}} The 100Gb MAC kernel implements the link layer connecting \projecttitle{} to the network fabric over a 100G Ethernet Subsystem~\cite{license}. The kernel also exposes two interfaces to the RoCE protocol kernel for transmitting (Tx) and receiving (Rx) network packets. 

\noindent{\underline{ARP server.}} 
The ARP server contains a lookup table with the correspondences between MAC and IP addresses. Right before the transmission, the RDMA packets at the {\tt Request generation} first pass through an MAC and IP encoding phase, where the {\tt Request generation} module extracts the remote MAC address from the lookup table in the ARP server.
% The ARP server contains a lookup table with the correspondences between MAC and IP addresses. Right before the transmission, the RDMA packets at the {\tt Request generation} first pass through a MAC and IP encoding phase. At this encoding phase, the {\tt Request generation} module extracts from the lookup (ARP table) in the ARP server the remote MAC address.

\noindent{\underline{IB protocol.}} 
The RoCE protocol kernel implements the reliable version of the IB protocol. Similarly to its original specification~\cite{rdma_specification}, the kernel implements State tables to store protocol queues (e.g., receive/send/completion queues). The State tables also store important metadata such as packet sequence numbers (PSNs), message sequence numbers (MSNs), and a Retransmission Timer. % to detect packet losses.
% The RoCE protocol kernel implements the reliable version of the IB protocol. Similarly to its original specification~\cite{rdma_specification}, the kernel implements the State tables to store the protocol queues QPs (i.e., receive queue, send queue, completion queue, etc.). The State tables also store important metadata such as (1) the packet sequence numbers (PSNs) to distinguish valid, invalid, and duplicate PSN regions, (2) the message sequence numbers (MSNs) to reconstruct fragmented network messages, and (3) a Retransmission Timer to detect packet losses.

\myparagraph{Dataflow}
The transmission path is shown with the blue-colored axes in Figure~\ref{fig:hardware-design}. The {\tt Req handler} receives requests issued by the host and initializes a DMA command to fetch the payload data from the host memory to the attestation kernel. Once the attestation kernel forwards the attested message to the {\tt Req handler}, the module passes the message from several states to append the appropriate headers {\tt IB hdr} along with metadata (e.g., RDMA op-code, the PSN and the QP number, etc.). The last part of the processing generates and appends UDP/IP headers (e.g., IP address, UDP port, and packet length). The message is then forwarded to the CMAC module. 

Similarly, the reception path is shown with the red-colored axes in Figure~\ref{fig:hardware-design}. The {\tt Request decoder} extracts the headers, metadata, and attested message. The message is forwarded to the attestation kernel for verification and finally copied to the host memory.

% \myparagraph{{Message format:}} The IB protocol in \projecttitle{} processes the following headers: IP, UDP, BTH (Base Transport Header), RETH (RDMA Extended Transport Header), and AETH (ACK Extended Transport Header) as defined in the RDMA Protocol Specification~\cite{rdma_specification, storm}.  The RoCE kernel adds the Ethernet header (L2 header), the IPv4/UDP headers (L3 headers), and the IB headers (L4 headers). It also adds a 32b end-to-end CRC (ICRC) that covers all invariant fields of the packet and offers protection beyond the coverage of the Ethernet Frame Checksum (FCS). 
The message format in \projecttitle{} follows the original RDMA specification~\cite{rdma_specification}; only the difference between our \projecttitle{} and the original RDMA messages is that the attestation kernel {\em extends} the payload by appending a 64B attestation $\alpha$ and the metadata. The metadata includes a 4B id for the session id of the sender, a 4B id for the device id (unique per device), and the appropriate {\tt send\_cnt}. This payload extension is negligible and does not harm the network throughput.  
% \atsushi{Can we say something positive: e.g., the RoCE protocol kernel does not need to be aware of this difference, or its extension doesn't badly affect the performance, etc.}\dimitra{Both are true, feel free to write in-place}

\begin{figure}[t!]
    \centering
    \includegraphics[width=.35\textwidth]{figures/remote_attestation.drawio.pdf}
    \caption{\projecttitle{} remote attestation protocol.}
    \label{fig:remote_attestation}
\end{figure}

\subsection{Remote Attestation Protocol} 
\label{subsec:nic_controller}
We design a remote attestation protocol for the \projecttitle{} to ensure that the \projecttitle{} device is genuine and the \projecttitle{} bitstream is flashed securely in the device along with the designer's configuration data (IPs, secrets, etc.).

\myparagraph{Design assumptions} We base our design for the remote attestation protocol on a NIC Controller, a hardware component that drives the device initialization as in~\cite{10.1145/3503222.3507733}. The Controller can be implemented as a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733} with no access to confidential information. After the initialization process, the Controller monitors JTAG/ICAP interfaces to ensure that the bitstream is not modified before use and prevent physical attacks as commercial IPs~\cite{secMon}.

\myparagraph{Boostrapping} We next describe the bootstrapping phase of the device in \projecttitle{}. At the manufacturing construction, the Manufacturer burns a secret device key \texttt{HW$_{key}$} that is unique to the device~\cite{secure_FPGAs}. At the \projecttitle{} initialization, the Protocol designer instructs the cloud provider to load the (encrypted) FPGA firmware from the storage medium using the embedded code in the BootROM device. The firmware is then decrypted using the \texttt{HW$_{key}$}. The firmware loads the controller binary \texttt{Ctrl$_{bin}$}, generates a key pair \texttt{Ctrl$_{pub, priv}$} that is bound to the specific device and binary, and lastly, generates and signs the measurement of the \texttt{Ctrl$_{bin}$} producing \texttt{Ctrl$_{bin}$cert}. The Protocol designer then establishes a TLS/SSL connection with the trusted IP vendor and sends the list of the participating machines and any configuration data. 

\myparagraph{Remote attestation} 
We describe the remote attestation protocol shown in Figure~\ref{fig:remote_attestation}. First of all, the IP vendor and the Controller also establish a secure communication channel. The IP vendor generates a random nonce \texttt{n} for freshness and an asymmetric key pair \texttt{V$_{pub, priv}$} and sends the \texttt{n} and the public key \texttt{V}$_{pub}$ to the Controller. The Controller uses the \texttt{V}$_{pub}$ and his own \texttt{Ctrl}$_{priv}$ to perform Diffie–Hellman key exchange with the vendor and establish a shared secret key \texttt{S$_{key}$} (1).
% which allows them from now on to securely communicate over insecure channels (8).
% The IP vendor and the Controller also establish a secure communication channel. The IP vendor generates a random nonce \texttt{n} for freshness and an asymmetric key pair, \texttt{V$_{pub, priv}$} for secure communication with the Controller, and sends the \texttt{n} and the public key \texttt{V}$_{pub}$ to the Controller (7). The Controller uses the \texttt{Vendor}$_{pub}$ and his own \texttt{Controller}$_{priv}$ to perform Diffie–Hellman key exchange with the vendor and establish a shared secret key \texttt{S$_{key}$} which allows them from now on to securely communicate over insecure channels (8).

The Controller is now ready to execute the remote attestation. First, it receives the encrypted bitstream \projecttitle{}$_{enc}$ from the vendor (2) and computes its measurement \texttt{h} (3). Next, it generates an attestation report \texttt{m} that contains the following data: the nonce \texttt{n}, the \texttt{h}, the \texttt{Ctrl$_{pub}$}, the measurement of the \texttt{Ctrl$_{bin}$} \texttt{H(Ctrl$_{bin}$)}, and its signature \texttt{Ctrl$_{bin}$cert} (4). The Controller signs the \texttt{m} with its private key \texttt{Ctrl$_{priv}$} and sends the attestation report to the vendor (5).

The IP vendor verifies the authenticity of the attestation report by completing the remote attestation process (6)---(8). First, the vendor verifies the authenticity of the attestation report m with the \texttt{Ctrl$_{pub}$} to verify that a genuine \texttt{Ctrl$_{bin}$} has signed \texttt{m} (6). Afterward, the vendor ensures that the \texttt{Ctrl$_{bin}$} runs in a genuine \projecttitle{} device by verifying that the measurement of the \texttt{Ctrl$_{bin}$} has been signed with an appropriate device key that has been installed by the Manufacturer (7). Lastly, the vendor verifies the nonce \texttt{n} for freshness and that the \texttt{h}, the measurement of \projecttitle{}$_{enc}$, is as expected (8). 
% Upon a successful attestation, it shares the vendor encryption key \texttt{VE$_{key}$} with the Controller (16). 

When all the verifications pass successfully, the remote attestation is completed. The IP vendor securely shares the vendor encryption key \texttt{VE$_{key}$} with the Controller by encrypting it with the previously established shared secret key \texttt{S$_{key}$} (9). The Controller decrypts the \projecttitle{} bitstream and loads it onto the FPGA (10). 
% Similarly, the vendor shares any configuration data. 
Finally, the IP vendor notifies the Protocol designer about the result of the remote attestation.


\subsection{Formal Verification of \projecttitle{} Protocols}
\label{subsec::formal_verification_remote_attestation}

% \pramod{Please tie to the high-level properties (tranferrable authentication and non-equivocation) of TNIC and then map it down to low-level TNIC protocols.}

We formally verify the security and safety properties of \projecttitle{} hardware. First, we verify the bootstrapping and the remote attestation protocol of \projecttitle{}. This provides a formal model used to argue about non-equivocation and transferable authentication. We use Tamarin~\cite{tamarin-prover}, a security protocol verification tool that analyzes symbolic models of protocols specified as multiset rewriting systems. We next present the verified security properties of \projecttitle{}, proofs are available in Appendix~\ref{sec:formal-verification-details}. 

% This model imposes the following assumptions: \emph{(i)}~all messages are composed of atomic terms using predefined functions \dimitra{What does that mean :) ?}\julian{I will update this but to quickly answer: tamarin does not consider individual bits, but instead works with more abstract terms like 'keys', 'hashes' and treats them as atomic, i.e. it is impossible to decompose them into individual parts/bits. Hence there is also only a set of defined functions \& equations to manipulate those terms, e.g. dec(enc(m)) = m, but functions that e.g. reverse the byte order of the bits or something similar, are not considered when evaluating what an attacker can do. This is usually fine because they do not change security on the high level we have here, but it would e.g. be less suited to analyzed low level cryptographic operations. In such cases you might want to also analyze the crypto functions you are using etc.} \emph{(ii)}~these cryptographic functions are perfect with no side-effects \dimitra{are not compromised?} \julian{That is one implication, another one is that e.g. hash functions do not produce hash collisions or that you can't extract key information from side channels etc. It's just that in reality any cryptographic primitive can be broken with some probability (usually very small) and tamarin assumes it to be impossible. This is so it tamarin is able to generate true/false statements about security properties. The alternative would be considering all the probabilities of breaking idividual crypto functions and composing them to obtain a overall probability of breaking a  security property. This is possible using a cryptographic model (e.g. using CryptoVerif) but more complex and generally more restrictive in what you can show.} \emph{(iii)}~attackers can read and delete all messages that are sent on the network and modify them in accordance with the set of available functions.



% Our verification work relies on properties of the already analyzed TLS handshake~\cite{tamarin_tls_proof} and proofs the desired security properties of the \projecttitle{} bootstrapping and attestation protocol.  The desired properties are modeled as lemmas that define valid and invalid system states. Tamarin then verifies the specified lemmas, by \emph{(i)} finding at least one trace  (series of state transitions) for the valid control states and \emph{(ii)} showing that there exists no trace leading to invalid states.

\myparagraph{Remote attestation}  We model the bootstrapping and remote attestation protocols as described in Figure~\ref{fig:remote_attestation}. We define multiple lemmas to ensure the secrecy of the private information involved in the protocol as well as the main attestation lemma which holds if and only if: once the last step of the remote attestation protocol is completed, the \projecttitle{} device is in a valid, expected state. 

\myparagraph{Transferable authentication} 
% We extend the analysis of the bootstrapping and attestation protocol in Tamarin with models for the network operations that upon the message transmission and reception execute the {\tt Attest} and {\tt Verify} functions (Algorithm~\ref{algo:primitives}), respectively. In simple words we prove that  \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages will never be assigned identical message sequencers ({\tt send\_cnts}) and secondly, the transferable authentication is met because each generated attestation is uniquely verified by the secret keys jointly with the unique sender's \projecttitle{} device identifier.
We extend the model with rules for the network operations that upon the message transmission and reception execute the {\tt Attest} and {\tt Verify} functions (Algorithm~\ref{algo:primitives}), respectively. This allows us to reason about transferable authentication by defining the following additional lemma: Any message that is accepted was sent by an authentic \projecttitle{} device in a valid configuration.

% In simple words we prove that  \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages will never be assigned identical message sequencers ({\tt send\_cnts}) and secondly, the transferable authentication is met because each generated attestation is uniquely verified by the secret keys jointly with the unique sender's \projecttitle{} device identifier.

% Formally, we define one additional lemma to help reason about the transferable authentication: \emph{(i)} this message was sent by an authentic \projecttitle{} device in a valid configuration \emph{(ii)} there is no message that was sent before, but not accepted \emph{(iii)} there is no message that was sent after, but accepted before this one \emph{(iii)} this message has not been accepted before.


\myparagraph{Non-equivocation} The model is further extended by three lemmas that help to reason about non-equivocation: For any message that is accepted it holds that \emph{(i)} there is no message that was sent before, but not accepted \emph{(ii)} there is no message that was sent after, but accepted before this one \emph{(ii)} this message has not been accepted before.

For this model, Tamarin successfully shows that there is no sequence of transitions that leads to any state where our lemmas are violated. Thus, the attestation and transferable authentication lemmas hold for our model, and the counters behave as expected to ensure non-equivocation.

==> backups/t-nic-hardware.bak.tex <==
\section{Trusted NIC Hardware}
\label{sec:t-nic-hardware}

Figure~\ref{fig:tfpga} shows our \projecttitle{} hardware implementation that implements trusted network operations on the SmartNIC device. \projecttitle{} is comprised of three hardware components: \emph{(i)} the attestation kernel that guarantees the non-equivocation and transferable authentication properties over the untrusted network ($\S$~\ref{subsec:nic_attest_kernel}), \emph{(ii)} the RoCE protocol kernel that implements the RDMA protocol on the FPGA including the transport and network layers ($\S$~\ref{subsec:roce_protocol_kernel}),  and \emph{(iii)} the NIC Controller which performs the remote attestation and initialization of the device ($\S$~\ref{subsec:nic_controller}). Importantly, we formally verify \projecttitle{}'s remote attestation and initialization protocol ($\S$~\ref{subsec::formal_verification_remote_attestation}).

%securely bootstraps the device and flushes the bitstream. % initializes the device, offers remote attestation to ensure the authenticity of the device and the flushed bitstream and guarantees run-time isolation.



% PUT THIS IN OVERVIEW To prevent equivocation and guarantee the validity of the network traffic, we require each node that participates in a distributed protocol to be equipped with a \trustedfpga{} subsystem. Each \trustedfpga{} is configured by the developer at the initialization with a secret (asymmetric) key, and it is uniquely identified by an identifier that corresponds to the node that hosts the subsystem.

%The secret key is private, whereas the public key is exposed to the application layer. Apart from the private key, the internal state of the \trustedfpga{} and the algorithm used to authenticate messages may be known publicly. %The private keys are generated and installed to each \trustedfpga{} during initialization.
%For now, we assume that the secret key is manually
%installed before system startup. In a future version, every
%CASH subsystem would maintain a private key and expose
%the corresponding public key. A shared secret key for every
%protocol instance may be generated during initialization, encrypted under the public key of every subsystem, and trans-
%ported securely to every replica.

\begin{algorithm}
\SetAlgoLined
\small
\textbf{function} \texttt{Attest(c\_id, msg)} \{ \\
\Indp
{\tt cnt} $\leftarrow$ {\tt send\_cnts[c\_id]++};\\
$\alpha$ $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)}; \\
\textbf{return} $\alpha${\tt ||msg||cnt};\\
\Indm
\} \\


\vspace{0.3cm}

\textbf{function} \texttt{Verify(c\_id, $\alpha$||msg||cnt)} \{ \\
\Indp
    $\alpha$' $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)};\\
    \textbf{if} {\tt (}$\alpha$' $=$ $\alpha$ {\tt \&\&} {\tt cnt} $=$ {\tt recv\_cnts[c\_id]++} {\tt )}\\
    \Indp
        \textbf{return} ($\alpha${\tt ||msg||cnt)}; \\
    \Indm
    \textbf{assert(False)}; \\
\Indm
\} \\
%\vspace{0.1cm}
\vspace{-1pt}
\caption{\texttt{Attest()} and \texttt{Verify()} functions.}
\label{algo:primitives}
\end{algorithm}

\if 0
\begin{center}
\begin{table}[ht]
\small
\centering
\begin{tabular}{ |m{2cm}||m{5.6cm}|}
 \hline
 {\tt ID} & A unique ID for this \projecttitle{} instance. \\
 {\tt keys[]} & (shared) Keys network sessions. \\
 {\tt send\_cnts[]} & Current counters values on transmission path per session.\\
 {\tt recv\_cnts[]} & Current counters values on reception path per session.\\
 \hline
 \end{tabular}
\caption{Attestation kernel state.}
\label{table:api}
\end{table}
\end{center}
\fi 

\subsection{NIC Attestation Kernel}
\label{subsec:nic_attest_kernel}
\myparagraph{Overview} The attestation kernel {\em shields} the network messages and materializes the properties of non-equivocation and transferable authentication by generating {\em attestations} for the transmitted messages. As shown in Figure~\ref{fig:tfpga}, the attestation kernel is pipelined on-the data path, processing the messages as they {\em flow} from host memory to the device and vice versa to optimize for throughput. The module resides in the data pipeline between the RoCE protocol kernel that transmits/receives the network messages and the XDMA engine which fetches and pushes data {\em asynchronously} from the host memory to the FPGA memory.

%{\noindent \underline{Attestation kernel state.}} 
\myparagraph{System state} \atsushi{Architecture, or Hardware design?} The attestation kernel is comprised of three components that represent its state and functionality: the HMAC component that generates the message authentication codes (MAC), the Keystore which stores the keys used by the HMAC module, and the Counters store that keeps the messages latest sent and received timestamp. 

%Table~\ref{table:api} summarizes the internal state of the attestation kernel (per device). 
Each \projecttitle{} device is initialized from the Protocol Designer during bootstrapping ($\S$~\ref{subsec:nic_controller}) with a unique identifier (ID) and some shared secret keys---ideally, one shared key for each session, which is stored in static memory (Keystore). The keys are shared and, hence, not known to the untrusted parties. % and as such even local (single-node) attestations always need pass through the \projecttitle{}. 

The \projecttitle{} also holds two counters per session stored in the Counters store (Figure~\ref{fig:tfpga}), the {\tt send\_cnts} to be used for sending messages and the \texttt{recv\_cnts} that holds the latest seen counter value for each session. The counters represent the messages' timestamp and are increased monotonically and deterministically after every send and receive operation to ensure that unique messages will be assigned to unique counters (for non-equivocation) and consequently, no messages can be lost, re-ordered, or doubly-executed.




\myparagraph{Design} \atsushi{Not design, maybe just Algorithm?} \atsushi{These paragraphs are a bit beefy} Algorithm~\ref{algo:primitives} shows the design of the attestation kernel. The module implements two core functions: the {\tt Attest} function which generates a unique and verifiable attestation for a message and the {\tt Verify} function which verifies the attestation of a received message. When the application transmits a message, the data flow passes through the {\tt Attest} function and upon a message reception, the message is verified (with {\tt Verify} function) before it is copied to the application's (host) memory. 

As shown in Figure~\ref{fig:tfpga}, a request passes from the application layer to the \projecttitle{} through two separate paths. The metadata and the request opcode (illustrated with dashed lines) pass through the control path from the host to the device and vice versa. On the other hand, the message data wires are first connected to the attestation kernel and then, the output is forwarded to the RoCE protocol kernel. The attestation kernel upon transmission executes the \texttt{Attest} function and generates an {\em attested} message comprised of the message data and its attestation certificate, or simply attestation $\alpha$. The function calculates $\alpha$ as the HMAC of the message concatenated with the counter {\tt send\_cnt} using the {\tt key} for that connection (Algorithm~\ref{algo:primitives}:~L3). It also increases the next available counter for subsequent future messages (Algorithm~\ref{algo:primitives}:~L2). The function forwards to the RoCe protocol the original message along with $\alpha$ for transmission (Algorithm~\ref{algo:primitives}:~L4).

%where the control flow forwards the request for \emph{increment} (\circled{1c}) and also fetches the corresponding sequencer \texttt{<mc\_id, v, cnt>} from the \emph{mc ids index} (\circled{1a}, \circled{1b}). After the increment the producing message is of the form \texttt{<sequencer, msg>} which is now being signed with the node's private key following the same workflow (\circled{2a}, \circled{2b}, \circled{2c}). The signed message \texttt{<(header, h(msg))$\sigma$, msg>}  can be logged (for recoverability) and is now forwarded to the network stack for transmission.

%{\noindent \underline{Verify path.}} 
Upon reception, the received message passes through the attestation kernel for verification before it is delivered to the application. Specifically, the \texttt{Verify} function checks the authenticity and the integrity of the received message by re-calculating the {\em expected} attestation ($\alpha$') based on the message payload and comparing it with the received attestation ($\alpha$) of the message (Algorithm~\ref{algo:primitives}:~L7---8). Following that, the verification also ensures that the received counter matches the expected counter for that connection to ensure \emph{continuity} (Algorithm~\ref{algo:primitives}:~L8). 

\myparagraph{Security analysis} This simple attestation kernel achieves to ensure the properties of non-equivocation and transferable authentication. First, \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages
will never be assigned identical {\tt send\_cnts}. The property is ensured because the {\tt send\_cnts} are never decremented. Secondly the \projecttitle{} ensures the transferable authentication because the cryptosystem is not broken, the keys are secret and each \projecttitle{} device has unique identifier.


\subsection{RoCE Protocol Kernel}
\label{subsec:roce_protocol_kernel}

\begin{figure}[t!]
    \centering
    %\includegraphics[width=.27\textwidth]{figures/trusted-nic-single-node-overview.drawio-1.pdf}
    \includegraphics[width=0.5\textwidth]{figures/hw-implementation.drawio.pdf}
    \caption{\projecttitle{} hardware architecture.}
     \label{fig:tfpga}\label{fig:tRDMA}
\end{figure}


\myparagraph{Overview} Figure~\ref{fig:tRDMA} shows the hardware implementation of \projecttitle{}. \atsushi{the sentence is repeated} The role of the attestation kernel has already been discussed in $\S$~\ref{subsec:nic_attest_kernel}. The attestation kernel is connected to the the RoCE protocol kernel that implements the IB Transport Protocol on top of the UDP/IPv4 (RoCE v2)~\cite{infiniband} (transport and network layers).  To send data at the transmission path, the {\tt Req handler} module in RoCE kernel receives the request opcode (metadata) issued by the host. The message to be sent is then fetched through the XDMA AXI stream interface and passes through the attestation kernel for processing. The request opcode and the attested message are forwarded to the {\tt Request generation} module that constructs the network packet. %This module retrieves and updates the metadata while it also appends the attested message at the end. %This module updates the State tables with specific-to-the-RoCE protocol important metadata such as the network packets sequence numbers, the re-transmission tables, etc.
%, specifically it appends the corresponding headers, i.e., RETH (RDMA Extended Transport Header), AETH (ACK Extended Transport Header) and BTH (Base Transport Header)

Upon a message's reception, the RoCE kernel parses the packet headers and updates the state of the protocol (stored in State tables). The attested message is then forwarded to the attestation kernel. Upon a successful verification, the message is delivered to the application memory.

\myparagraph{Hardware design} \atsushi{We can definitely shorten the following paras, as they are either public IPs or already presented by prior studies (i.e., Coyote). What is important here is to explain how the attestation kernel (what we propose) corporates with the existing RDMA HW stack. Can we highlight this point?} The RoCE kernel implements a reliable connection transport service based on IB Protocol (including the UDP/IPv4 layers).  As shown in Figure~\ref{fig:tfpga}, the attestation kernel and the RoCE protocol kernel are wired to the XDMA IP that allows for Direct Memory Access (DMA) over PCIe~\cite{Sidler2019InNetworkDP, fpga_dma} between the host and \projecttitle{}. Additionally, the RoCE protocol kernel is connected to a CMAC kernel and an ARP server IP. 

\noindent{\underline{CMAC kernel:}} The CMAC kernel implements the link layer connecting the \projecttitle{} to the outside network fabric. It contains an IP block for the 100G Ethernet Subsystem~\cite{license} that needs to be configured for each board. This kernel bridges the whole infrastructure to the GT pins, which are the I/O pins towards the QSFP network interfaces. It also exposes two 512-bit AXI4-Stream interfaces to the RoCE protocol kernel for transmitting (Tx) and receiving (Rx) network packets. 

%The ARP server is also responsible for generating the ARP requests at the initialization before any RDMA operations are executed.
\noindent{\underline{ARP server:}}  The ARP server contains a lookup table with the correspondences
between MAC and IP addresses.  On the rising edge of the start signal for the \projecttitle{} RoCE kernel, the ARP server generates an ARP request with the remote IP address and forwards it to the CMAC kernel. Upon the reception of the ARP request, the recipient \projecttitle{} device responds with its MAC address. The ARP server of the sender creates an entry with the current IP---MAC pair.

Upon a packet reception the {\tt Request decoder} module examines it and forwards it to the ARP server or the RoCE stack based on the headers. Similarly, right before the transmission, the RDMA packets at the {\tt Request generation} first pass through a MAC and IP encoding phase. At this encoding phase the {\tt Request generation} module will extract from the lookup (ARP table) in the ARP server the remote MAC address. Then, the RDMA packet is generated according to the IB protocol (discussed below) and forwarded to the CMAC kernel.
%then insert that generates and encodes the RoCE packets (with the UPD header), the IPv4, and the Ethernet header forward this RDMA packet to the CMAC kernel. 

%At the decoding phase, the {\tt Request decoder} will analyse the IP and input Ethernet packets and distribute them to either the RoCE kernel or arp\_server based on their header fields.


\begin{figure}[t!]
    \centering
    \includegraphics[width=.5\textwidth]{figures/net-stack-implementation.drawio.pdf}
    \caption{\projecttitle{} RoCE protocol kernel stack.}
    \label{fig:ib_protocol}
\end{figure}
%
%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=.45\textwidth]{figures/trusted-nic-message_format.drawio.pdf}
%    \caption{\projecttitle{} message format.}
%    \label{fig:message_format}
%\end{figure}

\noindent{\underline{RoCE Protocol kernel:}} Figure~\ref{fig:ib_protocol} shows the architecture RoCE protocol kernel that implements the IB protocol~\cite{rdma_specification}.  We show both the transmission and reception data paths that can be processed independently (for performance). The dashed lines show the control path (requests and metadata) and the bold lines show the payload workflow.


The state of the protocol is stored in the State tables structures in the device memory and are similar to the original IB protocol specification~\cite{rdma_specification}. Specifically, the State tables store the network messages and protocol queue pairs (QPs), i.e., receive queue, send queue, completion queue, etc., the packet sequence numbers (PSNs), the message sequence numbers (MSNs) and the Retransmission Timer (RT). The PSNs are needed to define the valid, invalid, and duplicate PSN regions. The MSNs store the message sequence numbers along with the current
(DMA) address of the messages because due to packet fragmentation in large messages the remote (host) address is only part of the first packet. Lastly, the Retransmission Timer implements one timer per queue pair to detect packet loss. %The timers are
%implemented as an array of time intervals stored in on-chip
%memory. The Retransmission Timer module is continuously
%iterating over this array and decreasing the time intervals of all
%active timers. If any timer reaches zero an event is triggered
%and forwarded to the transmitting data path to retransmit the
%lost packet(s).

\noindent{\underline{Message format:}} The IB protocol in \projecttitle{} processes the following headers: IP, UDP, BTH (Base Transport Header), RETH (RDMA Extended Transport Header) and AETH (ACK Extended Transport Header) as defined in the RDMA Protocol Specification~\cite{rdma_specification, storm}.  The RoCE kernel adds the Ethernet header (L2 header), the IPv4/UDP headers (L3 headers) and the IB headers (L4 headers). It also adds a 32b end-to-end CRC (ICRC) that covers all invariant fields of the packet and offers protection beyond the coverage of the Ethernet Frame Checksum (FCS). The difference of our \projecttitle{} messages compared with the original RDMA messages is that for each transmitted packet, the attestation kernel {\em extends} the payload by appending a 64B attestation $\alpha$ and the metadata. The metadata include a 4B id for the session id of the sender, a 4B id for the device id (unique per device) and the appropriate {\tt send\_cnt}. %As explained in $\S$~\ref{subsec:nic_attest_kernel}, the $\alpha$ is calculated as the HMAC of the original payload concatenated with the previous metadata. 

\noindent{\underline{IB Protocol:}} The IB Protocol is executed as follows (Figure~\ref{fig:tRDMA}). On the transmitting data path, the {\tt Request hdlr} module receives requests issued by the host. For sending data (i.e., remote writes) it further instructs the DMA engine to forward the payload data from the host (DMA-ed) memory to the attestation kernel. The request is then forwarded to the next stage where the RETH/AETH and BHT corresponding headers (RDMA op-code, the packet sequence number and the queue pair number, etc.) are generated and appended to the attested message (if applicable). The module is implemented as a finite-state-machine that retrieves and updates the protocol state in the State tables. At the last state of the transmission the stack generates the UDP/IP headers (e.g., IP address, UDP port, and packet length) and appends it to the message.

Similarly, on the reception path, the message passes through different processing stages to extract the current protocol header, all relevant metadata and further validate the attested message. After decoding, checking and extracting the IP checksum, UDP port and other metadata in the IP/UDP decoder module, the remaining part of message is forwarded to the next stage. The BTH and RETH/AETH module extracts further metadata such as the RDMA op-code, the packet sequence number (PSN) and the queue pair number (QPN) from the header. These metadata are checked against the protocol state in the State tables and if needed they are updated. Lastly, the final stage processes the RETH/AETH headers (implemented as finite-state-machine) and executes the operation based on the RDMA op-code. %and if required
%issues DMA commands and requests to generate response
%packets.

%Figure 3 illustrates how the extracted PSN is checked
%against the expected PSN: (1) requesting the State Table entry
%using the QPN as a key, (2) the State Table returns the corresponding entry, (3) checking if the expected PSN in the entry
%matches the extracted PSN, and (4) instructing the Packet
%Dropper module to either drop the packet or forward it to the
%next stage. In case of a match the state machine concurrently
%writes the updated, expected PSN back to the State Table.
%These steps take around 5 cycles per packet, given that the
%smallest possible Ethernet frame is 64 B corresponding to 8
%cycles, we can guarantee that the hardware pipeline can sustain line-rate processing at 10 Gbit/s. At 5 cycles, the update
%step is a potential bottleneck for small packets at higher band-
%widths. However, in Section 7 we show that the message rate
%at higher bandwidths is limited by the host issuing commands
%and not by the packet processing. 



%After going through the merger, the packet
%will be sent out with the net_tx AXI Stream port. The RX path for RDMA packets is the same as that
%of ARP packets. Ingress packets will be diverted to the rocev2 IP rather than the ARP server by the
%IP handler according to their packet headers.

%To achieve this, the {\tt Request generation} and {\tt Request decoder} modules are connected. First, it is connected to an IPv4 decoder component that, upon reception of a packet, extracts the Ethernet header and distributes it to the RoCE kernel or the lookup (ARP) table accordingly. Additionally the stack contains a MAC/IPv4 encoder that generates and encodes the RoCE packets (with the UPD header), the IPv4, and the Ethernet header. The MAC addresses are extracted from the lookup (ARP) table that stores the IPs along with the corresponding MAC addresses. The MAC/IPv4 encoder is also responsible for handling the ARP request/response packets.


%A memory mapped interface is also used for the RoCE kernel to communicate with the HBM on FPGA. It is an AXI4 memory-mapped Master interface. The HBM on Alveo U280 FPGAs is divided into 32 segments with 256 MB each. The
%segments are called pseudo channels (PCs).

%The RoCE kernel input and output data cables, e.g., \texttt{axis\_rdma\_sink} and \texttt{axis\_host\_sink}, are connected through the Attestation kernel through 64B data paths (512-bit AXI4-Stream interfaces). Then, the Attestation kernel and the host memory communication are achieved through an AXI4 memory-mapped Master interface. It is the responsibility of the host code to allocate and initialize host memory. Further, the kernel is connected to a 32B bus to receive the parameters, a 20 B bus to issue RDMA write operations, and a 12 B bus to issue local DMA commands.



%The parameters for each kernel should be set and passed to the kernels on FPGAs. The RoCE kernel requires many parameters to establish an RDMA connection. These parameters include the queue pair numbers, message sequence numbers, IP address, and UDP ports for both the local and remote sides. The local virtual address and the rKey are also part of parameters that need to be written to the RoCE kernel by the host. Third, to communicate with the memory on FPGAs, host memory should also be allocated and initialized. This is done by the host executable codes. 

%Finally, the CMAC kernel is hooked to the GT pins provided by
%the Vitis shell and then connected to a QSFP port. The network stack is then connected to the outside
%network fabric.
%\noindent {\underline{CMAC kernel.}} 



%\noindent {\underline{Workflow}} Figure~\ref{fig:tRDMA} shows the workflow of the secured transmission and reception data paths. The data paths are pipelined to achieve line-rate bandwidth. At an RDMA operation (RDMA\_WRITE) the Request hdlr module receives the request issued by the host. The payload is then fetched from the DMA engine through the XDMA AXI stream interface and passes through the attestation kernel which generates the cryptographic signature of the message. Then the request is forwarded to the next module that generates the corresponding RETH (RDMA Extended Transport Header), AETH (ACK Extended Transport Header) and BTH (Base Transport Header) headers. This module deploys a state machine to retrieve and update the metadata and finally append the attested payload. This stage requires updating the State Tables (yellow colored box) that include the message sequence numbers, the packet sequence numbers, the retransmission tables, etc.

%Upon the reception of a message, the protocol parses the headers (IP$\rightarrow$UDP$\rightarrow$BTH$\rightarrow$RETH/AETH) and updates the metadata at the State Tables. The attested payload is then passed to the verification kernel. Upon successful verification, the message is then forwarded to the application memory.


%\dimitra{write about opennic tradeoffs -- say here that the opennic is more suitable for SN1000 where the DPDK is offloaded to the embedded cores. "A Simpler and Faster NIC Driver Model for Network Functions"}

%\myparagraph{Message Format} %The counter ID not only safeguards against equivocation but imposes a total ordering, allowing for the verification process to detect stale, re-ordered, or missed messages.



%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=.4\textwidth]{figures/bootstrapping.drawio.pdf}
%    \caption{\trustednic{} bootstrapping process.}
%    \label{fig:bootstrapping}
%\end{figure}



\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/remote_attestation.drawio.pdf}
    \caption{\trustednic{} remote attestation protocol.}
    \label{fig:remote_attestation}
\end{figure}

\subsection{Remote attestation} 
\label{subsec:nic_controller}
\atsushi{It is not clear to me what/where the NIC controller is. According to the texts, maybe you want to explain an execution flow of secure boot and remote attestation? If so, it might be better to change the Subsection title. }


\myparagraph{Hardware design} The last component of the \projecttitle{} design is the Controller which enables the remote attestation and initialization of the \projecttitle{}. The Controller is a static bitstream, e.g., a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733} with no access to confidential information that drives the remote attestation protocol to achieve three goals. First, it proves to the Protocol Designer the genuineness of the \projecttitle{}. Secondly, it guarantees that the \projecttitle{} bitstream is flashed securely in the device and, lastly, it allows the Protocol Designer to securely load configuration data (IPs, membership list, etc.) to \projecttitle{}. Finally, during normal execution, the Controller operates independently within the FPGA and continuously monitors the post-initialization JTAG activity to ensure that the bitstream is not modified before use and to prevent any physical attacks~\cite{secMon}. \atsushi{Monitoring JTAG is not sufficient to track the bitstream state because JTAG is not a universal way to reconfigure FPGA. ICAP (Internal Configuration Access Port) might be better, but I'm not sure}



%The Manufacturer manufactures the physical FPGA chips that are installed in the cloud infrastructure and are managed and owned by the cloud provider. The IP Vendor is a trusted entity that has synthesized the actual bitstreams for the \projecttitle{} and distributes them to the Protocol Designers. 
%The Protocol Designers are the users: they  each equipped with an FPGA-based NIC. Then, they flush the \projecttitle{} IP into the devices to use them. 

%\myparagraph{Device and \projecttitle{} manufacturing} To support remote attestation, there are three key parties that need to cooperate: the Manufacturer of the silicon (e.g., FPGA-based NICs on top of which \projecttitle{} runs), the IP Vendor that is responsible to implement and distribute the \projecttitle{} bitstream and, lastly, the Protocol Designer who builds distributed protocols leveraging \projecttitle{}. We assume that the Protocol Designers source \projecttitle{} bitstreams only from trusted IP Vendors (The Protocol Designer and the IP Vendor can be the same entity.). In addition, the Manufacturer and the IP Vendor are trusted. 

%Figure~\ref{fig:bootstrapping} shows the bootstrapping process in \projecttitle{}.
\myparagraph{Boostrappng}  At the manufacturing construction the Manufacturer burns a secret device key (HW$_{key}$) that is unique to the device~\cite{secure_FPGAs}. At the \projecttitle{} initialization, the Protocol designer instructs the cloud provider to load the FPGA the (encrypted) firmware from the storage medium using the embedded code in the BootROM device (2). The firmware is then decrypted using the HW$_{key}$.  %, a static bitstream containing a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733} that contains no confidential information. The Controller, along with the IP Vendor, prior to flushing the \trustednic{} bitstream to the device, performs remote attestation to prove to the Protocol Designer the authenticity of the device and the bitstream. During normal execution, the Controller operates independently within the FPGA~\cite{secMon} and continuously monitors (post-initialization) JTAG activity to ensure that the bitstream is not modified before use and to prevent any physical attacks.

The firmware loads the controller binary Ctrl$_{bin}$ (3), generates a key pair Ctrl$_{pub, priv}$ that is bound to the specific device and binary (4) and lastly, generates and signs the measurement of the Ctrl$_{bin}$ producing Ctrl$_{bin}$cert (5). %It also generates a Controller key pair, \texttt{Controller}$_{pub, priv}$ which is bound to this specific device and Controller binary as in~\cite{10.1145/3503222.3507733}. The key pair is later used to establish secure communication with the Vendor and sign the measurement of the \projecttitle{} bitstream.% and prove the authenticity of the code and the device.

In addition, the Protocol designer establishes a TLS/SSL connection with the trusted IP vendor (Figure~\ref{fig:remote_attestation}, (6)) \atsushi{Figure 4 is suddenly referred here?} and sends the list of the participating machines and any configuration data. Before the remote attestation protocol is initialized, the IP vendor and the Controller establish a secure communication channel (7)---(8). The IP vendor generates a random nonce n (for freshness) and an asymmetric key pair, V$_{pub, priv}$ (for secure communication with the Controller) and  sends the n and the public key \texttt{V}$_{pub}$ to the Controller. The Controller uses the \texttt{Vendor}$_{pub}$ and his own \texttt{Controller}$_{priv}$ to perform Diffie–Hellman key exchange with the Vendor and establish a shared secret key S$_{key}$ (8) which allows them from now on to securely communicate over insecure channels.

\myparagraph{Remote attestation} The Controller now is ready to execute the remote attestation as shown in Figure~\ref{fig:remote_attestation}, (9)---(17). First, it receives the encrypted bitstream \projecttitle{}$_{enc}$ from the vendor (9) and computes its measurement h (10). Next, it generates an attestation report m that contains the following data: the nonce n, the measurment of the \projecttitle{}$_enc$ h, the Ctrl$_{pub}$, the measurement of the Ctrl$_{bin}$ and its signature with the device key Ctrl$_{bin}$cert (11). The Controller signs the attestation report m with its private key and sends the attestation report along with its signature to the vendor.%(12) \texttt{Controller}$_{priv}$ generating $\sigma$$_{msr}$~\circled{5}. The Controller sends to the IP Vendor\circled{6} the $msr$, the $\sigma$$_{msr}$ and the signature of the generated \texttt{SKey} (with its \texttt{Controller}$_{priv}$). 

The IP vendor verifies the authenticity of the attestation report completing the remote attestation process (13)---(15) and, upon a successful attestation, it shares the vendor encryption key VE$_{key}$ with the Controller (16). First, the vendor the authenticity of the attestation report m with the Ctrl$_{pub}$ that is included in the message to verify that a genuine Ctrl$_{bin}$ has signed m (13). Afterwards, the vendor ensures that the Ctrl$_{bin}$ runs in a genuine \projecttitle{} device by verifying that the measurement of the Ctrl$_{bin}$ has been signed with an appropriate device key that has been installed by the Manufacturer (14). Lastly, the vendor verifies the nonce for freshness and that the measurement of the loaded encrypted bitstream h is the expected. 
%Finally, theIP Vendor establishes a secure channel to the Security Kernel by
%first generating the same SessionKey as the Security Kernel using
%AttestKey pub and VerifKey priv , and verifying that σ SessionKey
%was signed by AttestKey priv .

When all the verifications pass successfully, the remote attestation is completed. The IP vendor securely shares the VE$_{key}$ with the Controller by encrypting it with the previously established shared secret key S$_{key}$ (16).  The Controller decrypts the \projecttitle{} bitstream and loads it onto the FPGA (17). Similarly, the vendor shares any configuration data. Finally, the IP vendor notifies the Protocol designer about the result of the remote attestation.

%, ensuring that the plaintext bitstream containing sensitive IP and Shield Keys are only handled in secure on-chip memory\circled{8}. Lastly, using the same \texttt{SKey} the IP Vendor distributes the configuration data to the \trustednic{} instances.

%The IP Vendor will now notify the Protocol Designer that the machine has been attested and configured successfully~\circled{9}.

%\dimitra{explain how the designer publishes the configuration and the public keys of the participant FPGAs.}

\subsection{Formal verification of \projecttitle{} operations}
\label{subsec::formal_verification_remote_attestation}
\myparagraph{Remote Attestation} \dimitra{JULIAN}

\myparagraph{Network operations}

==> backups/t-nic-hardware.bak2.tex <==
\section{Trusted NIC Hardware}
\label{sec:t-nic-hardware}

Figure~\ref{fig:hardware-design} shows our \projecttitle{} hardware architecture that implements trusted network operations on the SmartNIC device. \projecttitle{} is comprised of two key hardware components: \emph{(i)} the attestation kernel that guarantees the non-equivocation and transferable authentication properties over the untrusted network ($\S$~\ref{subsec:nic_attest_kernel}) and \emph{(ii)} the RoCE protocol kernel that implements the RDMA protocol on the FPGA including the transport and network layers ($\S$~\ref{subsec:roce_protocol_kernel}). Lastly, we design a remote attestation protocol for our \projecttitle{} based on the \projecttitle{} Controller module that we discuss $\S$~\ref{subsec:nic_controller}. Importantly, we formally verify \projecttitle{}'s remote attestation and initialization protocol ($\S$~\ref{subsec::formal_verification_remote_attestation}).

%securely bootstraps the device and flushes the bitstream. % initializes the device, offers remote attestation to ensure the authenticity of the device and the flushed bitstream and guarantees run-time isolation.



% PUT THIS IN OVERVIEW To prevent equivocation and guarantee the validity of the network traffic, we require each node that participates in a distributed protocol to be equipped with a \trustedfpga{} subsystem. Each \trustedfpga{} is configured by the developer at the initialization with a secret (asymmetric) key, and it is uniquely identified by an identifier that corresponds to the node that hosts the subsystem.

%The secret key is private, whereas the public key is exposed to the application layer. Apart from the private key, the internal state of the \trustedfpga{} and the algorithm used to authenticate messages may be known publicly. %The private keys are generated and installed to each \trustedfpga{} during initialization.
%For now, we assume that the secret key is manually
%installed before system startup. In a future version, every
%CASH subsystem would maintain a private key and expose
%the corresponding public key. A shared secret key for every
%protocol instance may be generated during initialization, encrypted under the public key of every subsystem, and trans-
%ported securely to every replica.

\begin{algorithm}
\SetAlgoLined
\small
\textbf{function} \texttt{Attest(c\_id, msg)} \{ \\
\Indp
{\tt cnt} $\leftarrow$ {\tt send\_cnts[c\_id]++};\\
$\alpha$ $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)}; \\
\textbf{return} $\alpha${\tt ||msg||cnt};\\
\Indm
\} \\


\vspace{0.3cm}

\textbf{function} \texttt{Verify(c\_id, $\alpha$||msg||cnt)} \{ \\
\Indp
    $\alpha$' $\leftarrow$ {\tt hmac(keys[c\_id], msg||cnt)};\\
    \textbf{if} {\tt (}$\alpha$' $=$ $\alpha$ {\tt \&\&} {\tt cnt} $=$ {\tt recv\_cnts[c\_id]++} {\tt )}\\
    \Indp
        \textbf{return} ($\alpha${\tt ||msg||cnt)}; \\
    \Indm
    \textbf{assert(False)}; \\
\Indm
\} \\
%\vspace{0.1cm}
\vspace{-1pt}
\caption{\texttt{Attest()} and \texttt{Verify()} functions.}
\label{algo:primitives}
\end{algorithm}

\if 0
\begin{center}
\begin{table}[ht]
\small
\centering
\begin{tabular}{ |m{2cm}||m{5.6cm}|}
 \hline
 {\tt ID} & A unique ID for this \projecttitle{} instance. \\
 {\tt keys[]} & (shared) Keys network sessions. \\
 {\tt send\_cnts[]} & Current counters values on transmission path per session.\\
 {\tt recv\_cnts[]} & Current counters values on reception path per session.\\
 \hline
 \end{tabular}
\caption{Attestation kernel state.}
\label{table:api}
\end{table}
\end{center}
\fi 

\subsection{NIC Attestation Kernel}
\label{subsec:nic_attest_kernel}
\myparagraph{Overview} 
The attestation kernel {\em shields} the network messages and materializes the properties of non-equivocation and transferable authentication by generating {\em attestations} for the transmitted messages. As shown in Figure~\ref{fig:hardware-design}, the attestation kernel is pipelined on the data path, processing the messages as they {\em flow} from host memory to the device and vice versa to optimize for throughput. The module resides in the data pipeline between the RoCE protocol kernel that transmits/receives the network messages and the PCIe DMA which fetches and pushes data {\em asynchronously} from the host memory to the FPGA memory.
%\atsushi{Figure 2 and the following paragraphs: "XDMA IP" and "CMAC" are specific terms for Xilinx FPGAs. If we want to make the hardware architecture/design vendor-agnostic, we should use another term such as "PCIe IP" and "Ethernet IP", for example, respectively.}


%{\noindent \underline{Attestation kernel state.}} 
\myparagraph{System design} The attestation kernel is comprised of three components that represent its state and functionality: the HMAC component that generates the message authentication codes (MAC), the Keystore which stores the keys used by the HMAC module, and the Counters store that keeps the messages latest sent and received timestamp. 

%Table~\ref{table:api} summarizes the internal state of the attestation kernel (per device). 
Each \projecttitle{} device is initialized from the Protocol Designer during bootstrapping ($\S$~\ref{subsec:nic_controller}) with a unique identifier (ID) and some shared secret keys---ideally, one shared key for each session, which is stored in static memory (Keystore). The keys are shared and, hence, not known to the untrusted parties. % and as such even local (single-node) attestations always need pass through the \projecttitle{}. 

The \projecttitle{} also holds two counters per session stored in the Counters store (Figure~\ref{fig:hardware-design}), the {\tt send\_cnts} to be used for sending messages and the \texttt{recv\_cnts} that holds the latest seen counter value for each session. The counters represent the messages' timestamp and are increased monotonically and deterministically after every send and receive operation to ensure that unique messages will be assigned to unique counters (for non-equivocation) and consequently, no messages can be lost, re-ordered, or doubly-executed.




\myparagraph{Algorithm} Algorithm~\ref{algo:primitives} shows the functionality of the attestation kernel. The module implements two core functions: the {\tt Attest} function which generates a unique and verifiable attestation for a message and the {\tt Verify} function which verifies the attestation of a received message. When the application transmits a message, the data flow passes through the {\tt Attest} function and upon a message reception, the message is verified (with {\tt Verify} function) before it is copied to the application's (host) memory. 

As shown in Figure~\ref{fig:hardware-design}, a request passes from the application layer to the \projecttitle{} through two separate paths, i.e., the data and control paths. The metadata and the request opcode pass through the control path from the host to the device and vice versa. On the other hand, the message data is first forwarded to the attestation kernel and then, the output is forwarded to the RoCE protocol kernel. The attestation kernel upon transmission executes the \texttt{Attest} function and generates an {\em attested} message comprised of the message data and its attestation certificate, or simply attestation $\alpha$. The function calculates $\alpha$ as the HMAC of the message concatenated with the counter {\tt send\_cnt} using the {\tt key} for that connection (Algorithm~\ref{algo:primitives}:~L3). It also increases the next available counter for subsequent future messages (Algorithm~\ref{algo:primitives}:~L2). The function forwards to the RoCE protocol the original message along with $\alpha$ for transmission (Algorithm~\ref{algo:primitives}:~L4).

%where the control flow forwards the request for \emph{increment} (\circled{1c}) and also fetches the corresponding sequencer \texttt{<mc\_id, v, cnt>} from the \emph{mc ids index} (\circled{1a}, \circled{1b}). After the increment the producing message is of the form \texttt{<sequencer, msg>} which is now being signed with the node's private key following the same workflow (\circled{2a}, \circled{2b}, \circled{2c}). The signed message \texttt{<(header, h(msg))$\sigma$, msg>}  can be logged (for recoverability) and is now forwarded to the network stack for transmission.

%{\noindent \underline{Verify path.}} 
Upon reception, the received message passes through the attestation kernel for verification before it is delivered to the application. Specifically, the \texttt{Verify} function checks the authenticity and the integrity of the received message by re-calculating the {\em expected} attestation ($\alpha$') based on the message payload and comparing it with the received attestation ($\alpha$) of the message (Algorithm~\ref{algo:primitives}:~L7---8). Following that, the verification also ensures that the received counter matches the expected counter for that connection to ensure \emph{continuity} (Algorithm~\ref{algo:primitives}:~L8). 

%\myparagraph{Security analysis} This simple attestation kernel achieves to ensure the properties of non-equivocation and transferable authentication. First, \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages
%will never be assigned identical {\tt send\_cnts}. The property is ensured because the {\tt send\_cnts} are never decremented. Secondly the \projecttitle{} ensures the transferable authentication because the cryptosystem is not broken, the keys are secret and each \projecttitle{} device has unique identifier.


\subsection{RoCE Protocol Kernel}
\label{subsec:roce_protocol_kernel}

\begin{figure}[t!]
    \centering
    %\includegraphics[width=.27\textwidth]{figures/trusted-nic-single-node-overview.drawio-1.pdf}
    %\includegraphics[width=0.45\textwidth]{figures/hw-implementation.drawio.pdf}
    %\caption{\projecttitle{} hardware architecture.}
     \includegraphics[width=\linewidth]{figures/hardware-implementation-colored.drawio.pdf}
    \caption{\projecttitle{} hardware architecture.}
     \label{fig:hardware-design}
\end{figure}


\myparagraph{Overview} The RoCE protocol kernel implements a reliable transport service on top of the IB Transport Protocol with UDP/IPv4 layers (RoCE v2)~\cite{infiniband} (transport and network layers) and it is connected to the attestation kernel as discussed in $\S$~\ref{subsec:nic_attest_kernel}. As shown in Figure~\ref{fig:hardware-design}, to send data at the transmission path, the {\tt Req handler} module in the RoCE kernel receives the request opcode (metadata) issued by the host. The message to be sent is then fetched through the PCie DMA engine and passes through the attestation kernel for processing. The request opcode and the attested message are forwarded to the {\tt Request generation} module that constructs the network packet. %This module retrieves and updates the metadata while it also appends the attested message at the end. %This module updates the State tables with specific-to-the-RoCE protocol important metadata such as the network packets sequence numbers, the re-transmission tables, etc.
%, specifically it appends the corresponding headers, i.e., RETH (RDMA Extended Transport Header), AETH (ACK Extended Transport Header) and BTH (Base Transport Header)

Upon a message's reception from the network, the RoCE kernel parses the packet headers and updates the state of the protocol (stored in State tables). The attested message is then forwarded to the attestation kernel. Upon a successful verification, the message is delivered to the application memory. 

%\atsushi{We can definitely shorten the following paras, as they are either public IPs or already presented by prior studies (i.e., Coyote). What is important here is to explain how the attestation kernel (what we propose) corporates with the existing RDMA HW stack. Can we highlight this point?} The RoCE kernel implements a reliable connection transport service based on IB Protocol (including the UDP/IPv4 layers).  As shown in Figure~\ref{fig:hardware-design}, the attestation kernel and the RoCE protocol kernel are wired to the XDMA IP that allows for Direct Memory Access (DMA) over PCIe~\cite{Sidler2019InNetworkDP, fpga_dma} between the host and \projecttitle{}. 

\myparagraph{Hardware design} The RoCE protocol kernel is additionally connected to a 100Gb MAC IP and an ARP server IP. 

\noindent{\underline{100Gb MAC.}} The 100Gb MAC kernel implements the link layer connecting \projecttitle{} to the network fabric over a 100G Ethernet Subsystem~\cite{license}. The  kernel also exposes two interfaces to the RoCE protocol kernel for transmitting (Tx) and receiving (Rx) network packets. %\atsushi{Here is also specific to the implementation (on Xilinx FPGAs) rather than the design.}

\noindent{\underline{ARP server.}} The ARP server contains a lookup table with the correspondences
between MAC and IP addresses. Right before the transmission, the RDMA packets at the {\tt Request generation} first pass through a MAC and IP encoding phase. At this encoding phase, the {\tt Request generation} module extracts from the lookup (ARP table) in the ARP server the remote MAC address.

%\noindent{\underline{CMAC kernel:}} The CMAC kernel implements the link layer connecting the \projecttitle{} to the outside network fabric. It contains an IP block for the 100G Ethernet Subsystem~\cite{license} that needs to be configured for each board. This kernel bridges the whole infrastructure to the GT pins, which are the I/O pins towards the QSFP network interfaces. It also exposes two 512-bit AXI4-Stream interfaces to the RoCE protocol kernel for transmitting (Tx) and receiving (Rx) network packets. 

%The ARP server is also responsible for generating the ARP requests at the initialization before any RDMA operations are executed.
%\noindent{\underline{ARP server:}}  The ARP server contains a lookup table with the correspondences
%between MAC and IP addresses.  On the rising edge of the start signal for the \projecttitle{} RoCE kernel, the ARP server generates an ARP request with the remote IP address and forwards it to the CMAC kernel. Upon the reception of the ARP request, the recipient \projecttitle{} device responds with its MAC address. The ARP server of the sender creates an entry with the current IP---MAC pair.

%Upon a packet reception the {\tt Request decoder} module examines it and forwards it to the ARP server or the RoCE stack based on the headers. Similarly, right before the transmission, the RDMA packets at the {\tt Request generation} first pass through a MAC and IP encoding phase. At this encoding phase the {\tt Request generation} module will extract from the lookup (ARP table) in the ARP server the remote MAC address. Then, the RDMA packet is generated according to the IB protocol (discussed below) and forwarded to the CMAC kernel.
%then insert that generates and encodes the RoCE packets (with the UPD header), the IPv4, and the Ethernet header forward this RDMA packet to the CMAC kernel. 

%At the decoding phase, the {\tt Request decoder} will analyse the IP and input Ethernet packets and distribute them to either the RoCE kernel or arp\_server based on their header fields.


%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=.45\textwidth]{figures/net-stack-implementation.drawio.pdf}
%    \caption{\projecttitle{} RoCE protocol kernel stack.}
%    \label{fig:ib_protocol}
%\end{figure}
%
%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=.45\textwidth]{figures/trusted-nic-message_format.drawio.pdf}
%    \caption{\projecttitle{} message format.}
%    \label{fig:message_format}
%\end{figure}

\noindent{\underline{IB protocol.}} The RoCE protocol kernel implements the reliable version of the IB protocol. Similarly to its original specification~\cite{rdma_specification}, the kernel implements the State tables to store the protocol queues QPs (i.e., receive queue, send queue, completion queue, etc.). The State tables also store important metadata such as (1) the packet sequence numbers (PSNs) to distinguish valid, invalid, and duplicate PSN regions, (2) the message sequence numbers (MSNs) to reconstruct fragmented network messages, and (3) a Retransmission Timer to detect packet losses.

The transmitting path is shown in Figure~\ref{fig:hardware-design} with the blue-colored axes. The {\tt Req handler} receives the requests issued by the host and initializes a DMA command to fetch the payload data from the host (DMA-ed) memory to the attestation kernel. Once the attestation kernel forwards the attested message to the {\tt Req handler}, the module passes the message from several states to append the appropriate headers along with metadata (e.g., RDMA op-code, the PSN and the QP number, etc.). The last part of the processing generates and appends the UDP/IP headers (e.g., IP address, UDP port, and packet length). The message is then forwarded to the CMAC module. Similarly, on the reception path (shown in the red-colored axes), the {\tt Request decoder} extract the headers, metadata, and attested message. The later is forwarded for verification and finally copied to the host memory.

%Similarly, on the reception path, the message passes through different processing stages to extract the current protocol header, all relevant metadata and further validate the attested message. After decoding, checking and extracting the IP checksum, UDP port and other metadata in the IP/UDP decoder module, the remaining part of message is forwarded to the next stage. The BTH and RETH/AETH module extracts further metadata such as the RDMA op-code, the packet sequence number (PSN) and the queue pair number (QPN) from the header. These metadata are checked against the protocol state in the State tables and if needed they are updated. Lastly, the final stage processes the RETH/AETH headers (implemented as finite-state-machine) and executes the operation based on the RDMA op-code.

%Figure~\ref{fig:ib_protocol} shows the architecture RoCE protocol kernel that implements the IB protocol~\cite{rdma_specification}.  We show both the transmission and reception data paths that can be processed independently (for performance). The dashed lines show the control path (requests and metadata) and the bold lines show the payload workflow.


%The state of the protocol is stored in the State tables structures in the device memory and are similar to the original IB protocol specification~\cite{rdma_specification}. Specifically, the State tables store the network messages and protocol queue pairs (QPs), i.e., receive queue, send queue, completion queue, etc., the packet sequence numbers (PSNs), the message sequence numbers (MSNs) and the Retransmission Timer (RT). The PSNs are needed to define the valid, invalid, and duplicate PSN regions. The MSNs store the message sequence numbers along with the current
%(DMA) address of the messages because due to packet fragmentation in large messages the remote (host) address is only part of the first packet. Lastly, the Retransmission Timer implements one timer per queue pair to detect packet loss. %The timers are
%implemented as an array of time intervals stored in on-chip
%memory. The Retransmission Timer module is continuously
%iterating over this array and decreasing the time intervals of all
%active timers. If any timer reaches zero an event is triggered
%and forwarded to the transmitting data path to retransmit the
%lost packet(s).

\myparagraph{{Message format:}} The IB protocol in \projecttitle{} processes the following headers: IP, UDP, BTH (Base Transport Header), RETH (RDMA Extended Transport Header) and AETH (ACK Extended Transport Header) as defined in the RDMA Protocol Specification~\cite{rdma_specification, storm}.  The RoCE kernel adds the Ethernet header (L2 header), the IPv4/UDP headers (L3 headers) and the IB headers (L4 headers). It also adds a 32b end-to-end CRC (ICRC) that covers all invariant fields of the packet and offers protection beyond the coverage of the Ethernet Frame Checksum (FCS). The difference of our \projecttitle{} messages compared with the original RDMA messages is that for each transmitted packet, the attestation kernel {\em extends} the payload by appending a 64B attestation $\alpha$ and the metadata. The metadata include a 4B id for the session id of the sender, a 4B id for the device id (unique per device) and the appropriate {\tt send\_cnt}. %As explained in $\S$~\ref{subsec:nic_attest_kernel}, the $\alpha$ is calculated as the HMAC of the original payload concatenated with the previous metadata. 

%\noindent{\underline{IB Protocol:}} The IB Protocol is executed as follows (Figure~\ref{fig:hardware-design}). On the transmitting data path, the {\tt Request hdlr} module receives requests issued by the host. For sending data (i.e., remote writes) it further instructs the DMA engine to forward the payload data from the host (DMA-ed) memory to the attestation kernel. The request is then forwarded to the next stage where the RETH/AETH and BHT corresponding headers (RDMA op-code, the packet sequence number and the queue pair number, etc.) are generated and appended to the attested message (if applicable). The module is implemented as a finite-state-machine that retrieves and updates the protocol state in the State tables. At the last state of the transmission the stack generates the UDP/IP headers (e.g., IP address, UDP port, and packet length) and appends it to the message.

%Similarly, on the reception path, the message passes through different processing stages to extract the current protocol header, all relevant metadata and further validate the attested message. After decoding, checking and extracting the IP checksum, UDP port and other metadata in the IP/UDP decoder module, the remaining part of message is forwarded to the next stage. The BTH and RETH/AETH module extracts further metadata such as the RDMA op-code, the packet sequence number (PSN) and the queue pair number (QPN) from the header. These metadata are checked against the protocol state in the State tables and if needed they are updated. Lastly, the final stage processes the RETH/AETH headers (implemented as finite-state-machine) and executes the operation based on the RDMA op-code. %and if required
%issues DMA commands and requests to generate response
%packets.

%Figure 3 illustrates how the extracted PSN is checked
%against the expected PSN: (1) requesting the State Table entry
%using the QPN as a key, (2) the State Table returns the corresponding entry, (3) checking if the expected PSN in the entry
%matches the extracted PSN, and (4) instructing the Packet
%Dropper module to either drop the packet or forward it to the
%next stage. In case of a match the state machine concurrently
%writes the updated, expected PSN back to the State Table.
%These steps take around 5 cycles per packet, given that the
%smallest possible Ethernet frame is 64 B corresponding to 8
%cycles, we can guarantee that the hardware pipeline can sustain line-rate processing at 10 Gbit/s. At 5 cycles, the update
%step is a potential bottleneck for small packets at higher band-
%widths. However, in Section 7 we show that the message rate
%at higher bandwidths is limited by the host issuing commands
%and not by the packet processing. 



%After going through the merger, the packet
%will be sent out with the net_tx AXI Stream port. The RX path for RDMA packets is the same as that
%of ARP packets. Ingress packets will be diverted to the rocev2 IP rather than the ARP server by the
%IP handler according to their packet headers.

%To achieve this, the {\tt Request generation} and {\tt Request decoder} modules are connected. First, it is connected to an IPv4 decoder component that, upon reception of a packet, extracts the Ethernet header and distributes it to the RoCE kernel or the lookup (ARP) table accordingly. Additionally the stack contains a MAC/IPv4 encoder that generates and encodes the RoCE packets (with the UPD header), the IPv4, and the Ethernet header. The MAC addresses are extracted from the lookup (ARP) table that stores the IPs along with the corresponding MAC addresses. The MAC/IPv4 encoder is also responsible for handling the ARP request/response packets.


%A memory mapped interface is also used for the RoCE kernel to communicate with the HBM on FPGA. It is an AXI4 memory-mapped Master interface. The HBM on Alveo U280 FPGAs is divided into 32 segments with 256 MB each. The
%segments are called pseudo channels (PCs).

%The RoCE kernel input and output data cables, e.g., \texttt{axis\_rdma\_sink} and \texttt{axis\_host\_sink}, are connected through the Attestation kernel through 64B data paths (512-bit AXI4-Stream interfaces). Then, the Attestation kernel and the host memory communication are achieved through an AXI4 memory-mapped Master interface. It is the responsibility of the host code to allocate and initialize host memory. Further, the kernel is connected to a 32B bus to receive the parameters, a 20 B bus to issue RDMA write operations, and a 12 B bus to issue local DMA commands.



%The parameters for each kernel should be set and passed to the kernels on FPGAs. The RoCE kernel requires many parameters to establish an RDMA connection. These parameters include the queue pair numbers, message sequence numbers, IP address, and UDP ports for both the local and remote sides. The local virtual address and the rKey are also part of parameters that need to be written to the RoCE kernel by the host. Third, to communicate with the memory on FPGAs, host memory should also be allocated and initialized. This is done by the host executable codes. 

%Finally, the CMAC kernel is hooked to the GT pins provided by
%the Vitis shell and then connected to a QSFP port. The network stack is then connected to the outside
%network fabric.
%\noindent {\underline{CMAC kernel.}} 



%\noindent {\underline{Workflow}} Figure~\ref{fig:tRDMA} shows the workflow of the secured transmission and reception data paths. The data paths are pipelined to achieve line-rate bandwidth. At an RDMA operation (RDMA\_WRITE) the Request hdlr module receives the request issued by the host. The payload is then fetched from the DMA engine through the XDMA AXI stream interface and passes through the attestation kernel which generates the cryptographic signature of the message. Then the request is forwarded to the next module that generates the corresponding RETH (RDMA Extended Transport Header), AETH (ACK Extended Transport Header) and BTH (Base Transport Header) headers. This module deploys a state machine to retrieve and update the metadata and finally append the attested payload. This stage requires updating the State Tables (yellow colored box) that include the message sequence numbers, the packet sequence numbers, the retransmission tables, etc.

%Upon the reception of a message, the protocol parses the headers (IP$\rightarrow$UDP$\rightarrow$BTH$\rightarrow$RETH/AETH) and updates the metadata at the State Tables. The attested payload is then passed to the verification kernel. Upon successful verification, the message is then forwarded to the application memory.


%\dimitra{write about opennic tradeoffs -- say here that the opennic is more suitable for SN1000 where the DPDK is offloaded to the embedded cores. "A Simpler and Faster NIC Driver Model for Network Functions"}

%\myparagraph{Message Format} %The counter ID not only safeguards against equivocation but imposes a total ordering, allowing for the verification process to detect stale, re-ordered, or missed messages.



%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=.4\textwidth]{figures/bootstrapping.drawio.pdf}
%    \caption{\trustednic{} bootstrapping process.}
%    \label{fig:bootstrapping}
%\end{figure}



\begin{figure}[t!]
    \centering
    \includegraphics[width=.45\textwidth]{figures/remote_attestation.drawio.pdf}
    \caption{\trustednic{} remote attestation protocol.}
    \label{fig:remote_attestation}
\end{figure}

\subsection{Remote Attestation Protocol} 
\label{subsec:nic_controller}
We design a remote attestation protocol for the \projecttitle{} to ensure that the \projecttitle{} device is genuine and the \projecttitle{} bitstream is flashed securely in the device along with the designer's configuration data (IPs, secrets, etc.).

\myparagraph{Design assumptions} We base our design for the remote attestation protocol on the NIC Controller, a hardware component that drives the device initialization as in~\cite{10.1145/3503222.3507733}. The Controller can be implemented as a static bitstream (a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733}) with no access to confidential information. After the initialization process, the Controller monitors the JTAG/ICAP ports to ensure that the bitstream is not modified before use and prevent physical attacks as commercial IPs~\cite{secMon}.
%\atsushi{It is not clear to me what/where the NIC controller is. According to the texts, maybe you want to explain an execution flow of secure boot and remote attestation? If so, it might be better to change the Subsection title. }






%The Manufacturer manufactures the physical FPGA chips that are installed in the cloud infrastructure and are managed and owned by the cloud provider. The IP Vendor is a trusted entity that has synthesized the actual bitstreams for the \projecttitle{} and distributes them to the Protocol Designers. 
%The Protocol Designers are the users: they  each equipped with an FPGA-based NIC. Then, they flush the \projecttitle{} IP into the devices to use them. 

%\myparagraph{Device and \projecttitle{} manufacturing} To support remote attestation, there are three key parties that need to cooperate: the Manufacturer of the silicon (e.g., FPGA-based NICs on top of which \projecttitle{} runs), the IP Vendor that is responsible to implement and distribute the \projecttitle{} bitstream and, lastly, the Protocol Designer who builds distributed protocols leveraging \projecttitle{}. We assume that the Protocol Designers source \projecttitle{} bitstreams only from trusted IP Vendors (The Protocol Designer and the IP Vendor can be the same entity.). In addition, the Manufacturer and the IP Vendor are trusted. 

%Figure~\ref{fig:bootstrapping} shows the bootstrapping process in \projecttitle{}.
\myparagraph{Boostrappng} We next describe the bootstrapping phase of the device and the remote attestation mechanism in \projecttitle{}. At the manufacturing construction, the Manufacturer burns a secret device key (HW$_{key}$) that is unique to the device~\cite{secure_FPGAs}. At the \projecttitle{} initialization, the Protocol designer instructs the cloud provider to load the FPGA the (encrypted) firmware from the storage medium using the embedded code in the BootROM device (2). The firmware is then decrypted using the HW$_{key}$.  %, a static bitstream containing a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733} that contains no confidential information. The Controller, along with the IP Vendor, prior to flushing the \trustednic{} bitstream to the device, performs remote attestation to prove to the Protocol Designer the authenticity of the device and the bitstream. During normal execution, the Controller operates independently within the FPGA~\cite{secMon} and continuously monitors (post-initialization) JTAG activity to ensure that the bitstream is not modified before use and to prevent any physical attacks.

The firmware loads the controller binary Ctrl$_{bin}$ (3), generates a key pair Ctrl$_{pub, priv}$ that is bound to the specific device and binary (4), and lastly, generates and signs the measurement of the Ctrl$_{bin}$ producing Ctrl$_{bin}$cert (5). %It also generates a Controller key pair, \texttt{Controller}$_{pub, priv}$ which is bound to this specific device and Controller binary as in~\cite{10.1145/3503222.3507733}. The key pair is later used to establish secure communication with the Vendor and sign the measurement of the \projecttitle{} bitstream.% and prove the authenticity of the code and the device.

In addition, the Protocol designer establishes a TLS/SSL connection with the trusted IP vendor and sends the list of the participating machines and any configuration data. Before the remote attestation protocol is initialized, the IP vendor and the Controller establish a secure communication channel (7)---(8). The IP vendor generates a random nonce n (for freshness) and an asymmetric key pair, V$_{pub, priv}$ (for secure communication with the Controller) and  sends the n and the public key \texttt{V}$_{pub}$ to the Controller. The Controller uses the \texttt{Vendor}$_{pub}$ and his own \texttt{Controller}$_{priv}$ to perform Diffie–Hellman key exchange with the Vendor and establish a shared secret key S$_{key}$ (8) which allows them from now on to securely communicate over insecure channels.

\myparagraph{Remote attestation} The Controller is now ready to execute the remote attestation as shown in Figure~\ref{fig:remote_attestation}, (9)---(17). First, it receives the encrypted bitstream \projecttitle{}$_{enc}$ from the vendor (9) and computes its measurement h (10). Next, it generates an attestation report m that contains the following data: the nonce n, the measurement of the \projecttitle{}$_enc$ h, the Ctrl$_{pub}$, the measurement of the Ctrl$_{bin}$ and its signature with the device key Ctrl$_{bin}$cert (11). The Controller signs the attestation report m with its private key and sends the attestation report along with its signature to the vendor.%(12) \texttt{Controller}$_{priv}$ generating $\sigma$$_{msr}$~\circled{5}. The Controller sends to the IP Vendor\circled{6} the $msr$, the $\sigma$$_{msr}$ and the signature of the generated \texttt{SKey} (with its \texttt{Controller}$_{priv}$). 

The IP vendor verifies the authenticity of the attestation report by completing the remote attestation process (13)---(15) and, upon a successful attestation, it shares the vendor encryption key VE$_{key}$ with the Controller (16). First, the vendor the authenticity of the attestation report m with the Ctrl$_{pub}$ that is included in the message to verify that a genuine Ctrl$_{bin}$ has signed m (13). Afterward, the vendor ensures that the Ctrl$_{bin}$ runs in a genuine \projecttitle{} device by verifying that the measurement of the Ctrl$_{bin}$ has been signed with an appropriate device key that has been installed by the Manufacturer (14). Lastly, the vendor verifies the nonce for freshness and that the measurement of the loaded encrypted bitstream h is as expected. 
%Finally, theIP Vendor establishes a secure channel to the Security Kernel by
%first generating the same SessionKey as the Security Kernel using
%AttestKey pub and VerifKey priv , and verifying that σ SessionKey
%was signed by AttestKey priv .

When all the verifications pass successfully, the remote attestation is completed. The IP vendor securely shares the VE$_{key}$ with the Controller by encrypting it with the previously established shared secret key S$_{key}$ (16).  The Controller decrypts the \projecttitle{} bitstream and loads it onto the FPGA (17). Similarly, the vendor shares any configuration data. Finally, the IP vendor notifies the Protocol designer about the result of the remote attestation.


%\myparagraph{Hardware design} The last component of the \projecttitle{} design is the Controller which enables the remote attestation and initialization of the \projecttitle{}. The Controller is a static bitstream, e.g., a soft CPU~\cite{microblaze, nios, 10.1145/3503222.3507733} with no access to confidential information that drives the remote attestation protocol to achieve three goals. First, it proves to the Protocol Designer the genuineness of the \projecttitle{}. Secondly, it guarantees that the \projecttitle{} bitstream is flashed securely in the device and, lastly, it allows the Protocol Designer to securely load configuration data (IPs, membership list, etc.) to \projecttitle{}. Finally, during normal execution, the Controller operates independently within the FPGA and continuously monitors the post-initialization JTAG activity to ensure that the bitstream is not modified before use and to prevent any physical attacks~\cite{secMon}. \atsushi{Monitoring JTAG is not sufficient to track the bitstream state because JTAG is not a universal way to reconfigure FPGA. ICAP (Internal Configuration Access Port) might be better, but I'm not sure}

%, ensuring that the plaintext bitstream containing sensitive IP and Shield Keys are only handled in secure on-chip memory\circled{8}. Lastly, using the same \texttt{SKey} the IP Vendor distributes the configuration data to the \trustednic{} instances.

%The IP Vendor will now notify the Protocol Designer that the machine has been attested and configured successfully~\circled{9}.

%\dimitra{explain how the designer publishes the configuration and the public keys of the participant FPGAs.}

\subsection{Formal Verification of \projecttitle{} Operations}
\label{subsec::formal_verification_remote_attestation}
We formally verify the security and safety properties of \projecttitle{} hardware. First, we verify the bootstrapping and the remote attestation protocol of \projecttitle{} ensuring that the correct bitstream has securely flushed to a genuine SmartNIC device. Secondly we verify that the properties of the non-equivocation and the transferable authentication are met under normal operation. 

We use Tamarin~\cite{tamarin-prover}, a security protocol verification tool that analyzes symbolic models of protocols specified as multiset rewriting systems. This model imposes the following assumptions: \emph{(i)}~all messages are composed of atomic terms using predefined functions \dimitra{What does that mean :) ?} \emph{(ii)}~these cryptographic functions are perfect with no side-effects \dimitra{are not compromised?} \emph{(iii)}~attackers can read and delete all messages that are sent on the network and modify them in accordance with the set of available functions.

\myparagraph{Remote Attestation} We model the bootstrapping and remote attestation protocols as described in Figure~\ref{fig:remote_attestation}.

%using Tamarin~\cite{tamarin-prover}. Tamarin is a security protocol verification tool that analyzes symbolic models of protocols specified as multiset rewriting systems. This model imposes the following assumptions: \emph{(i)}~all messages are composed of atomic terms using predefined functions \emph{(ii)}~these cryptographic functions are perfect with no side-effects \emph{(iii)}~attackers can read and delete all messages that are sent on the network and modify them in accordance with the set of available functions.

Our verification work relies on properties of the already analyzed TLS handshake~\cite{tamarin_tls_proof} and proofs the desired security properties of the \projecttitle{} bootstrapping and attestation protocol.  The desired properties are modeled as lemmas that define valid and invalid system states. Tamarin then verifies the specified lemmas, by \emph{(i)} finding at least one trace  (series of state transitions) for the valid control states and \emph{(ii)} showing that there exists no trace leading to invalid states.

We define multiple lemmas to ensure the secrecy of the private secrets involved in the protocol as well as the main attestation lemma which holds if and only if: once the last step of the remote attestation protocol is completed, the \projecttitle{} device is in a valid, expected state. 

In our model, Tamarin found at least one trace for every control state and proved that there is no trace to any state where our lemmas are violated. Thus, our attestation lemmas hold for our model.



%\julian{The following is my addition, using the Tamarin proofs - I don't know how to integrate them, feel free to rephrase/delete if required}

\myparagraph{Network operations} We extend the analysis of the bootstrapping and attestation protocol in Tamarin with models for the network operations that upon the message transmission and reception execute the {\tt Attest} and {\tt Verify} functions (Algorithm~\ref{algo:primitives}), respectively. In simple words we prove that  \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages will never be assigned identical message sequencers ({\tt send\_cnts}) and secondly, the transferable authentication is met because each generated attestation is is uniquely verified by the secret keys jointly with the unique sender's \projecttitle{} device identifier.
 %since valid attestations can only be generated by \projecttitle{} with access to the secret key(s), and since the hardware  includes the ID in any attestation, no other party can have generated the attestation. because each device is uniquely idetified the keys are secret and each \projecttitle{} device has unique identifier.

Formally, we define the following lemmas: \emph{(i)} this message was sent by an authentic \projecttitle{} device in a valid configuration \emph{(ii)} there is no message that was sent before, but not accepted \emph{(iii)} there is no message that was sent after, but accepted before this one \emph{(iii)} this message has not been accepted before.

Tamarin, again, found at least one trace for every control state and proved that there is no trace to any illegal state in this extended model. Hence transferable authentication holds for our model and the counters behave as expected to ensure non-equivocation. 


%This simple attestation kernel achieves to ensure the properties of non-equivocation and transferable authentication. First, \projecttitle{} attestation kernel prevents equivocation by ensuring that two attestations of different messages
%will never be assigned identical {\tt send\_cnts}. The property is ensured because the {\tt send\_cnts} are never decremented. Secondly the \projecttitle{} ensures the transferable authentication because the cryptosystem is not broken, the keys are secret and each \projecttitle{} device has unique identifier.

==> backups/t-nic-network-lib.bak.tex <==
\section{Trusted Network Library}
\label{sec:t-nic-software}
The section provides an overview of the \projecttitle{} programming APIs ($\S$~\ref{sec:net-lib}) as well as an example of a generic protocol translation ($\S$~\ref{subsec:transformation}).

\subsection{Programming APIs}
\label{sec:net-lib}
\projecttitle{} implements a programming API that  resembles the traditional programming frameworks on top of the classical RDMA API that improve adoption~\cite{erpc}. Our API, shown in Table~\ref{tab:apis}, allows system designers to leverage modern RDMA-enabled networks as they have been proven to be the most efficient design in modern distributed systems\cite{f04eb9b864204bab958e72055062748c, farm, hermes, rdma-design, rdma-scale, octopus, Mitchell2013}. In addition, our \projecttitle{} API extends the security semantics of the traditional RDMA operations materializing the minimum necessary security properties required for robust replication, i.e.,  transferable authentication and non-equivocation (discussed in $\S$~\ref{sec:background}). 

%We specifically provide a unified abstraction where we designed and implemented peer-to-peer and group communication primitives that follow the standardized classical and widely-adopted~\cite{f04eb9b864204bab958e72055062748c, farm, hermes, rdma-design, rdma-scale, octopus, Mitchell2013} RDMA API.





%The local virtual address and the are also passed by the user.


\if 0
\begin{center}
\begin{table*}[ht]
\centering
\begin{tabular}{ |m{3.4cm}||m{12cm}|}
 \hline
 \multicolumn{2}{|c|}{{\bf Initialization API}} \\
 \hline
 \texttt{init\_local\_queue()} & \\
 \texttt{init\_connection()} & \dimitra{write me} \\
 \hline
 \texttt{send\_pk()} &  \\
 \hline
 \multicolumn{2}{|c|}{{\bf Network API}} \\
 \hline
 \texttt{remote\_write()} &  \\
 \texttt{remote\_read()} &  \\
 \texttt{send()} &  \\
 \hline
 \texttt{poll()}&  \\
  \hline
  \multicolumn{2}{|c|}{{\bf Security API}} \\
 \hline
 \texttt{check\_attestation()} &  \\
 \hline
 \end{tabular}
\caption{\projectlibrary{} API.}
\end{table*}\label{table:api}
\end{center}

Table~\ref{table:api} shows the core API implemented by our \projectlibrary{}.
\fi

\myparagraph{Initialization API}  Prior to exchanging network messages, the \projecttitle{} system needs to be configured by the application to establish RDMA connections. Specifically, the application creates one ibv struct for each peer-to-peer connection {\tt ibv\_qp\_conn()} which sets up and stores the queue pair, the local and remote IP addresses, and device UDP ports and others. In addition, the application needs to allocate the ibv memory that will be registered to the \projecttitle{} hardware. The code calls into the {\tt init\_lqueue()} that initializes the local queue pairs and  registers the ibv memory to the \projecttitle{}. Once the application configures its \projecttitle{} appropriately, it synchronizes itself with the remote side using the {\tt ibv\_sync()}. This function utilizes a common NIC to communicate with the remote machine and exchange important information such as its registered memory base address, queue pair numbers, etc. After all these steps are completed the application can use the \projecttitle{} network API to exchange data in a secure manner. %In addition, the application needs to exchange its registered memory base address ({\tt exchange\_qp()}) with a remote machine. 

\begin{table}
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 \multicolumn{2}{|c|}{{\bf Initialization API}} \\ [0.5ex] \hline 
 {\tt ibv\_qp\_conn()} & Creates an ibv struct \\
 {\tt alloc\_mem()}    & Allocates host ibv memory \\
 {\tt init\_lqueue()}    & Registers local memory to \projecttitle{} \\
% {\tt exchange\_qp()} & Connects with remote IPs \\
 {\tt ibv\_sync()} & Exchanges ibv memory addresses \\
 %{\tt add\_qp()} &  $2f+1$ \\
 \hline
 \hline
 \multicolumn{2}{|c|}{{\bf Network API}} \\ [0.5ex] \hline 
 {\tt local\_send()}    & Generates an attested message \\
 {\tt local\_verify()}    & Verifies a message \\
 {\tt auth\_send()} &  Transmits an attested message \\
 {\tt poll()} &  Polls for incoming messages \\
 {\tt rem\_read/write()} &  Fetches/writes remote memory \\
 \hline
  %\hline
 %\multicolumn{2}{|c|}{{\bf Configuration API}} \\ [0.5ex] %\hline 
 %{\tt secrets()}    & (shared) keys' exchange \\
 %\hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{\projecttitle{} programming API.}
\label{tab:apis}
%\vspace{-18pt}
\end{table}




\myparagraph{Network API} Our network API adopts the programming paradigm of high-performant general libraries on top of RDMA~\cite{erpc} on top of the one-sided RDMA-verbs~\cite{rdma}. Specifically, \projecttitle{} executes shielded one-sided RDMA reliable operations that offer the same reliability guarantees as the classical one-sided RDMA over Reliable Connection (RC). The networking stack imposes a FIFO ordering (per connection), similar to TCP/IP networking.

We expose to the user the {\tt auth\_send()} operation which sends an attested message by implementing an RDMA reliable write of the message concatenated with its attestation. We also support the classical RDMA operations for reads and writes. The remote side can {\tt poll()} to fetch the number of the completed operations. In contrast to classical RDMA we have not used background threads for polling. The function returns the number of the completed operations. The poll function is only updated when the verification at the \projecttitle{} hardware has been successful. 

In addition, we implemented local operations where we generate or verify an attested message without transmitting in the network. The local attestations and verification's pass through the \projecttitle{} hardware and are copied back to host local memory.

In \projecttitle{}, we do not implement a hardware-assisted multicast. Even in the standard RDMA libraries, hardware-based multicast is barely used in practice~\cite{f04eb9b864204bab958e72055062748c} and is only supported only over unreliable connections. In \projecttitle{}, we can support equivocation-free multicast through uni-casts of the same attested message generated by {\tt local\_send()} as in~\cite{levin2009trinc}.

\if 0
Compared to classical, little-adopted, RDMA that only supports h/w multicast for unreliable connections~\cite{f04eb9b864204bab958e72055062748c}, \projecttitle{} allows for multicast reliable operations that prevent equivocation. However, we have not implemented multicast on hardware. Instead, multicasts in \projecttitle{} can be implemented through unicasts of the same attested message generated by {\tt local\_send()}.
\fi

%\myparagraph{Authentication API} All \trustedfpga{}s in the membership have exchanged keys as part of their initialization. Applications can request the public keys of their local and/or remote \trustedfpga{}s to verify the attestation of a received message (if it is required by the protocol).





\subsection{A Generic Transformation Recipe}
\label{subsec:transformation}
We now show how to use \projecttitle{} programming API to construct a generic transformation of a distributed system operating under the CFT model to a system that targets Byzantine settings.  Our transformation is defined as a set of wrapper functions on top of the send and receive operations~\cite{clement2012}. For safety, our transformation further needs to meet the following properties in order to provide the same guarantees that are expected by the original CFT system~\cite{clement2012, making_distributed_app_rob, 268272}.

\begin{itemize}
    \item \myparagraph{Safety} If the sender $S$ is correct and a correct receiver receives a message $m$ from $S$, then the sender $S$ must have executed send with $m$.
    \item \myparagraph{Integrity} If a correct receiver receives and delivers a message $m$, then $m$ is a valid (state machine) message.
\end{itemize}

Listing~\ref{lst:transformation} shows our proposed generic send and receive operations that we applied in a scenario between two nodes where the first node (sender) sends messages to the second node (receiver) that follows the sender. For each message the sender (executes the {\tt send}) needs to send the (client) msg, its current state (e.g., sender's output as a response to the current client msg) and  the follower's previous state known to the sender. The last piece of data is optional and can be used to ensure that both the sender and the receiver have the same view of the system (Listing~\ref{lst:transformation}:L4-6). The receiver, on the other hand, needs to {\em simulate} the leader's state and upon a valid message reception (Listing~\ref{lst:transformation}:L12-13), it needs to verify that the sender's output/state is the expected (Listing~\ref{lst:transformation}:L14). To ensure that the receiver is not lagging behind, it might also want to ensure that it is in the same view with the leader. To achieve so it verifies that its latest sent message has been received by the leader (Listing~\ref{lst:transformation}:L15-16).

\myparagraph{Correctness arguments for the transformation} Next we explain how our generic transformation satisfies the listed above requirements. First, the safety requirement is directly ensured by \projecttitle{} transferable authentication property. Since a faulty node cannot impersonate a correct node, if \projecttitle{} validates and delivers a message m from a sender, then the sender must have send m. Thanks to our  reliable network operations where the \projecttitle{} hardware will retry the send attempts (transparently to the application), liveness between correct nodes is ensured. 

%by attaching the corresponding  authentication tokens of pi’s inputs that led to sending the output message.
The integrity property requires the follower to obtain a guarantee that a message from the leader has been derived from a valid protocol execution scenario. In our transformation, the follower simulates the leader's state and jointly with the transferable authentication mechanism, we can always prove the validity of leader's output and state. Following this, the integrity requirement is met in the follower by replaying the client msg and verifying that the sender's output is legitimate.

For the case of the replication protocols we further require the following property.
\begin{itemize}
\item \myparagraph{Consistency (for replication protocols)} If correct replicas $R_1$ and $R_2$ receive valid messages $m_i$ and $m_j$  respectively from sender $S$, then either (a) $Bpg_{,i}$ is a prefix of $Bpg_{,j}$ , (b) $Bpg_{,j}$ is a prefix of $Bpg_{,i}$, or (c) $Bpg_{,i}$ = $Bpg_{,j}$ (where $Bpg_{,x}$ is the process behavior that supports the validity of message $m_x$).
\end{itemize}

The consistency requirement is seamlessly enforced  through the \projecttitle{} non-equivocation primitive. Our approach to prevent equivocation requires \projecttitle{} to  register a monotonic sequence number to each outgoing message. This enforces a total order on the leader's messages and along with the integrity requirement this is sufficient to consistently. Importantly, we ensure that correct followers/receivers will never miss any past messages. As such, when two followers receive from the same sender (using the equivocation-free multicast we discuss in $\S$~\ref{subsec:net_lib}) they will follow the exact same transition path. %By forcing the sender to also transmit all its state and previous known message from the receiver, the receiver can validate detect missing messages and inconsistencies in each communication step.


%Resultantly, when two receivers p1 and p2 hear
%from the same sender pg their behaviors corresponding to the
%sender pg will follow the exact same state transition path.
%However, as pg may not send all messages, a behavior of
%process (say) p1 can form a prefix of a behavior by process
%p2, and vice versa.

{\small
\begin{lstlisting}[frame=h,style=customc,
                    label={lst:transformation},
                    caption= Generic application send and recv wrapper functions for transformation using \projecttitle{}: blue sections (native) and orange sections (\projecttitle additions).]
// generic send wrapper function
void send(P_id, char[] msg) {
    // current state
@\Hilight@    state = hash(my_state);
@\Hilight@    to_be_sent = msg || state || prev_receiver_msg;
@\HilightYlinewidth@    auth_send(follower, to_be_send);
}

// upon receiveing a send(follower, msg) message
void recv(msg) {
@\HilightYlinewidth@ // message authenticity and integrity checked in TNIC hw
auto [attestation, msg || state || prev_receiver_msg] = deliver();
@\HilightYlinewidth@    [msg, cnt] = verify_msg(recv_msg);
@\Hilight@    verify_sender_state(state);
@\HilightYlinewidth@    local_verify(prev_receiver_msg);
@\Hilight@    verify_system_view(prev_receiver_msg);
@\Hilight@    apply(msg);
}
\end{lstlisting}
}

==> backups/t-nic-network-lib.bak2.tex <==
\section{Trusted Network Library}
\label{sec:t-nic-software}
The section provides an overview of the \projecttitle{} programming APIs ($\S$~\ref{sec:net-lib}) as well as an example of a generic protocol translation ($\S$~\ref{subsec:transformation}).

\subsection{Programming APIs}
\label{sec:net-lib}
\projecttitle{} implements a programming API that resembles the traditional programming frameworks on top of the classical RDMA API that improves adoption~\cite{erpc}. Our API, shown in Table~\ref{tab:apis}, allows system designers to leverage modern RDMA-enabled networks as they have been proven to be the most efficient design in modern distributed systems\cite{f04eb9b864204bab958e72055062748c, farm, hermes, rdma-design, rdma-scale, octopus, Mitchell2013}. 

In contrast to traditional RDMA operations, our \projecttitle{} API extends the security semantics offering the properties of non-equivocation and transferable authentication as the lower bound to build trustworthy distributed systems ($\S$~\ref{subsec:trustworthy_ds}).

%We specifically provide a unified abstraction where we designed and implemented peer-to-peer and group communication primitives that follow the standardized classical and widely-adopted~\cite{f04eb9b864204bab958e72055062748c, farm, hermes, rdma-design, rdma-scale, octopus, Mitchell2013} RDMA API.





%The local virtual address and the are also passed by the user.


\if 0
\begin{center}
\begin{table*}[ht]
\centering
\begin{tabular}{ |m{3.4cm}||m{12cm}|}
 \hline
 \multicolumn{2}{|c|}{{\bf Initialization API}} \\
 \hline
 \texttt{init\_local\_queue()} & \\
 \texttt{init\_connection()} & \dimitra{write me} \\
 \hline
 \texttt{send\_pk()} &  \\
 \hline
 \multicolumn{2}{|c|}{{\bf Network API}} \\
 \hline
 \texttt{remote\_write()} &  \\
 \texttt{remote\_read()} &  \\
 \texttt{send()} &  \\
 \hline
 \texttt{poll()}&  \\
  \hline
  \multicolumn{2}{|c|}{{\bf Security API}} \\
 \hline
 \texttt{check\_attestation()} &  \\
 \hline
 \end{tabular}
\caption{\projectlibrary{} API.}
\end{table*}\label{table:api}
\end{center}

Table~\ref{table:api} shows the core API implemented by our \projectlibrary{}.
\fi

\myparagraph{Initialization API}  Prior to exchanging network messages, the \projecttitle{} system needs to be configured by the application to establish RDMA connections. Specifically, the application creates one ibv struct for each peer-to-peer connection {\tt ibv\_qp\_conn()} which sets up and stores the queue pair, the local and remote IP addresses, device UDP ports, and others. In addition, the application needs to allocate the ibv memory that will be registered to the \projecttitle{} hardware. The code calls into the {\tt init\_lqueue()} that initializes the local queue pairs and registers the ibv memory to the \projecttitle{}. Once the application configures its \projecttitle{} appropriately, it synchronizes itself with the remote side using the {\tt ibv\_sync()}. This function utilizes a common NIC to communicate with the remote machine and exchange important information such as its registered memory base address, queue pair numbers, etc. After all these steps are completed, the application can use the \projecttitle{} network API to exchange data in a secure manner. %In addition, the application needs to exchange its registered memory base address ({\tt exchange\_qp()}) with a remote machine. 

\begin{table}
\begin{center}
\begin{tabular}{ |c|c| } 
 \hline
 \multicolumn{2}{|c|}{{\bf Initialization API}} \\ [0.5ex] \hline 
 {\tt ibv\_qp\_conn()} & Creates an ibv struct \\
 {\tt alloc\_mem()}    & Allocates host ibv memory \\
 {\tt init\_lqueue()}    & Registers local memory to \projecttitle{} \\
% {\tt exchange\_qp()} & Connects with remote IPs \\
 {\tt ibv\_sync()} & Exchanges ibv memory addresses \\
 %{\tt add\_qp()} &  $2f+1$ \\
 \hline
 \hline
 \multicolumn{2}{|c|}{{\bf Network API}} \\ [0.5ex] \hline 
 {\tt local\_send()}    & Generates an attested message \\
 {\tt local\_verify()}    & Verifies a message \\
 {\tt auth\_send()} &  Transmits an attested message \\
 {\tt poll()} &  Polls for incoming messages \\
 {\tt rem\_read/write()} &  Fetches/writes remote memory \\
 \hline
  %\hline
 %\multicolumn{2}{|c|}{{\bf Configuration API}} \\ [0.5ex] %\hline 
 %{\tt secrets()}    & (shared) keys' exchange \\
 %\hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{\projecttitle{} programming API.}
\label{tab:apis}
%\vspace{-18pt}
\end{table}




\myparagraph{Network API}
\projecttitle{} executes shielded one-sided RDMA reliable operations that offer the same reliability guarantees as the classical one-sided RDMA over Reliable Connection (RC). The networking stack imposes a FIFO ordering (per connection), similar to TCP/IP networking.

We expose to the user the {\tt auth\_send()} operation which sends an attested message by implementing an RDMA reliable write of the message concatenated with its attestation. We also support the classical RDMA operations for reads and writes. The remote side can {\tt poll()} to fetch the number of the completed operations. In contrast to classical RDMA we have not used background threads for polling. The function returns the number of the completed operations. The poll function is only updated when the verification at the \projecttitle{} hardware has been successful.  \projecttitle{} offers local operations for generating and verifying attested messages within a single-node setup.


%In addition, we implemented local operations where we generate or verify an attested message without transmitting in the network. The local attestations and verification's pass through the \projecttitle{} hardware and are copied back to the host's local memory.

%\atsushi{E.g., TNIC does not support a hardware-assisted multicast.}
\projecttitle{} does not support a hardware-assisted multicast. Even in the standard RDMA libraries, hardware-based multicast is barely used in practice~\cite{f04eb9b864204bab958e72055062748c} whereas it is only supported only over unreliable connections. However, \projecttitle{} can support equivocation-free multicast through uni-casts of the same attested message generated by {\tt local\_send()} as in~\cite{levin2009trinc}.

\if 0
Compared to classical, little-adopted, RDMA that only supports h/w multicast for unreliable connections~\cite{f04eb9b864204bab958e72055062748c}, \projecttitle{} allows for multicast reliable operations that prevent equivocation. However, we have not implemented multicast on hardware. Instead, multicasts in \projecttitle{} can be implemented through unicasts of the same attested message generated by {\tt local\_send()}.
\fi

%\myparagraph{Authentication API} All \trustedfpga{}s in the membership have exchanged keys as part of their initialization. Applications can request the public keys of their local and/or remote \trustedfpga{}s to verify the attestation of a received message (if it is required by the protocol).





\subsection{A Generic Transformation Recipe}
\label{subsec:transformation}
\myparagraph{Transformation properties} We now show how to use \projecttitle{} programming API to construct a generic transformation of a distributed system operating under the CFT model to a system that targets Byzantine settings.  Our transformation is defined as a set of wrapper functions on top of the send and receive operations~\cite{clement2012}. For safety, our transformation further needs to meet the following properties in order to provide the same guarantees that are expected by the original CFT system~\cite{clement2012, making_distributed_app_rob, 268272}.

\begin{itemize}
    \item \myparagraph{Safety} If the sender $S$ is correct and a correct receiver receives a message $m$ from $S$, then the sender $S$ must have executed send with $m$.
    \item \myparagraph{Integrity} If a correct receiver receives and delivers a message $m$, then $m$ is a {\em valid} message.
\end{itemize}

Listing~\ref{lst:transformation} shows our proposed generic {\tt send} (Listing~\ref{lst:transformation}:L2-7) and {\tt recv} (Listing~\ref{lst:transformation}:L10-18) operations that we applied in a scenario between two nodes where the first node (sender) receives client requests and forwards the requests to the second node (receiver) who is following the sender. For each transmitted message ({\tt tx\_msg}), the sender sends the (client) msg, its current state (e.g., sender's output as a response to the current client msg), and the follower's previous state known to the sender. The last piece of data is optional depending on the consistency guarantees of the derived system and can be used to ensure that both the sender and the receiver have the same view of the system (Listing~\ref{lst:transformation}:L4-6). 

The receiver, on the other hand, {\em simulates} the sender's state to verify its actions. Importantly, upon a valid message reception (Listing~\ref{lst:transformation}:L12-13), the receiver verifies that the sender's action as a response to the client request is the expected (Listing~\ref{lst:transformation}:L14). In addition, the receiver ensures that it is not lagging behind and it has the same ``view'' of the system inputs as the sender by verifying that the sender has {\em seen} the receiver's latest sent message (Listing~\ref{lst:transformation}:L15-16).


{\small
\begin{lstlisting}[frame=h,style=customc,
                    label={lst:transformation},
                    caption= Generic application send and recv wrapper functions for transformation using \projecttitle{}: blue sections (native) and orange sections (\projecttitle additions).]
// generic send wrapper function
void send(P_id, char[] msg) {
    // current state
@\Hilight@    state = hash(my_state);
@\Hilight@    tx_msg = msg || state || prev_receiver_msg;
@\HilightYlinewidth@    auth_send(follower, tx_msg);
}

// upon receiving a send(follower, msg) message
void recv(recv_msg) {
@\HilightYlinewidth@ // message authenticity and integrity checked in TNIC hw
auto [attestation, msg || state || prev_receiver_msg] = deliver();
@\HilightYlinewidth@    [msg, cnt] = verify_msg(msg);
@\Hilight@    verify_sender_state(state);
@\HilightYlinewidth@    local_verify(prev_receiver_msg);
@\Hilight@    verify_system_view(prev_receiver_msg);
@\Hilight@    apply(msg);
}
\end{lstlisting}
}


\myparagraph{Correctness arguments for the transformation} Next we explain how our generic transformation recipe satisfies the listed above requirements. First, the safety requirement is directly satisfied by \projecttitle{}'s transferable authentication property. A faulty node cannot impersonate a correct node; if \projecttitle{} validates and delivers a message $m$ from a sender, then the sender must have sent $m$. \projecttitle{} reliable network operations, where the \projecttitle{} hardware transparently retries failed sends ensures liveness properties between correct nodes. 

%by attaching the corresponding  authentication tokens of pi’s inputs that led to sending the output message.
The integrity property requires the receiver to obtain a guarantee that a message from the sender has been derived from a valid execution scenario of the business logic. In our transformation, the follower simulates the leader's state and jointly with the transferable authentication mechanism, we can always prove the integrity and the validity of sender's output and state. %Following this, the integrity requirement is met in the receiver by replaying the client msg and verifying that the sender's output is legitimate.

% \atsushi{Why is this 3rd property shown here, far from the other two properties? -> Now I understand; ignore this.}

\myparagraph{Consistency property for replication} Since \projecttitle{} aims to provide a general approach to transform distributed systems for Byzantine settings it also needs to ensure the consistency property as an additional property to be met for the specific case of the CFT replication protocols~\cite{clement2012}.
\begin{itemize}
\item \myparagraph{Consistency} If correct replicas $R_1$ and $R_2$ receive valid messages $m_i$ and $m_j$  respectively from sender $S$, then either (a) $Bpg_{,i}$ is a prefix of $Bpg_{,j}$ , (b) $Bpg_{,j}$ is a prefix of $Bpg_{,i}$, or (c) $Bpg_{,i}$ = $Bpg_{,j}$ (where $Bpg_{,x}$ is the process behavior that supports the validity of message $m_x$).
\end{itemize}

The consistency requirement is enforced through the \projecttitle{}'s non-equivocation primitive. \projecttitle{} tackles with equivocation by assigning  a (unique) monotonic sequence number to each outgoing message. Consequently, \projecttitle{} enforces a total order on the leader's outgoing messages which along with the integrity requirement is sufficient for the consistency guarantees. Importantly, \projecttitle{} ensures that correct followers/receivers cannot miss any past messages. Following this, two followers that receive from the same leader/sender (using the equivocation-free multicast we discuss in $\S$~\ref{subsec:net_lib}) they will follow the exact same transition (execution) path. %By forcing the sender to also transmit all its state and previous known message from the receiver, the receiver can validate detect missing messages and inconsistencies in each communication step.


%Resultantly, when two receivers p1 and p2 hear
%from the same sender pg their behaviors corresponding to the
%sender pg will follow the exact same state transition path.
%However, as pg may not send all messages, a behavior of
%process (say) p1 can form a prefix of a behavior by process
%p2, and vice versa.


==> backups/t-nic-network.bak.tex <==
\section{Trusted Network Stack}
\label{sec:t-nic-network}


\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.5\textwidth]{figures/trusted-nic-overview.drawio.pdf}
    \includegraphics[width=0.5\textwidth]{figures/trusted_nic_overview_lat-network_stack_system_design.drawio-1.pdf}
    \caption{\projecttitle{} system network stack.}
    \label{fig:network_stack_design}
\end{figure}


We build a software \projecttitle{} system network stack that operates as the {\em middle layer} between the \projecttitle{} programming APIs (see $\S$~\ref{sec:net-lib}) and the hardware implementation of \projecttitle{}. Figure~\ref{fig:network_stack_design} shows the overview of \projecttitle{}'s system network stack design. Specifically, \projecttitle{} system stack comprised of two core components: {\em (1)} the \projecttitle{} driver and the mapped REGs pages that are responsible for the configuration (shown in dashed lines) and host---device communication respectively and {\em (2)} the RDMA OS abstractions that executes networking operations. 

\subsection{\projecttitle{} Driver and Mapped REGs pages} 

The \projecttitle{} driver is invoked at the initialization of the device to make the appropriate configurations of the \projecttitle{} hardware.  To achieve that, it loads a kernel module that sets up the device and provides its static configuration, specifically the device MAC address, the device QSFP port and a (configurable) network IP that is used by the application code to exchange messages. 

The driver additionally provides an implementation of the {\tt mmap} system call as part of its {\tt file\_operations structure}~\cite{device_drivers} to reserve and map the device to a user-space addresses range. We refer to these mappings with the term Mapped REGs pages. In our \projecttitle{} we reserve one page of 4KB that equals the page granularity of our system for each connected device and are represented as pseudo-devices in {\tt /dev/fpga<ID>}. Specifically, accessing and writing to the pseudo-device equals to accessing the control and status registers of the FPGA. As such the software system stack, and consequently the applications, can directly intact with the control path of the \projecttitle{} hardware at low latency bypassing the operating system. 

These device mappings also expose the control registers for the  transmission/reception queues. In our current \projecttitle{} configuration, the depth is set to 22. If the queues are full, the ibv library temporarily blocks and continuously monitors the queues for finding empty slots.  The application pass down to the device any requests and their related parameters whereas the ibv library encodes and stores to the pages the following data request opcode, queue id and other identifiers, remote and local offset and data len. %The \projecttitle{} hardware network stack decodes the metadata and parameters into the  update the pages entries about the completed requests and other statistics.

\subsection{RDMA OS Abstractions} The RDMA OS abstractions is a user-space library that enables the networking operations in the \projecttitle{} hardware bypassing the kernel for performance. As shown in Figure~\ref{fig:network_stack_design}, the application is using the \projecttitle{} programming API that calls into the RDMA OS library to materialize the networking operations. The blue colored lines show the data path that operate on a separate bus from the control path (black lines). The RDMA OS abstractions system stack overall is comprised of two parts, the network (RDMA) library that is colored in purple in Figure~\ref{fig:network_stack_design} (e.g., ibv library, ibv structs and ibv memory) and the OS library that is colored in red in Figure~\ref{fig:network_stack_design} (process and scheduler libraries).

\myparagraph{Network (RDMA) library} The network (RDMA) library includes all the logic and the data structures required for implementing the RDMA protocol. The ibv library is executing the application's networking operations by posting the requests to the hardware. Specifically, it creates an internal representation of the request and the associated data and metadata (i.e. request opcode, remote IP, local address, remote base address and offset, data length, etc.) encodes all related parameters and writes them in their specific offsets in the REGs pages to update the control registers in the \projecttitle{} hardware. The \projecttitle{} decodes the inputs to execute the appropriate RDMA protocol. Similarly to the classical RDMA implementation, the ibv structs manage all the connections' internal metadata, such as queues per connection, local and remote memory addresses, rkeys, etc. 

As shown in Figure~\ref{fig:network_stack_design}, the submission and reception of
requests and responses mandate the allocation of application network
buffers. The \projecttitle{} system stack follows the memory management design that has already been established in widely direct network I/O libraries~\cite{erpc, dpdk, rdma} for performance. Specifically, in \projecttitle{} application network buffers need to be mapped to a specific \projecttitle{}-memory, called the ibv memory. The ibv memory is allocated at the connection creation by the application through the ibv library. It resides within the application's address space with full read/write permissions and it is registered to the \projecttitle{} for remote reads and writes without involving the CPU.

Applications should wisely use this memory to eliminate unnecessary data copies from  applications' buffers to network buffers. Specifically, while applying \projecttitle{} into four systems and use-cases ($\S$~\ref{sec:use_cases}), we allocated all application buffers from the ibv memory, hence the network buffers (registered RDMA memory). In \projecttitle{} the ibv memory buffers is allocated in the {\tt huge page} memory area (2MB) and is available for DMA transfers from and to the \projecttitle{} hardware.  



\myparagraph{OS library} The OS library in \projecttitle{} implements the scheduling and coordination of the application threads regarding the network operations and \projecttitle{} device access. Specifically, each \projecttitle{} device is represented by one or more \projecttitle{}-processes (process library) depending on the number of applications that are using the device. The \projecttitle{}-process in \projecttitle{} is not a separate  scheduling entity (i.e., a thread as in classical OSes). In contrast, it is an object handle managed by the scheduler library (in Figure~\ref{fig:network_stack_design}) that acquires locks on the respective REG pages and invokes data transfers and network operations. Specifically, when the scheduler marks the the \projecttitle{}-process as eligible for execution, the process can write the request's data and metadata in its associated offset in the corresponding REG page. The scheduler library in \projecttitle{} is lightweight and its core responsibility is to ensure that the access to the mapped REG pages, hence the device, are executed in an isolated way. For performance, the data to be sent (blue lines) is never copied across \projecttitle{} system stack, instead, the \projecttitle{}-process only sets the necessary encoded metadata to the REGs pages and directly posts the command in the first available command slot. As discussed, the \projecttitle{} hardware will later fetch the data from the ibv memory through a DMA transfer (blue lines in the Figure~\ref{fig:network_stack_design}).

%Upon a transmission the {\tt ibv library} which is creates an internal representation of the request and the associated data and metadata (i.e. request opcode, remote IP, local address, remote base address and offset, data lenght, etc.). Then the request is executed as part of a (virtual) process that is mapped to a specific id ({\tt pid}) similar to the classical OS process abstraction. When the scheduler marks the process as eligible for execution, the process writes the request's data and metadata in its associated REG page. To improve for performance the actual data to be sent are not copied within all the system stack, instead, the process writes the local address and the length of the data (in bytes) to be sent and posts the command. The {\dimitra{;....}}


==> backups/t-nic-network.bak2.tex <==
\section{Trusted Network Stack}
\label{sec:t-nic-network}


\begin{figure}[t!]
    \centering
    %\includegraphics[width=0.5\textwidth]{figures/trusted-nic-overview.drawio.pdf}
    \includegraphics[width=0.45\textwidth]{figures/network_stack_system_design.drawio.pdf}
    \caption{\projecttitle{} system network stack.}
    \label{fig:network_stack_design}
\end{figure}


We build a software \projecttitle{} system network stack that operates as the {\em middle layer} between the \projecttitle{} programming APIs (see $\S$~\ref{sec:net-lib}) and the hardware implementation of \projecttitle{}. Figure~\ref{fig:network_stack_design} shows the overview of \projecttitle{}'s system network stack design that is comprised of two core components: {\em (1)} the \projecttitle{} driver and the mapped REGs pages that are responsible for configuring the device at the initialization and host---device communication respectively, and {\em (2)} the RDMA OS abstractions that execute networking operations. 

\subsection{\projecttitle{} Driver and Mapped REGs Pages} 

%\atsushi{What's the meaning of "the appropriate configurations"? Also, explaining a device driver might be a bit boring}
The \projecttitle{} driver is invoked at the initialization of the device, prior to the remote attestation protocol ($\S$~\ref{subsec:nic_controller}), to configure the \projecttitle{} hardware with its static configuration (the device MAC address, the device QSFP port, and the network IP used by the application). 
%To achieve that, it loads a kernel module that sets up the device and provides its static configuration, specifically the device MAC address, the device QSFP port, and a (configurable) network IP that is used by the application code to exchange messages. 

Additionally, the driver enables kernel-bypass networking---similarly to the original (user-space) RDMA protocol---by mapping the \projecttitle{} device to a user-space addresses range, the Mapped REGs pages. In our \projecttitle{}, we reserve one page at the page granularity of our system for each connected device that are represented as pseudo-devices in {\tt /dev/fpga<ID>}. Read and write access to the pseudo-device is equal to accessing the control and status registers of the FPGA. As such, the applications can directly intact with the control path of the \projecttitle{} hardware at low latency while bypassing the operating system. 

%\atsushi{The implementation optimization shown here can be simplified or omitted (not so bad, but may be less prioritized)}
%The driver additionally provides an implementation of the {\tt mmap} system call as part of its {\tt file\_operations structure}~\cite{device_drivers} to reserve and map the device to a user-space addresses range. We refer to these mappings with the term Mapped REGs pages. In our \projecttitle{}, we reserve one page of 4KB that equals the page granularity of our system for each connected device and are represented as pseudo-devices in {\tt /dev/fpga<ID>}. Specifically, accessing and writing to the pseudo-device is equal to accessing the control and status registers of the FPGA. As such, the software system stack, and consequently the applications, can directly intact with the control path of the \projecttitle{} hardware at low latency while bypassing the operating system. 

%\atsushi{Very implementation-specific, so we can simplify them; not explain how we implement, but what the device driver does.}
%These device mappings also expose the control registers for the transmission/reception queues. In our current \projecttitle{} configuration, the depth is set to 22. If the queues are full, the ibv library temporarily blocks and continuously monitors the queues to find empty slots.  The application passes down to the device any requests and their related parameters, whereas the ibv library encodes and stores to the pages the following data request opcode, queue id and other identifiers, remote and local offset, and data len. %The \projecttitle{} hardware network stack decodes the metadata and parameters into the  update the pages entries about the completed requests and other statistics.

\subsection{RDMA OS Abstractions} 
%\atsushi{Overall: can we highlight what functionalities the OS abstractions enable rather than how they are implemented?}
The RDMA OS abstractions are a user-space library that enables the networking operations in the \projecttitle{} hardware bypassing the kernel for performance. As shown in Figure~\ref{fig:network_stack_design}, invocations of the \projecttitle{} programming API calls into the RDMA OS library are comprised of two parts: \textit{the network (RDMA) library} (colored in purple) that implements the software part of the RDMA protocol, and \textit{the OS library} (colored in red) that schedules the \projecttitle{} requests.


\myparagraph{Network (RDMA) library}  The network (RDMA) library includes all the logic and data (e.g., the queues per connection, the local and remote memory addresses, the RDMA keys that denote the memory access permissions) required for implementing the RDMA protocol. It executes the application's networking operations by posting the requests to the hardware. More specifically, it creates an internal representation of the request and the associated data and metadata (i.e., request opcode, remote IP, local address, remote base address, offsets, data length, etc.), it encodes all related parameters and, finally, it writes them in specific offsets in the REGs pages to update the control registers of \projecttitle{} hardware. In case there are no empty transmission queues, the ibv library {\tt yields} until there is an empty slot in the queue.

%These device mappings also expose the control registers for the transmission/reception queues. In our current \projecttitle{} configuration, the depth is set to 22. If the queues are full, the ibv library temporarily blocks and continuously monitors the queues to find empty slots.  The application passes down to the device any requests and their related parameters, whereas the ibv library encodes and stores to the pages the following data request opcode, queue id and other identifiers, remote and local offset, and data len.

%The \projecttitle{} decodes the inputs to execute the appropriate RDMA protocol. The ibv library manages the ibv structs manage that store all the connections' internal metadata, such as queues per connection, local and remote memory addresses, rkeys, etc. 

As shown in Figure~\ref{fig:network_stack_design}, the transmission and reception of requests and responses mandate the allocation of application network buffers. We adopt similar memory management as in widely-used user-space networking libraries~\cite{erpc, dpdk, rdma}. Importantly, in \projecttitle{} application network buffers need to be mapped to a specific \projecttitle{}-memory, called the ibv memory. The ibv memory area is allocated at the connection creation in the {\tt huge page} area by the application through the ibv library. It resides within the application's address space with full read/write permissions, it is eligible for DMA transfers and it is registered to the \projecttitle{} for remote reads and writes without involving the CPU. 

%Applications should wisely use this memory to eliminate unnecessary data copies from applications' buffers to network buffers. Specifically, while applying \projecttitle{} into four systems and use-cases ($\S$~\ref{sec:use_cases}), we allocated all application buffers from the ibv memory, hence the network buffers (registered RDMA memory). In \projecttitle{}, the ibv memory buffers are allocated in the {\tt huge page} memory area (2MB) and available for DMA transfers from and to the \projecttitle{} hardware.  


\myparagraph{OS library} The \projecttitle{}-OS library is a lightweight user-space library that is responsible for scheduling the \projecttitle{} requests and ensuring isolated access to the mapped REG pages, hence the device. To improve performance, the \projecttitle{} data path eliminates unnecessary data copies throughout the network stack. In fact, the data to be sent (shown in blue lines in Figure~\ref{fig:network_stack_design} is directly fetched from the hardware through DMA transfers. 

The OS library creates a \projecttitle{}-process object to represent each \projecttitle{} device.  This \projecttitle{}-process in \projecttitle{} is not a separate scheduling entity (i.e., a thread as in classical OSes). In contrast, it is an object handle, exposed to the ibv library but managed by the \projecttitle{}-OS library that manages and acquires locks on the respective REG pages to ensure isolated access to the \projecttitle{} hardware.




%never copied across \projecttitle{} system stack; instead, the \projecttitle{}-process only sets the necessary encoded metadata to the REGs pages and directly posts the command in the first available command slot. As discussed, the \projecttitle{} hardware will later fetch the data from the ibv memory through a DMA transfer (blue lines in Figure~\ref{fig:network_stack_design}).

%Upon a transmission the {\tt ibv library} which is creates an internal representation of the request and the associated data and metadata (i.e. request opcode, remote IP, local address, remote base address and offset, data lenght, etc.). Then the request is executed as part of a (virtual) process that is mapped to a specific id ({\tt pid}) similar to the classical OS process abstraction. When the scheduler marks the process as eligible for execution, the process writes the request's data and metadata in its associated REG page. To improve for performance the actual data to be sent are not copied within all the system stack, instead, the process writes the local address and the length of the data (in bytes) to be sent and posts the command. The {\dimitra{;....}}


==> related_work2.tex <==
\subsection{\revcont{Discussion}}
\myparagraph{\rev{B2}{\projecttitle{}'s applicability}}
\revcont{As FPGA-based SmartNICs are widely adopted by major cloud providers for hardware acceleration~\cite{211249}, we believe that \projecttitle{} has the potential for broader industry application. In addition,  ASIC-based NICs can also provide the same functionalities by integrating \projecttitle{}'s hardware modules into an optimized System-on-Chip (SoC).}
%\revcont{As FPGA-based SmartNICs are widely adopted by major cloud providers for hardware acceleration~\cite{211249}, we believe that \projecttitle{} has the potential for broader industry application. In addition, \projecttitle{}’s APIs are generic and CPU-agnostic, making them more suitable for cloud environments than programming heterogeneous TEEs.}

%\revcont{\projecttitle{} demonstrates its minimalistic root of trust, which suffices for building BFT distributed systems. 
%ASIC-based NICs can also provide the same functionalities by integrating \projecttitle{}'s hardware modules into an optimized System-on-Chip (SoC). }
%which would be more optimized than the FPGA-based approach

\myparagraph{\rev{C1}{Use cases}}
\revcont{The paper deliberately focuses on distributed cloud applications as \projecttitle{}'s primary use cases. Trust in shared third-party clouds is a more critical concern than in other environments, posing unique challenges in trust, performance, and scalability. While the current scope is specific, the underlying principles could extend to other use cases, such as HPC or on-premise computing.}
%However,  \projecttitle{} addresses these using SmartNICs, which are already widely deployed in modern clouds~\cite{211249}. 


\myparagraph{\rev{D3}{Message drops}}
\revcont{
\projecttitle{} guarantees packet retransmission between two correct nodes until their successful reception  extending a RoCE implementation that supports reliable operations. The application need not re-send the message as it receives a different sequence number, which is not accepted (or verified) by the remote \projecttitle{} until all preceding messages have been received. %Instead, \projecttitle{} extends a RoCE implementation that supports reliable operations where the remote side acknowledges the receipt of a message using specific ACK messages. 
% \projecttitle{} guarantees packet retransmission between two correct nodes until their successful reception. The application need not re-send the message as it would receive a different sequence number, which would not be accepted (or verified) by the remote \projecttitle{} until all preceding messages have been received. Instead, \projecttitle{} extends a RoCE implementation that supports reliable operations where the receipt of a message is acknowledged by the remote side using specific ACK messages.
}

\myparagraph{\rev{D4, E3}{View-change and recovery}}
\revcont{Detailing view-change and recovery in \projecttitle{} protocols are beyond the scope of our work. \projecttitle{} could adopt similar techniques as in TrInc~\cite{trinc} without interfering with these operations. In a new leader's election, replicas can establish new connections with new connection identifiers. As such, previous connections will not block execution, and state transfers (e.g., view-change) can be carried out effectively. } 

%\revcont{Detailing view-change and recovery in \projecttitle{} protocols are beyond the scope of this paper, while \projecttitle{} could adopt techniques such as the ones used by TrInc~\cite{trinc}. Importantly, \projecttitle{} does not interfere with these operations. During a new leader's election, replicas can establish new connections with new connection identifiers. As a result, previous connections will not block execution, and state transfers (e.g., view-change) can be carried out effectively. } 
% \rev{D4, E3}{We do not implement view-change or recovery in \projecttitle{} protocols, while \projecttitle{} does not interfere with these operations. During a new leader's election, replicas can establish new connections with new connection identifiers. As a result, previous connections will not block execution, and state transfers (e.g., view-change) can be carried out effectively. For recovery, \projecttitle{} could adopt techniques such as the ones used by TrInc~\cite{trinc}. } 

% \myparagraph{\rev{E1}{Impact of RDMA on security}}
\myparagraph{\rev{E1}{PCIe transaction encryption}}
\revcont{\projecttitle{} does not use encrypted PCIe transactions for the CPU-to-device communication, which allows attackers to modify the PCIe transactions. However, this vulnerability is not unique to \projecttitle{}; it applies to any network stack, including those based on the OS, since the OS responsible for CPU-to-device communication is untrusted. }

\section{Related work}
%\pramod{the related work bucket should not start with individual papers. It should first summarize the field/area/bucket area, and then give example systems, and lastly, it should end with an overall comparison of the the research field with our solution. In this way, you avoid direct comparison with individual work. Can you please re-write it?}

\myparagraph{Trustworthy distributed systems} Classical BFT systems~\cite{Castro:2002, Suri_Payer_2021, DBLP:journals/corr/abs-1803-05069, Chan2018PaLaAS, DBLP:journals/corr/abs-1807-04938, Chan2018PiLiAE, bft-smart, 6681599} provide BFT guarantees at the cost of high complexity, performance, and scalability overheads. \projecttitle{} bridges the gap between BFT and prior limitations, designing a {\em silicon root-of-trust} with generic trusted networking abstractions that materialize the BFT security properties.

\myparagraph{Trusted hardware for distributed systems} Trustworthy systems~\cite{10.1145/3492321.3519568, minBFT, 10.1145/3552326.3587455, 10.1145/3492321.3519568, treaty, avocado, ccf} leverage trusted hardware to optimize the performance of classical BFT at the cost of generalization and easy adoption. The systems suffer from high latencies (50us---105ms)~\cite{levin2009trinc, 10.1145/2168836.2168866}, build large TCBs~\cite{treaty, avocado}, and rely on specific TEEs~\cite{minBFT, hybster}. In contrast, our \projecttitle{} aims to offer performance and generality, while our minimalistic TCB is verifiable and unified in the heterogeneous cloud. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{eval-plots/plots/hw_eval_attest_util.pdf}
    \vspace{-20pt}
  \caption{\rev{(d)}{The scalability analysis of \projecttitle{} hardware. The resource usage is normalized to the U280 FPGA capacity.} }
  % \caption{Latency evaluation of send operations for various packet sizes across five competitive network stacks with various security properties.}
    % \felix{Figure: BRAM = RAMB36 (including RAMB18) + URAM. "CARRY8" is the 4th most used resource of the attestation kernel and is used for "Others" as an upper bound for all other resources.}
    % More resource utilization details: https://github.com/dgiantsidi/replication-protos/blob/main/plots/asplos_submission/attestation_kernel_util.md
    \label{fig:scalability}
   %\vspace{-2pt}
\end{figure}

\myparagraph{SmartNIC-assisted systems} Networked systems offer fast network operations with emerging (programmable) SmartNIC devices~\cite{liquidIO_smartnics, u280_smartnics, bluefield_smartnics, broadcom_smartnics, netronome_smartnics, alibaba_smartnics, nitro_smartnics, msr_smartnics}. Some of them~\cite{246498, 211249, 10.1145/3387514.3405895, 10.1145/3365609.3365851, 10.1145/3127479.3132252,  258971, 246486, 179716, 227655, 10.1145/3286062.3286068, shan2022supernic, 10.1145/3390251.3390257} offload the network functions to the hardware and reduce the host processing and energy overheads. In contrast, others~\cite{10.1145/3341302.3342079, 10.1145/2872362.2872367, 234944, 9220629, 6853195, 10292786, 10.1145/3477132.3483555, 280678, 10.1145/3132747.3132756, honeycomb, 288659, 10329593} build generic execution frameworks to optimize a wide variety of distributed systems. Our \projecttitle{} follows a similar approach by building a high-performant unified network stack with SmartNICs and offloading security properties to the NIC hardware.


\myparagraph{SmartNIC-assisted network stacks} SmartNICs effectively provide high-performance network stacks. Another line of research~\cite{coyote, corundum, storm, 8891991, 280712, 9114811, opennic_project} re-designs generic networking protocols, from RDMA/RoCE to TCP/IP network stacks, on top of FPGA-based SmartNICs for performance. Our \projecttitle{} further extends its security semantics with the properties of non-equivocation and transferable authentication. 

\myparagraph{Programmable HW for network security} Programmable hardware, SmartNICs, and switches are used to shield networking. Recent systems~\cite{10.1145/3603269.3604874, 10.1145/3620678.3624786, 10.1145/3563647.3563654, 10.1145/3321408.3323087, 278292} leverage programmable switches and FPGAs to offload security processing and boost performance in the context of blockchain systems~\cite{10.1145/3603269.3604874} or security functions (e.g., access control, DNS traffic inspection)~\cite{10.1145/3620678.3624786, 10.1145/3563647.3563654, 10.1145/3321408.3323087}. Our \projecttitle{} similarly offloads security into the hardware, but it carefully uses SmartNICs to overcome the processing bottlenecks of the switches. 







==> system_model.tex <==
\section{System Model}

==> use_cases.tex <==
\section{Protocols Implementation}\label{sec:use_cases-appendix}
We next present the implementation details of four distributed systems shown in Table~\ref{tab:use_cases_options} using \projecttitle{}, presented in Section~\ref{sec:use_cases}.

\begin{table}
\begin{center}
\small
\begin{tabular}{ |c|c|c|c| } 
 \hline
 System & $N$ & $f$ ($N=3$) & Byz. faults \\ [0.5ex] \hline \hline
 A2M    & 1 & 0 & Prevention\\
 BFT &  $2f+1$ & $f=1$ & Prevention\\
 Chain Replication &  $2f+1$ & $f=1$ & Prevention\\
 PeerReview & $f+1$ & $f=2$ & Detection\\
 \hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{Properties of the four trustworthy distributed systems implemented with \projecttitle{}.}
\label{tab:use_cases_options}
%\vspace{-18pt}
\end{table}

\subsection{Attested Append-Only Memory (A2M)}\label{sec:use_cases::a2m}



%\atsushi{What's the purpose of designing the TNIC-log? Can we explain the motivation in the first paragraph?}


We designed a single-node trusted log system based on the A2M system (Attested Append-Only Memory)~\cite{A2M} using \projecttitle{}. A2M has been proven to be an effective building block in improving the scalability and performance of various BFT systems~\cite{sundr, Castro:2002, AbdElMalek2005FaultscalableBF}. We show the {\em how} to use \projecttitle{} to build this foundational system while we also show that \projecttitle{} minimizes the system's TCB jointly with the performance improvements discussed in $\S$~\ref{sec:eval}.

\myparagraph{System model} Our \projecttitle{} version and the original A2M systems are single-node systems that target a similar goal; they both build a trusted append-only log as an effective mechanism to combat equivocation. The clients are only allowed to append entries to a log and each log entry is associated with a monotonically increasing sequence number. As such, each data item, e.g., a network message, is bound to a unique sequence number which is a well-known approach for equivocation-free operations~\cite{clement2012, hybster}. 

A2M was originally built using CPU-side TEEs---specifically, Intel SGX--- whereas we build its \projecttitle{} derivative. While the original A2M system keeps its entire state and the log within the TEE, we use \projecttitle{} to keep the (trusted) log in the untrusted memory. As such, in contrast to the original A2M, \projecttitle{} effectively reduces the overall system's TCB. Our evaluation showed that naively porting the application within the TEE has adverse performance implications in lookup operations.


%the trusted component \atsushi{Here explains that TNIC-log brings better memory efficiency than A2M, which could also be written in the first paragraph to highlight the advantage of TNIC}.

\myparagraph{Execution} Similarly to A2M, we expose three core operations: the \texttt{append}, \texttt{lookup}, and \texttt{truncate} operations to add, retrieve, and delete items of the log, respectively. A2M stores the lowest and highest sequence numbers for each log. Upon appending an entry, A2M increases the highest sequence number and associates it with the newly appended entry. When truncating the log, the system advances the lowest sequence number accordingly. We now show how we designed the operations using \projecttitle{} APIs.




\begin{algorithm}
\SetAlgoLined
\small
%\vspace{0.02cm}
\textbf{function} \texttt{append(id, ctx)} \{ \\
\Indp
 [$\alpha$,\texttt{i},\texttt{ctx}] $\leftarrow$ \texttt{local\_send(id,ctx)};\\
 \texttt{log[id].append(log\_entry($\alpha$,\texttt{i},\texttt{ctx}))};\\
 {\bf return} \texttt{[$\alpha$,\texttt{i},\texttt{ctx}]};\\
\Indm
\} \\

\vspace{0.15cm}

\textbf{function} \texttt{lookup(id, i)} \{ \\
\Indp
    {\bf return} \texttt{log[id].get(i)};\\
\Indm
\} \\
\vspace{0.15cm}
\textbf{function} \texttt{truncate(id, head, z)} \{ \\
\Indp
    [$\alpha$,\texttt{tail},\texttt{ctx}] $\leftarrow$ \texttt{append(id,} \textsc{trnc}\texttt{||id||z||head)};\\
        
    %[$\alpha_{2}$,\texttt{idx},\texttt{ctx}$_{2}$]
    \texttt{e} $\leftarrow$ \texttt{append(}\textsc{manifest}\texttt{,[$\alpha$,\texttt{tail},\texttt{ctx}])};\\
    {\bf return} \texttt{e};\\
\Indm
\} \\

\vspace{0.15cm}
\textbf{function} \texttt{verify\_lookup(id, e, head, tail)} \{ \\
\Indp
    \textbf{assert}(\texttt{e.i}$>=$\texttt{tail)};\\
    \texttt{local\_verify(id, e)};\\
\Indm
\} \\
\vspace{-1pt}
\caption{Attested Append-Only Memory (A2M) using \projecttitle{}.}
\label{algo:tnic_log}
\end{algorithm}

\myparagraph{Append operation} The \texttt{append(id,ctx)} operation takes a data item, \texttt{ctx}, and appends it to the log with identifier \texttt{id}. A log entry at index \texttt{i} is comprised of three items: the sequence number of that entry (\texttt{i}), the context of the entry (\texttt{ctx}), and the {\em authenticator} field, namely the digest of the \texttt{ctx||i} as in~\cite{levin2009trinc}. In our implementation, we additionally support the original A2M {\em authenticator} format calculated as the cumulative digest \texttt{c\_digest[i]} for that entry which is calculated as \texttt{c\_digest[i]=hash(ctx||sq||c\_digest[i-1])} where \texttt{c\_digest[0]=0}. The sequence number \texttt{i} is then increased to distinguish any entry that will be appended in the future. %With the cumulative digest we create a set of chains and as such we cannot his method does not cause any values to be forgotten.





\myparagraph{Lookup operation} The \texttt{lookup(id, i)} retrieves the log entry at index \texttt{i} of log with identifier \texttt{id}. Compared to A2M where lookups are compelled to access the trusted hardware, \projecttitle{}-log only performs a local memory access. 
The function does not verify whether the entry is legitimate. Developers need to implement the \texttt{verify\_lookup(id, entry, head, tail)} to verify the attestation. The boundaries of the log (i.e., \texttt{head} and \texttt{tail}) can always be retrieved by replaying a specific log, which keeps the state changes, the \textsc{manifest}. We explain how \textsc{manifest} works in the next paragraph.

\myparagraph{Truncate operation} The \texttt{truncate(id, head, z)}, where \texttt{z} is a nonce provided by the client for freshness, ``forgets'' all log entries with sequence numbers lower than \texttt{head}. A non-Byzantine client will never be able to successfully verify a forgotten entry of the log. To do that, \projecttitle{}-log makes use of an additional log \textsc{manifest}, which keeps the logs' state changes. First, the operation attests to the {\em tail} of the log by appending a specific entry which includes the nonce for a correct client to be later able to verify the operation. Then, the algorithm will append the last attested message of the log to the \textsc{manifest} log and return the attested message for the second append. To retrieve the boundaries of a log, clients can always attest to the tail of the \textsc{manifest} and read backward until they find a \textsc{trnc} entry.


\noindent\fbox{\begin{minipage}{\columnwidth}
\myparagraph{System design takeaway} \projecttitle{} minimizes the required TCB in A2M system while it offers faster lookup operations compared to its original version.
\end{minipage}}
%\atsushi{Can we explain more which point is improved thanks to TNIC?}

%Since the logs reside in the untrusted host memory, their integrity can be compromised by malicious adversaries. However, these adversaries cannot impersonate \projecttitle{} and generate verifiable attestations in any way. As such we do not worry about entries that are not written yet (these will never be verifiable). 
%If an adversary compromises the \textsc{MANIFEST}, \projecttitle{}-log might become responsive. However, this affects availability but not safary and it is beyond the scope of this work similar to other systems [A2M, Trinc, Damysus]. 


\subsection{Byzantine Fault Tolerance (BFT)}\label{sec:use_cases::byz_smr}
%\atsushi{unclear to me what is the advantage of using TNIC to implement the Byzantine SMR. Can we somehow highlight this point?}
%\dimitra{@Atnoni: Can we afford a network partition? 2f+1 w/ f=2, Assume Byz. leader and Byz. follower that drive execution with one correct replica---the others are on purpose exluded by the faulty leader. The client will have a correct reply always because it will wait for f+1 (=3) identical replies. Although if the most up to date correct replica afterwards is partitioned out then we just block; the remaining correct replicas will have lost one message and block until they get it ... }
%\pramod{ToDo: Pesudocode.}

As a second example for \projecttitle{} applications, we build a Byzantine Fault Tolerance protocol (BFT) that implements a State Machine Replication (SMR) based on a counter. Clients send increment counter requests to the SMR and receive the updated counter value. Despite its simplicity, this particular system can represent an ordering service that is a fundamental building block in various distributed applications ranging from event logging and databases systems to serverless and blockchain systems~\cite{rafthyperledger, Kafka, boki, 10.1145/3286685.3286686, scalog}. Our BFT combats equivocation through \projecttitle{} that serializes all messages. As such, \projecttitle{} optimizes the number of participant nodes compared to the classical BFT and further reduces the message complexity.

\myparagraph{System model} We consider a system of $N=2f+1$ replicas (or {\em nodes}) that communicate with each other over unreliable point-to-point network links. At most $f$ of these replicas can be Byzantine (aka {\em faulty}), i.e., can behave arbitrarily. The rest of the replicas are {\em correct}. Recall that classical BFT protocols require an extra set of $f$ replicas, in total $3f+1$ replicas to handle $f$ Byzantine failures. One of the replicas is the {\em leader} that drives the protocol, whereas the remaining replicas are (passive) followers. There is only a single active leader at a time.

For liveness, we assume a partial synchrony model~\cite{FLP, 10.1145/226643.226647}. We have only explored deterministic protocol specifications; the correct replicas begin in the same state, and receiving the same inputs in the same order will arrive at the same state, generating the same outputs. Lastly, as in classical BFT protocols, we cannot prevent Byzantine clients who otherwise follow the protocol from overwriting correct clients’ data.


\myparagraph{Execution} We implement BFT with \projecttitle{} as a leader-based State-Machine-Replication (SMR) protocol for a Byzantine model that stores and increases the value of the counter. The leader receives clients' requests to increment the counter. The leader, in turn, executes the protocol and applies the changes to its state machine---in our case, the leader computes and stores the next available counter value. Subsequently, the leader broadcasts the request along with some metadata to the passive followers. The metadata includes, among others, the leader's calculated output in response to the client's command, namely, the increased counter value the leader has calculated and the {\em state} of the followers known to the leader. In our implementation, the {\em state} is represented as the signed hash of the counter value of each follower (known to the leader).

The followers, in turn, execute and apply the incremented counter value to their state machines. However, they first attest to the leader's actions to detect misbehavior. To do so, they audit and validate its sent output through re-execution. Precisely, the followers except for their state machine, {\em simulate} leader's state machine. Each follower replica must add an extra counter representing the state the value counter is expected to have, leading to a $2\times$ extra space complexity. A follower will update the leader's value based on the commands received and then compare its calculated leader's value with the received one. In addition, the followers will validate the state of the replicas (including the leader and all other replicas). They only have to check if their previous state equals the other replicas' state.

After a replica validates the protocol, it applies the increments to its local counter. The followers will reply to the client with the result of the operation. In addition, they will reply to the leader, which will validate the follower's output. The leader, upon successful validation, will also reply to the client. The client can trust the result if they receive identical replies from the quorum, i.e., at least $f+1$ identical messages from different replicas (including the leader). This guarantees that at least one correct replica has responded with the correct result.


\myparagraph{Failure handling} Our strategy to verify the leader's execution jointly with the primitives of non-equivocation and transferable authentication offered by \projecttitle{} shields the protocol against a Byzantine leader. The leader cannot equivocate; even if it attempts to send different requests for the same round to different followers, executing the {\tt local\_send()} will assign different counter values that healthy followers can detect. As such, a leader in that case will be exposed. 

Likewise, the equivocation mechanism allow correct followers to discard stale message requests sent through replay attacks on the network. If a follower is Byzantine, a healthy leader or any healthy replica will detect it. For $f\geq2$, it is impossible for a faulty leader and, at most, $f-1$ remaining Byzantine follower to compromise the protocol. Either these faults will be detected by a healthy replica during the validation phase, or the protocol will be unavailable, i.e., if the leader in purpose only communicates with the Byzantine followers. This directly affects BFT correctness requirements; a client will never get at least $f+1$ matching replies. For protocols to progress in case of a faulty leader, they must pass through a recovery protocol or view-change protocols similar to those described in previous works~\cite{minBFT, Castro:2002}. Recovering is beyond the scope of this work, and as such, we did not implement it.


\noindent\fbox{\begin{minipage}{\columnwidth}
\myparagraph{System design takeaway} \projecttitle{} optimizes the replication factor and the message complexity of BFT.
\end{minipage}}

%\antonis{Could be phrased a bit better.}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.6\linewidth]{figures/bft-pb.drawio.pdf} 
%    \caption{\projecttitle{} application on a Byzantine SMR protocol.\pramod{We can drop this figure.}} \label{fig:byz_smr}
%\end{figure}

\begin{algorithm}
\SetAlgoLined
\small
%\vspace{0.02cm}
\textbf{function} \texttt{leader(req)} \{ \\
\Indp
 {\tt output} $\leftarrow$ \texttt{execute(req)};\\
 {\tt msg} $\leftarrow$ \texttt{req||output};\\
 {\tt attested\_msg} $\leftarrow$ \texttt{local\_send(msg)};\\
 \texttt{rem\_write(}\textsc{followers[:]}{\tt, attested\_msg)};\\

{\bf upon reception of {\tt ack} from \textsc{followers}:}\\
    \Indp
        {\tt [{$\alpha$ || attested\_msg || follower\_output}]} $\leftarrow$ \texttt{upon\_delivery(ack)};\\
        {\bf assert(}\texttt{validate\_follower(attested\_msg, follower\_output)}{\bf)};\\
    \Indm

 \texttt{auth\_send(}\textsc{client}{\tt,msg)};\\
\Indm
\} \\

\vspace{0.15cm}

\textbf{function} \texttt{follower(msg)} \{ \\
\Indp
{\bf upon reception of {\tt msg}:}\\
    \Indp
        {\tt [{$\alpha$ || req || output}]} $\leftarrow$ \texttt{upon\_delivery(req)};\\
    \Indm

    {\bf assert(}\texttt{validate\_leader(req, output)}{\bf)};\\
    {\tt current\_output} $\leftarrow$ \texttt{execute(req)};\\
    
    \texttt{auth\_send(}\textsc{client}{\tt, req|| current\_output)};\\
    {\tt ack\_msg} $\leftarrow$ \texttt{msg|| current\_output};\\
    \texttt{auth\_send(}\textsc{middle}{\tt, ack\_msg)};\\
\Indm
\} \\
\vspace{-1pt}
\caption{BFT using \projecttitle{}.}
\label{algo:tnic_bft}
\end{algorithm}

%
%\dimitra{>Github code issues:
%\begin{itemize}
%    \item Line 239: has a logical bug regarding the message batching
%    \item Lines 205--210: unnecessary hash re-calcucations--- might improve performance if fixed
%    \item Continuation function needs improvement for correctness/completeness (leader should store the output for each on-going command).
%    \item For correctness, leader should have only one outstanding operation at a time.
%\end{itemize}}



%\lstinputlisting[language=C++]{codelets/pb.cc}




\subsection{Chain Replication (CR)}\label{sec:use_cases::byz_chain_rep}

\begin{algorithm}
\SetAlgoLined
\small
%\vspace{0.02cm}
\textbf{function} \texttt{head\_operation(req)} \{ \\
\Indp
 {\tt output} $\leftarrow$ \texttt{execute(req)};\\
 {\tt msg} $\leftarrow$ \texttt{req||output};\\
 \texttt{auth\_send(}\textsc{middle}{\tt,msg)};\\ \texttt{auth\_send(}\textsc{client}{\tt,msg)};\\
\Indm
\} \\

\vspace{0.15cm}

\textbf{function} \texttt{middle\_tail\_operation(msg)} \{ \\
\Indp
    {\bf assert(}\texttt{validate\_chain(msg)}{\bf)};\\
    {\tt output} $\leftarrow$ \texttt{execute(req)};\\
    {\tt chained\_msg} $\leftarrow$ \texttt{msg||output};\\
    {\bf if} (!\textsc{tail})\\
    \Indp
    \texttt{auth\_send(}\textsc{middle}{\tt,chained\_msg)};\\
    \Indm
    \texttt{auth\_send(}\textsc{client}{\tt,req||output)};\\
\Indm
\} \\
\vspace{0.15cm}
\textbf{function} \texttt{validate(msg)} \{ \\
\Indp
    \texttt{len} $\leftarrow$ \texttt{sz};\\
    \texttt{[req, out, cmt]} $\leftarrow$ \texttt{unmarshall(msg[0:len])};\\
    {\bf assert(}\texttt{memcmp(req, out)}{\bf)};\\
    {\bf assert(}\texttt{(cmt == expected\_cmt)}{\bf)};\\
    {\bf for} {\tt(i = 1; i < }{\sc node\_id}; {\tt i++)} \{\\
    \Indp
    \texttt{[out, cmt]} $\leftarrow$ \texttt{unmarshall(msg[len:len+\textsc{sz}])};\\
    {\bf assert(}\texttt{memcmp(req, out)}{\bf)};\\
    {\bf assert(}\texttt{(cmt == expected\_cmt)}{\bf)};\\
    \texttt{len} $\leftarrow$ \texttt{len} + \texttt{sz};\\
    \Indm
    {\bf return} {\tt True};\\
\Indm
\} \\
\vspace{-1pt}
\caption{Chain Replication using \projecttitle{}.}
\label{algo:tnic_chain_replication}
\end{algorithm}



We implement a Byzantine Chain Replication using \projecttitle{} that represents the replication layer of a Key-Value store. Chain Replication is a foundational protocol to build state-machine-replication and originally operates under the CFT model using $f+1$ nodes to tolerate up to $f$ failures. We show {\em how} to use \projecttitle{} to shield the protocol without changes to the core of the algorithm (states, rounds, etc.) while keeping the same replication factor.




\myparagraph{System model} We make the same assumptions for the system as in the BFT in Appendix $\S$~\ref{sec:use_cases::byz_smr}. For error detection and reconfiguration, we further assume a centralized (trusted) configuration service as in~\cite{10.1007/978-3-642-35476-2_24} that generates new configurations upon receiving reconfiguration requests from replicas. Recall that classical Chain Replication under the CFT model also relies on reliable failure detectors~\cite{chain-replication}. For liveness, we also assume that the configuration service will eventually create a configuration of correct replicas that do not intentionally issue reconfiguration requests to perform Denial-of-Service attacks. 

Clients send requests to {\tt put} or {\tt get} a value and receive the result. The replicas (e.g. head, middle, and {\em tail} nodes) are connected in a chained fashion, and the requests flow from the head node to the tail through the intermediate middle replicas. 

Similar to previous BFT protocols~\cite{Castro:2002, minBFT}, malicious primaries, i.e., the head, that do not forward the message intentionally are detected in clients' side and trigger reconfiguration.


\myparagraph{Execution} To execute a request \texttt{req}, e.g., {\tt put}/{\tt get}, a client first obtains the current configuration from the configuration service and sends {\tt req} to the head of the chain. The head orders and executes the request, and then it creates a {\em proof of execution message}, which is sent along the chain. The proof of execution includes the {\tt req} and the leader's action ({\tt out}) in response to that request. In our case, the leader sends the {\tt req} along with the commit index it has assigned to it. The message is then sent (signed) to the middle node that follows in the chain.

The middle node checks the validity of the message by verifying that the head's output is correct, executes the {\tt req}, and forwards the request to the following replica. Similarly, every other node executes the original request, verifies the output of all previous nodes, and sends the original request as well as a vector of all previous outputs. A replica needs to construct a {\em proof of execution message} that achieves one goal. It allows the following replicas in the chain to verify all previous replicas so far. As such the messages is of the form < < <{\tt req}, {\tt out$_{leader}$}>$_{\sigma_0}$, {\tt out$_{middle1}$}>$_{\sigma_1}$, .., {\tt out$_{tail}$}>$_{\sigma_N}$. The tail is the last node in the chain that will execute and verify the execution of the request. 


In contrast to the CFT version of the Chain Replication protocol, local operations in the tail, {\tt get} or {\tt ack} in a {\tt put} request cannot be trusted. 

As such the replicas in the chain need to reply to the clients with their output after they have forwarded their proof of execution message. Clients can wait for at least $f$ replicas replies and the tail reply to collide. Clients can execute the {\tt get} requests similarly to {\tt write} requests, which will traverse the entire chain, or clients can consult the majority and broadcast the request to $f+1$ replicas, including the tail. 


\myparagraph{Failure handling} By definition of the protocol, all nodes will see and execute all messages in the same order that is imposed by the head node. As such, all correct replicas will always be in the same state. In addition, network partitions that may split the chain into two (or more) individual chains that operate independently cannot affect safety: the clients will need to verify at least $f+1$ identical replies. In case a correct replica or a client detects a violation (by examining the proof of execution message or having to hear for too long from a node), they can expose the faulty node and request a reconfiguration.

\noindent\fbox{\begin{minipage}{\columnwidth}
\myparagraph{System design takeaway} \projecttitle{} {\em seamlessly} shields the Chain Replication system for Byzantine settings with the same replication factor as the original CFT system while it improves performance compared to its TEEs-based competitors.
\end{minipage}}

%\dimitra{>Github code issues:
%\begin{itemize}
%    \item check\_outputs function (L:67): Did you miss a validation step regarding transferable authentication?
%\end{itemize}}

%\lstinputlisting[language=C++]{codelets/cr.cc}
%\myparagraph{Write protocol} {\underline{Failure-free execution.}} The operation flows from the head to the tail. The leader executes the request and sends the original request as well as the output of that request. Every other node executes the original request, verifies the output of all previous nodes and sends the original request as well as a vector of all previous outputs. Lastly, the tail executes the request and replies back to the client with the proof of protocol execution.

%\myparagraph{Read protocol} The client can execute a read request similarly to the write request. As the requests can be re-ordered by malicious nodes, including the tail, local reads in the tail, in contrast to original CFT version of the protocol, cannot be trusted. As an optimization for the read-only requests, clients can consult the majority and broadcast the request to $f+1$ replicas including the tail. Since all replicas see all messages (by definition of the protocol), at least one replica will be correct and up to date. Therefore upon $f+1$ replies that collide, clients can trust the result.

%\myparagraph{{Failures detection}} The non-equivocation and transferable authentication primitives ensure that the nodes cannot impersonate others and cannot replay network traffic. As such, while malicious nodes might try deviate from the protocol in any way, e.g., re-order commands, compromise the commands, etc., correct replicas will detect misbehavior's. Even in the scenario where the tail node is faulty and execute the protocol erroneous, the fault will eventually be detected (upon access) as all nodes see all messages and thus, the vector of outputs will not be correct. %Lastly, the unprotected area can be compromised which is detected as the fpga\_cache will have for each key the lastly send command.



\subsection{Accountability (PeerReview)}
\label{sec:use_cases::accountability}





We implement an accountability protocol based on the PeerReview system~\cite{bftdetection, peer-review}. Compared to the previous three BFT systems that prohibit an improper action from taking effect, accountability protocols~\cite{268272, bftdetection, peer-review} slightly weaken the system (fault) model in favor of performance and scalability. Specifically, our protocol {\em allows} Byzantine faults to happen (e.g., correct nodes might be convinced by a malicious replica to permanently delete data). Still, it guarantees that malicious actions can always be detected. Accountability protocols can be applied to different systems as generic guards that trade security for performance~\cite{peer-review}, e.g., networked file systems, bit-torrent systems, etc. 

The original version of the system did not use trusted components and as such, incurred a high message complexity O($n^2$) to combat equivocation. \projecttitle{} to improve that message complexity.

\myparagraph{System model} We only detect faults that directly or indirectly affect a message, implying that {\em (i)} correct nodes 
can observe all messages sent and received by that node and {\em (ii)}  Byzantine faults that are not observable through the network cannot be detected. For example, a faulty storage node might report that it is out of disk space, which cannot be verified without knowing the actual state of its disks.

We further assume that each protocol participant acts according to a deterministic specification protocol. As such, detection can be accomplished even with a single correct machine, requiring only $f+1$ machines. This does not contradict the impossibility results for agreement~\cite{FLP} because detection systems do not guarantee safety.


\myparagraph{Execution} The participants communicate through network messages generated by \projecttitle{}.  In addition, each participant maintains a {\em tamper-evident} log that stores all messages sent and received by that node as a chain. A log entry is associated with an entry index, the entry data, and an authenticator, calculated as the signed hash of the tail of the log and the current entry data. 

We frame our protocol in the context of an overlay multicast protocol~\cite{10.1145/945445.945474} widely used in streaming systems. The nodes are organized as a tree where the streaming content (e.g., audio, video) flows from a source, i.e., {\em root} node, to clients ({\em children} nodes). To support many clients, each client can act as a source to other clients, which will be connected as children nodes. 

In our implementation, we consider nodes in a tree topology. The tree's height is equal to one, comprising one source node and two client (children) nodes connected to the source. Algorithm~\ref{algo:tnic_accountability_protocol} ($\S$~\ref{sec:use_cases-appendix}) shows the operations of our implemented accountability protocol. When the source sends a context (executes the \texttt{root()} function), it implicitly includes a signed statement that this message has a particular sequence number (generated by \projecttitle{}). The clients execute the {\tt child()} function that validates the received message, logs the received message, executes the result, and responds back to the source. 


\begin{algorithm}[t]
\SetAlgoLined
\small
%\vspace{0.02cm}
\textbf{function} \texttt{root(ctx)} \{ \\
\Indp
 \texttt{auth\_send(}\textsc{child}{\tt,ctx)};\\
 {\bf upon reception of \texttt{response}:};\\
 \Indp
    {\bf assert(}\texttt{validate\_reception(response)}{\bf)};\\
    \texttt{log(response)};\\
\Indm
\Indm
\} \\

\vspace{0.15cm}

\textbf{function} \texttt{child($\alpha$||cmd||seq)} \{ \\
\Indp
    {\bf assert(}\texttt{validate\_reception($\alpha$||cmd||seq)}{\bf)};\\
    \texttt{log($\alpha$||cmd||seq)};\\
    {\tt result} $\leftarrow$ \texttt{execute(cmt)};\\
    {\tt response} $\leftarrow$ \texttt{log(result||cmd)};\\
    \texttt{auth\_send(}\textsc{root}{\tt, response)};\\
\Indm
\} \\
\vspace{0.15cm}
\textbf{function} \texttt{log\_audit()} \{ \\
\Indp
    {\bf{while}} \texttt{last\_id < log\_tail} \{\\
    \Indp

        \texttt{entry} $\leftarrow$ \texttt{validate\_log\_entry\_at(last\_id)};\\
        \texttt{last\_id++};\\
        {\bf assert(}\texttt{replay(entry)}{\bf{)}};\\
    \Indm
    \}\\
\Indm
\} \\
%\vspace{-1pt}
\caption{ (PeerReview) Accountable systems using \projecttitle{}.}
\label{algo:tnic_accountability_protocol}
\end{algorithm}


Each node is assigned to a set of {\em witness} processes to detect faults. Similarly to the original system, we assume that the set of nodes and its witnesses set {\em always} contain a correct process. The witnesses audit and monitor the node's log. To detect bad behaviors (or expose non-responsive nodes), the witnesses read the node's log and replay it to run the participant’s state machine. As such, they ensure the participant’s state is consistent with proper operation. 

Specifically, each witness for a participant node keeps track of n, a log sequence number, and s, the state that the participant should have been in after sending or receiving the message in log entry n. It initializes n to 0 and s to the initial state of the participant.

Whenever a witness wants to audit a node, it sends its n and a nonce.
The participant returns an attestation of all entries between n and its current log entry using the nonce. The witness then runs the reference implementation, starting at state $s$, and progressing through all the log entries. If the reference implementation sends the same messages in the log, then the witness updates n, which is the state of the reference implementation at that point. If not, then the witness has proof it can present of the participant’s failure to act correctly.




The original PeerReview system requires a receiver node to forward messages to the original sender’s witnesses so they can ensure this message is {\em legitimate}, i.e., it appears in the sender’s log. No other conflicting message is sent to another peer (equivocation). As such, a peer must communicate (in every round) with the witness set of any other peer, leading to a quadratic message complexity. \projecttitle{} eliminates the overhead; in fact a participant that sends or receives a message needs to attest and append the message and its attestation in each own log. A participant can process received messages only if they are accompanied by attestations generated by the sender's \projecttitle{} hardware. 



\noindent\fbox{\begin{minipage}{\columnwidth}
\myparagraph{System design takeaway} \projecttitle{} can be used to optimize accountable systems, e.g., PeerReview, while optimizing their message complexity thanks to how it handles equivocation.
\end{minipage}}


%As demonstrated with A2M, TrInc can
%easily supply a trusted log without the assistance of a
%witness set. Our first modification is to include such a
%trusted log. Whenever a participant sends or receives a
%message, it logs that message with an attestation from
%its trinket. A participant should only process a received
%message if it is accompanied by an attestation that the
%message has been logged by the sender’s trinket.


%As the source might cheat by equivocating with witnesses regarding the messages it sends to clients \atsushi{what does it mean?}, the root is also required to log the (signed) response received by clients that includes proof that clients executed the protocol. That could be either the client's hash of its own log or, in our particular example, the command the client received from the source. 

%Lastly, the source might on purpose 
%For this reason, when a participant receives a message from another, it also logs the attestation generated forwards this message to the
%sender’s witnesses, so they can ensure this message actually appears in the sender’s log.

\if 0
\begin{itemize}
    \item (f+1) nodes
    \item deterministic actions (let's say it is a log for NFS or a DB)
    \item each node: has an in-memory (append-only) log
    \item each message: signed(H) || H (payload) || payload = {action, log\_index}
    \item nodes cannot equivocate + cannot impersonate others -> we mask Byz-faults as network partition (or slow replicas)
    \item Correct nodes will identify unresponsive nodes and can prove their correctness by auditing their log with their own log
    \item Logs are chains of the history -> tamperproof
\end{itemize}
\fi


\if 0
\dimitra{SOOOOS -> finalize the pseudocode for all protocols + recovery}

\dimitra{
Motivate the replication protocols in the context of widely-adopted generally purposed DS (transactions, storage system, shared log).
\begin{itemize}
    \item Raft (use cache for replicated distributed txs~\cite{cockroachdb_raft})
    \item Chain replication (use case for fault-tolerant distributed storage system~\cite{corfudb})
    \item AllConcur (use case for a leaderless shared-log~\cite{})
\end{itemize}
}
\dimitra{SOS -> discuss correctness of recovery (reconciliation)}


\subsection{Raft}

\myparagraph{Write protocol} {\underline{Failure-free operation.}} The leader executes the client request, e.g., assigns to it an id, stores it in a queue with all on-going requests and generates an output (the assigned id with hash of the command). Then it broadcasts the message to all followers (replication phase). A follower executes the protocol, replicating the command but also verify that the request from the leader is generated through a valid execution scenario. In other words, it simulates the leader's protocol. As a result, it sends back its output (as a follower) and the calculated output (as a leader). When the leader receives $f+1$ identical replies, which denotes that at least one correct replica validated that the leader executed the protocol's round correctly. The execution returns back to the untrusted cpu where the leader procceeds with the second round. 

The leader replies back to the client assigning the proofs of the majority (for the protocol execution). 

\lstinputlisting[language=C++]{codelets/raft.cc}

\myparagraph{Read protocol} Read commands can be executed identically to writes as leaders can violate correctness and consistency guarantees by returning valid, yet stale replies to the client. As an optimization, read-only commands can be executed as a multicast broadcast to all replicas, waiting for $f+1$ identical replies.


\myparagraph{Failure detection} The non-equivocation layer guarantees that all followers will receive the messages in the same order and will not miss any past messages. The transferable authentication layer guarantees that a faulty replica, including the leader, cannot impersonate other nodes and compromise the protocol. For example, the client expects $f+1$ identical proofs that at least $f+1$ replicas have executed and validated the protocol.
\fi



\if 0
\subsection{Decentralized atomic broadcast}
We implement a decentralized (leaderless) atomic broadcast based on~\cite{}, \texttt{BFTcast}. All replicas receive all messages and apply the requests in a pre-defined order.

\myparagraph{Write protocol} \noindent{\underline{Failure-free execution.}} Each node multicasts (a batch of) requests to every other node. The first round is completed when all nodes have received all messages of the protocol. Then each node executes the requests in the pre-defined order, e.g., based on the node id and computes the outcome (e.g., certificate) which is send as a confirmation to every other node. Similarly to the \texttt{BFTcr}, \texttt{BFTcast} replicas are receiving all messages from all other replicas in the system. As such, misbehavior of Byzantine nodes might only affect availability but not safety.


\lstinputlisting[language=C++]{codelets/decentralized_atomic_broadcast.cc}


\myparagraph{Read protocol} In line with the previous protocols clients cannot trust individuals. Reads can be executed similarly to writes, requiring all replicas to execute the request. As an optimization, clients can consult the majority ($f+1$) by broadcasting the reads and requiring as in classical BFT protocols at least $f+1$ identical replies.


\myparagraph{{Failures detection}} The transferable authentication primitives guarantees that replicas cannot impersonate others, therefore correct replicas can distinguish if the protocol has been executed correctly. The non-equivocation primitive guarantees that all replicas will see the same message for the same round. Byzantine nodes can violate the pre-defined order of execution. Thanks for the all-to-all communication of the second phase of the protocol whose goal is to verify that everyone executed the protocol correctly, failures will be detected from the correct replicas which will halt the protocol. Note that in this protocol we do not require the fpga\_cache as in each round the correct replicas will have the correct value of the log tail.

\subsection{Dealing with failures} In the case of faulty followers, the service remains available because the correct replicas (majority) include the leader. Consequently, the protocol is executed correctly.

In case the leader is faulty, the protocol execution can be violated. This in turn might lead to replicas states not being consistent, the system not making any progress and the clients not receiving valid responses to their requests. 

Followers detect the leader's failures (e.g., the leader deviates from the protocol or performs Denial-of-Service attacks to all or some servers), by \emph{(i)} validating the leader's execution and \emph{(ii)} using timers (to detect an un-responsive leader), in similar fashion as in~\cite{Veronese2013EfficientBF, Castro:2002, 10.1007/978-3-642-35476-2_24}. The use of timers do not violate safety, instead it might trigger a view-change operation and recovery. Specifically, when a replica $s_i$ times-out it broadcasts to all a \texttt{prep-view-change} request. When the replica $s_i$ receives $(f+1)$ positive responses to its prep-view-change request (which implies that at least one healthy replica has agreed to perform this view-change), then it broadcasts to all a view-change request. The view change request includes the new epoch and a concatenation of the log. At this point, that replica stops accepting
messages for the current view. A replica receives at least $(f+1)$ logs from other replicas so that it will receive at least the biggest log. The $f+1$ healthy replicas will need to decide on a new leader, e.g., in Raft or Chain-replication and then prior to executing new reqs, the replicas needs to synchronize their state based on the logs. The new leader, needs to re-execute the protocol for each request in the ``longest'' log. Similarly, with the leader-validation the replicas can detect faulty leaders.




A faulty leader can introduce bogus operations by itself. However, this is indistinguishable from a Byzantine client that executes bogus operations and BFT does not protect against malicious clients that want follow the protocol. To avoid cases where the leader executes requests to overwrite the data, the message format could also include the clients' request. The replicas should then only executed requests that were originated by authenticated clients.

\fi
